Dealing with Popularity Bias in Recommender Systems for Third-party Libraries: How far Are We?

Recommender systems for software engineering (RSSEs) assist software engineers in dealing with a growing information overload when discerning alternative development solutions. While RSSEs are becoming more and more effective in suggesting handy recommendations, they tend to suffer from popularity bias, i.e., favoring items that are relevant mainly because several developers are using them. While this rewards artifacts that are likely more reliable and well-documented, it would also mean that missing artifacts are rarely used because they are very specific or more recent. This paper studies popularity bias in Third-Party Library (TPL) RSSEs. First, we investigate whether state-of-the-art research in RSSEs has already tackled the issue of popularity bias. Then, we quantitatively assess four existing TPL RSSEs, exploring their capability to deal with the recommendation of popular items. Finally, we propose a mechanism to defuse popularity bias in the recommendation list. The empirical study reveals that the issue of dealing with popularity in TPL RSSEs has not received adequate attention from the software engineering community. Among the surveyed work, only one starts investigating the issue, albeit getting a low prediction performance.

==> src/AMLinSE.tex <==

%\vspace{-.2cm}
%Section~\ref{sec:Definitions} provides a brief description of the main definitions for concepts used in this paper. To motivate our work, Section~\ref{sec:Example} presents an example where a snippet could cause harm to software systems. Finally, Section \ref{sec:Attacks} provides a categorization of the main types of attacks to general-purpose recommender systems so that they can be subsequently contextualized to RSSE.

This section introduces basic definitions necessary to understand AML for API recommenders, provides a motivating example for our work, overviews the types of attacks that can affect RSSE, and shows, in particular, how API/code snippet recommenders could be subject to AML attacks.

%Afterwards, in Section~\ref{sec:RSSE} we review state-of-the-art RSSE providing API function calls and code snippets, as well as analyze the threats they might be exposed to.
% into a system.  %external 

%================================
%Source code based recommendation systems can provide support for tasks such as how to use a given API or framework, provide hints on things missing from the code, suggest how to reuse or correct existing code, or help novices learn a new project, programming paradigm, language or style.
%================================

%programmers may search for. 




 

%"/usr/bin/logger " */r.exe"rm";/*

% \textsc{msg.getBytes()}

%By embedding and executing the t
%. For instance, a spyware may be disguised in a legitimate library, 




\subsection{Definitions} \label{sec:Definitions}
In the following  we introduce the concepts of APIs, declarations, software projects/libraries, and usage patterns by referring to the code snippet in Listing~\ref{lst:ExampleSnippet}.

\lstset{basicstyle=\normalsize\ttfamily, breaklines=true, xleftmargin=2em, frame=single, framexleftmargin=15pt, belowcaptionskip=10pt}
\begin{lstlisting}[caption={A snippet seen as harmless, but actually harmful.}, label=lst:ExampleSnippet, style=JavaStyle,captionpos=t,numbers=left,escapechar=|]
import java.io.OutputStream;
import java.net.Socket;

public class Test {
  public static void main(String[] args) throws Exception { |\label{line:main}|
	Test test = new Test();
	test.debug("hello");
  }
  public void debug(String msg) throws Exception { |\label{line:debug}|
	String s = "/usr/bin/logger ";
	Runtime r = Runtime.getRuntime();     
	if (System.getProperty("os.name").equals("linux")) {
		r.exec(s + msg);
	} else {
		Socket socket = new Socket("loghost", 514); |\label{line:socket}|
		OutputStream out = socket.getOutputStream(); |\label{line:out}|
		out.write(new byte[] {0x2A, 0x2F, 0x72, 0x2E, 0x65, 0x78, 0x65, 0x22, 0x72, 0x6D, 0x22, 0x3B, 0x2F, 0x2A }); |\label{line:code}|
		out.write(msg.getBytes());
	}
  }
}	
\end{lstlisting}

An \textit{API} is a source code unit that offers some reusable pieces of functionality, which can be used according to a precisely defined interface without the need to be aware of its implementation details. In this way, an API works as a black-box, favoring reuse and modularity~\cite{Parnas1971Information,robillard2009makes}.

%, \ie like a black-box.
% offered by a project
% an interface that abstracts a piece of
%This interface is meant to support reuse and modularity~\cite{Parnas1971Information,robillard2009makes}. 

A \textit{method declaration} comprises a name, a list of parameter types, a return type, and a body. A declaration may involve other method declarations as for instance, the \texttt{\hl{\small main(String[]\; args)}} declaration (Line~\ref{line:main}) that calls the method \texttt{\hl{\small debug(String\; msg)}} inside its body.

%$e \in D$. %is a call made from a declaration  to  
%$d \in D$, 
%An API $a$, \eg~the \textit{Criteria API} in Fig.~\ref{fig:originalCode}, consists of a set $T_X$ of public types, \eg~\textit{Socket} and \textit{OutputStream}. Each type in $T_{X}$ consists of a set of public methods and fields that are available to client projects, \eg the method \textit{createQuery} of the type \textit{CriteriaQuery}.

%\MAX{some reviewers may find this definition problematic, because a project contains other artifacts beyond classes. Second, it is not independent. Third, the source code elements may or may not be classes, even if we say we can restrict to classes}
A \textit{software project} $P$ includes the outcome of software development activities, which are performed to meet the requirements of the wanted system. Different programming languages can be employed to develop the artifacts building up a software project. By focusing on object-oriented programming languages, software artifacts mainly consist of classes defined in different declarations, \ie $D$. The example in Listing~\ref{lst:ExampleSnippet} can be considered as an explanatory and straightforward project even though, in practice, software projects are much more complex with a significant number of declarations and APIs. 

%\MAX{I added the reuse point below, otherwise the difference between library and project is unclear. However, why we have the constraint of ``maintained by a third party''? you can develop your own libraries. Clearly, in our scope only third-party libraries can be risky. We can define therefore the term ``third-party library'' instead of ``library''}
A \textit{library} is a software module/project providing reusable pieces of functionality.


%\MAX{must define what if $F$}
Each API consists of public methods $M$ and fields $F$ that are available to client projects (\eg see the \texttt{\small{\hl{getOutputStream()}}} method of the type \texttt{\hl{\small{java.net.Socket}}} as used in Listing \ref{lst:ExampleSnippet}).
An \textit{API method invocation} is a call made from a declaration $d \in D$ to another declaration $m \in M$. Finally, an \textit{API field access} is an entry to a field $f \in F$ from a declaration $d \in D$. The union of the set of API method invocations $MI$ and the set of field accesses $FA$ in $P$ results in the set of \text{API usage pattern} $U = MI \cup FA$. An \textit{API usage pattern} is a sequence $( u_1, u_2, ..., u_n )$, $\forall u_k \in U$.

%(or code snippet) 

%For the sake of presentation, in the scope of this paper the following terms are used interchangeably: \emph{method declaration} vs. \emph{declaration} and \emph{API} vs. \emph{invocation}.

\subsection{Motivating example} \label{sec:Example}

During the development process, programmers may look for and embed relevant APIs or code snippets useful for their tasks~\cite{Nguyen:2019:FRS:3339505.3339636}.
While this is a common practice as it helps increase productivity~\cite{DBLP:books/sp/rsse14/MensL14}, it also poses security concerns.

Let us consider a developer who is using a tailored tool to search for snippets relevant to her context. Such a type of system has been chosen as it represents a typical scenario in software development where the recommendation needs to be learned from public repositories, and the adoption of a malicious API or code snippet may put the software system under development at risk~\cite{10.1145/2976749.2978333}. 
There exist quite a large number of recommender systems that can provide APIs or code snippets. Among others,  
%Strathcona \cite{DBLP:conf/sigsoft/HolmesWM05}, 
XSnippet~\cite{10.1145/1167473.1167508}, MUSE~\cite{Moreno:2015:IUT:2818754.2818860}, MAPO~\cite{Zhong2009MAPO}, \UM~\cite{Wang2013Mining}, CodeKernel \cite{DBLP:conf/kbse/Gu0019}, or \FC~\cite{Nguyen:2019:FRS:3339505.3339636}, to name a few, are some of the most notable API recommenders. In this respect, we anticipate two %possible
scenarios in which the developer is trapped by hostile attempts as follows: She is provided with either \emph{(i)} APIs coming from legitimate libraries, which may trigger disruptions/fatal errors if being executed in certain contexts/under some usage scenarios; or \emph{(ii)} intentionally harmful APIs embedded in a fake library. 

%,9359479

% In the scope of this paper, we are interested in the first scenario, \ie mainstream APIs. 
%This section introduces a scenario where a software system can be compromised with imperceptibly malicious code snippets.

To illustrate the first scenario, \ie normal APIs causing fatal errors, we refer to the example\footnote{This code originates from the following blog post: \url{https://bit.ly/31R760l}} in Listing~\ref{lst:ExampleSnippet}. The Java-written snippet looks harmless as first sight, however, once being executed it has a severe consequence on the hosting client. To be concrete, 
the bytecode \texttt{\hl{\small 0x2A, 0x2F,..., 0x2F, 0x2A}} (Line~\ref{line:code}) corresponds to the following string: \texttt{\hl{\small */r.exe"rm";/*}}. The implication of 
the \texttt{\hl{\small out.write()}} method with the string as parameter 
in the Windows operating system is the deletion of 
random files.\footnote{The snippet is dangerous, and thus we advise against running it. Detailed explanations can be found in the original blog post.} In this case, while \texttt{\hl{\small out.write()}} is a \emph{native method} which comes from \texttt{\hl{\small java.io.OutputStream}} -- a mainstream library -- it still induces a detrimental effect in the hosting platform.% once being executed.

%/usr/bin/logger "
%At first sight, the code looks harmless, however once being invoked, it will delete all the files in the current directory.\footnote{The snippet is dangerous, and thus we advise against running it.}
%framexleftmargin=4.0em,
%\vspace{-.1cm}

The second scenario is when the developer is provided with intentionally harmful APIs embedded in a fake third-party library. %, and disguising it in a legitimate snippet with a copycat name, \ie one that closely resembles a popular API. 
As an example, Listing~\ref{lst:ExampleLibrary} depicts a third-party library with the \texttt{\hl{\small FileManager}} class, which wraps the malicious code in Listing~\ref{lst:ExampleSnippet} using the %disguised 
\texttt{\hl{\small writeLog()}} decla\-ration. Though the name has nothing to do with the code, it makes the declaration appear more legitimate, helping disguise the intent better~\cite{10.1145/3463274.3463809}. Eventually, the library is compiled and published as a JAR file.

%\clearpage

\begin{lstlisting}[caption={A third-party library to wrap malicious code.}, label=lst:ExampleLibrary, style=JavaStyle,captionpos=t,numbers=left,escapechar=|]
package tools;
import java.io.IOException;
import java.io.OutputStream;
import java.net.Socket;
public class FileManager {
  public void writeLog(String msg) throws Exception { 
    String s = "/usr/bin/logger ";
    Runtime r = Runtime.getRuntime();  
    if (System.getProperty("os.name").equals("linux")) {
      r.exec(s + msg);
    } else {
      Socket socket = new Socket("loghost", 514); 
      OutputStream out = socket.getOutputStream(); 
      out.write(new byte[] { 0x2A, 0x2F, 0x72, 0x2E, 0x65, 0x78, 0x65,
        0x22, 0x72, 0x6D, 0x22, 0x3B, 0x2F, 0x2A });
      out.write(msg.getBytes());
    }
  }
}	
\end{lstlisting}



Listing~\ref{lst:NewSnippet} is the new version of the project in Listing~\ref{lst:ExampleSnippet}, however it is rewritten by means of the library, which is embedded through the \texttt{\hl{\small import\; tools.FileManager}} directive (Line~\ref{line:import}). % tools.FileManager
%
%In our recent published work~\cite{EASE2021VP}, we already succeeded in manipulating also third-party library recommender systems. In this respect, we see that adversarial attacks using tailored APIs are highly feasible, and they can have disastrous consequences on the executing client.
%as a JAR file 
%
%\vspace{-.2cm}
%
The resulting snippet in Listing~\ref{lst:NewSnippet} is more compact, and it offers the same functionality as the project
in Listing~\ref{lst:ExampleSnippet}; however, all the intent is hidden in the library. The final usage pattern consists of only two API calls, \ie \texttt{\hl{\small FileManager\; fm\; =\; new\; FileManager()}} and \texttt{\hl{\small fm.writeLog()}}. In this way, attackers render their attempt more practical by exposing the code in Listing~\ref{lst:NewSnippet} to the public, waiting for the developer to take the bait.


%\vspace{-.1cm}



\begin{lstlisting}[caption={The new snippet using the third-party library.}, label=lst:NewSnippet, style=JavaStyle,captionpos=t,numbers=left,escapechar=|]
import java.io.OutputStream;
import java.net.Socket;
import tools.FileManager; |\label{line:import}|

public class Test {
  public static void main(String[] args) throws Exception{ 
 	FileManager fm = new FileManager();
	fm.writeLog("Kernel - Starting service");    
  }
}	
\end{lstlisting}

Such a type of attack is effective, as it can be tailored for any specific purpose, \eg creating a backdoor to render unauthorized access~\cite{DBLP:conf/ndss/WuGCHCD19} once being successfully invoked. However,  
it also requires additional effort to plant the malicious library in OSS platforms and to trick the developer into calling it. 


%wrapping all malicious code in an 
%\vspace{-.15cm}



At the same time, both scenarios may appear to be unrealistic, as the possibility of encountering such snippets/APIs under normal circumstances is low, \ie the developer would never come across the code when using recommender systems. However, by manipulating the training data in OSS platforms, \eg \GH, adversaries can boost up the snippets' visibility/popularity so that API recommenders will adopt and provide it to the developer. As such, the suggested snippet poses a potential danger to the software systems embedding it.



%In the scope of this paper, we limit ourselves to the problem of recommending APIs, both conventional ones with fatal effects, and those with malicious behaviors by their nature. 
%While this covers both the first and the second scenario, by the latter, as a prerequisite it is necessary to favor a fake library hosting malicious APIs to the developer. We consider the issue our future work.

%\MAX{I rewrote this but it needs to be checked better}
To reveal potential risks that maliciously handled training data might cause, in this paper, we start from the assumption that some users have already adversarially-manipulated training sets. 
%Note that in the context of this paper we start from the assumption that somebody has already manipulated a training set. 
It is out of our scope to develop mechanisms to inject malicious snippets on crowdsourced repositories (\eg on Stack Overflow) or make fake APIs become popular, \eg by boosting their stars/forks and adding pages on Q\&A forums.  
For the sake of presentation, in the rest of this paper, we call an API causing negative effects or errors as \emph{a malicious API}, regardless of its origin, \ie whether it comes from a legitimate or from a fake library.



%In the next subsection, we investigate the possibilities of conducting such an attack to recommender systems.

%are interested in consider the first attack scenario, 
% within the current folder

\subsection{Types of attacks to recommender systems} \label{sec:Attacks}


In a supervised learning task, given a training dataset D with $n$ pairs of input sample and the corresponding label $(x, y)$, 
where $x$ is the input sample, and $y$ is the corresponding class label, a classification is defined as seeking a candidate function that can predict the class label $y$ around the input sample $x$. 
%This boils down to solving an empirical risk minimization (ERM) problem by means of the following equation \cite{DDM20a}:
%\begin{equation}
%\underset{a}{min} \sum_{x,y\in D} l(f(x_{i},\theta ),y_{i}) 
%\end{equation}
%where $l(.)$ is the empirical risk function, or the loss function, $\theta$ is the model parameter. 
Adversarial attempts try to generate perturbed examples in the form of: $x_p$ = $x + \delta$, by means of a non-random perturbation $\delta$, which leads to an erroneous prediction, \eg misclassification.

Similarly, attackers to RSSE may try to craft the training data with their malicious examples which, once being recommended, can cause harm the target system. Adversarial attempts to recommender systems may belong to the following two main categories~\cite{10.1145/3463274.3463809}: %DDM20a

%\color{red}
%Attacks to recommender systems are classified into two main categories as follows \cite{DDM20a}: 

\begin{enumerate}
%	\noindent
	\item In \emph{poisoning attacks}, adversaries manipulate a model by fabricating its input data.
	\item Meanwhile, with \emph{evasion attacks}, hostile users dodge being detected by concealing bogus contents, which then will be classified as legitimate by ML models.
\end{enumerate}

Two interventions are possible with poisoning attacks: 

\begin{enumerate}
	\item \emph{Nuke attacks} attempt to downgrade/defame the targeted items \cite{10.1007/978-3-030-49461-2_18,4216981}, forcing them to vanish from the recommendation list. 
	\item In contrast, \emph{push attacks} promote the targeted items, aiming to boost their visibility/popularity. This will increase the possibility of being discovered and thus recommended by search engines.
\end{enumerate}

%\color{black}

Besides the aforementioned attacks, there are malicious behaviors that can affect specific types of recommender systems. For instance, memory-based collaborative filtering techniques suffer from average attacks \cite{lam_shilling_2004} in which fake users try to impersonate real ones using ratings. %Another common vulnerability of such systems is hubness \cite{10.1145/1835449.1835482}, which occurs especially with clustering algorithms. 
In the scope of this work, we focus on push attacks as they fit well to the example in Section~\ref{sec:Example}, \ie promoting malicious APIs so that they will be recommended to developers. We will cope with the other types of attacks in our future work.

%=================================================
%Once being embedded, a malicious library may force apps open port~\cite{DBLP:conf/ndss/WuGCHCD19}, ich allows for unauthorized access. A malicious API call may cause disruption to the whole software system. % A malicious API call may cause disruption to the whole software system.
%=================================================



%We also develop a new static diagnostic tool to reveal that 61.8% of the open-port apps are solely due to embedded SDKs, and 20.7% suffer from insecure API usages.


%\begin{figure}[t]
%	\centering
%	\vspace{-.1cm}
%	\includegraphics[width=0.86\linewidth]{figs/PushAttacks.pdf}
%	%\vspace{-.1cm}
%	\caption{Manipulating \GH repositories.} %Performing push attacks
%	\vspace{-.3cm}
%	\label{fig:PushAttacks}
%\end{figure}

\subsection{Push attacks to API and code snippet RSSE} 
\label{sec:InjectingAPIs}

As mentioned in Section~\ref{sec:Example}, although the code in Listing~\ref{lst:ExampleSnippet} is dangerous, it is unlikely that developers encounter something similar  under normal circumstances. 
To expose the code to recommenders, attackers need to manipulate the training data by performing a \emph{push attack} (see Section~\ref{sec:Attacks}). In such a misdeed, they forcefully favor the targeted items by boosting their popularity. This increases the possibility of being discovered and thus, recommended by search engines.


We encounter the following challenge: ``\emph{How should a fake API be planted, so that it will be incorporated by recommendation engines?}'' In fact, recommender systems rely heavily on similarity measures, \ie they employ algorithms to search for similar artifacts, which are used to deduce recommendations~\cite{10.1145/3463274.3463809}. This is the case not only for general-purpose recommender systems~\cite{Ricci2011}, but also for several RSSE~\cite{DBLP:conf/sigsoft/HolmesWM05,Moreno:2015:IUT:2818754.2818860,Nguyen:2019:FRS:3339505.3339636,10.1145/1167473.1167508,Wang2013Mining,Zhong2009MAPO}. For instance, library recommenders search for libraries from the most similar projects in the training data~\cite{NGUYEN2019110460,DBLP:journals/sqj/NguyenRRR20,6671293}. Similarly, various systems for providing APIs and code also exploit a similarity measure~\cite{Fowkes:2016:PPA:2950290.2950319,9359479}, or a kernel~\cite{DBLP:conf/kbse/Gu0019} to retrieve similar projects and snippets. More importantly, to produce recommendations, RSSE need to rely on 
OSS repositories, such as \GH, or Maven, which are subject to changes from the public. 


\begin{figure}[t!]
	\centering
	\vspace{-.1cm}
	\includegraphics[width=0.99\linewidth]{figs/PushAttacks.pdf}
	%\vspace{-.1cm}
	\caption{The process of manipulating \GH to promote malicious repositories.} %Performing push attacks
	\vspace{-.3cm}
	\label{fig:PushAttacks}
\end{figure}



Let us imagine a scenario in which one increases the popularity of malicious APIs\footnote{As stated in Section~\ref{sec:Example}, we consider an API malicious if it causes fatal errors, no matter where it comes from, \ie either a legitimate or a fake library.} by planting them to OSS projects, as many as possible. Fig.~\ref{fig:PushAttacks} illustrates the process in which attackers may exploit to plant malicious data. First, well-maintained repositories are forked from \GH, \eg those that have good indicators in terms of stars, forks, or watchers. Afterward, the projects are injected with fake APIs, and then uploaded back to \GH. Malicious repositories in \GH are not scarce, but \emph{dime a dozen}~\cite{Rokon2020SourceFinderFM}. To boost up the popularity of an API pattern, the APIs can be seeded into a significant number of declarations, for each training project. Attackers may create fake accounts to star, fork, and watch malicious repositories to increase their credibility/visibility, thus exposing them better to search engines.\footnote{Such manipulation has been recently revealed \url{https://zd.net/3bg3CK9}.}





==> src/APIRecSys.tex <==
%\begin{landscape}
\begin{table*}[t!]
	\centering
%	\vspace{-.3cm}
%	\footnotesize
	\scriptsize

	\caption{Notable RSSE for mining APIs and/or code snippets (Listed in chronological order).}
	\begin{tabular}{|p{1.80cm} | p{0.65cm} | p{0.4cm} | p{1.20cm} | p{5.2cm} |p{5.2cm} |  p{0.45cm} |}	\hline
		\textbf{System} & \textbf{Venue} & \textbf{Year} & \textbf{Data source} & \textbf{Working mechanism} & \textbf{Potential risks} & \textbf{Avail.} \\ \hline
%		& \multicolumn{4}{|c|}{\textbf{Library recommendation}} \\  \hline 
%        {\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Library rec.}}}} & LibRec~\cite{6671293} & WCRE & 2013 & \GH  \\ \cline{2-5} %WRCE\footnote{WRCE was the former edition of SANER}
%		& LibCUP~\cite{SAIED2018164} & JSS & 2017 & \GH  \\ \cline{2-5}
%		& LibD~\cite{7985674} & ICSE & 2017 & Android markets  \\ \cline{2-5}
%		& LibFinder~\cite{Ouni:2017:SSL:3032135.3032325} & IST & 2018 & \GH  \\ \cline{2-5}
%%		\rowcolor{verylightgray}
%		& CrossRec~\cite{NGUYEN2019110460} & JSS & 2020 & \GH  \\ \cline{2-5}
%		& LibSeek~\cite{9043686} & TSE & 2020 & Google Play, \GH, MVN  \\ \hline
%%		& \multicolumn{4}{|c|}{\textbf{API recommendation}} \\  \hline 
%in the repositories that is used to retrieve the API snippets.
%		\color{red}
		%Strathcona \cite{DBLP:conf/sigsoft/HolmesWM05} & ESEC/FSE & 2005 & Local repositories & Strathcona suggests relevant API usages by searching in a local code repository. It employs six different heuristics that compute the similarity at the structural level to increase the quality of the retrieved code snippets. \circledb{S}  & The system uses a local repository which is automatically generated from existing source code examples. Attackers can easily inject malicious APIs into such a knowledge-base to fool the developed heuristics. & \untick \\ \hline
%		\color{red}
		%XSnippet~\cite{10.1145/1167473.1167508} & OOPSLA & 2006 & Eclipse projects & Relevant API snippets are retrieved by invoking different queries that consider both the parents of the class and the lexical visible type. A graph-based mining algorithm is then used to deliver the final recommendations by employing a breadth-first search algorithm. \circledb{S} & As the underpinning algorithm mines common tree paths, a poisoning attack may succeed in altering the outcomes of the system by adding similar tree branches, \ie XSnippet can be deceived with fake projects containing bad classes and methods. & \untick \\ \hline
%		\color{red}
		%MAPO~\cite{Zhong2009MAPO} & ECOOP & 2009  & SourceForge & API patterns are recommended by extracting related information from developers' context using the BIDE mining algorithm~\cite{1319986}. The resulting data is clustered and ranked according to their similarity with the client code. \circledb{S} \circled{C} &  Since BIDE~\cite{1319986} works by mining from common patterns, MAPO can be steered by malicious code inserted into projects with popular API sequences. The clustering engine also contributes to the introduction of fake code to users. & \untick\\ \hline%\cline{2-6}
%		Precise~\cite{zhang_automatic_2012} & ICSE & 2012 & OSS projects \\ \hline
		%UP-Miner exploits SeqSim and BIDE to mine from source code. 
		\UM \cite{Wang2013Mining} & MSR & 2013  & Microsoft Codebase & \UM works on the basis of clustering, %is dependent on the similarity among API sequences. It 
		computing %In other words, UP-Miner computes 
		similarity at the sequence level, \ie APIs that are usually found together using BIDE~\cite{1319986}. Finally, it clusters to group frequent sequences into patterns.  \circledb{S} \circled{C} & Similar to MAPO, as \UM depends on BIDE, an attacker can inject malicious code in the training in projects disguised as similar to trick \UM. In this way, it may recommend to developers harmful snippets. & \tick\\ \hline
%		\color{red}
		MUSE \cite{Moreno:2015:IUT:2818754.2818860} & ICSE  & 2015 & Java projects  & MUSE automatically retrieves relevant API usages using static analysis techniques. It then ranks the resulting snippets employing code cloning detection as the similarity measure. \circledb{S}  & As it works by means of similarity among snippets, MUSE can be affected by malicious code embedded in similar projects planted in public platforms, \eg \GH. & \untick   \\ \hline %the conducted analysis is syntactic
%		\color{red}
		SALAD \cite{DBLP:conf/icse/NguyenPVN16} & ICSE & 2016 & Google Play & SALAD %is a statistical approach that 
		learns API usages directly from bytecode extracted from Android apps. It relies on a hidden Markov model that predicts relevant API patterns according to their probabilities. \circledb{S} & Since the most probable usages are retrieved as recommendations, a hostile user may plant malicious bytecode in Google Play to trick SALAD into recommending to developers. & \untick \\ \hline % should be enough to compromise the recommendation capabilities		
		DeepAPI \cite{Gu2016DeepAPI} & ESEC/ FSE & 2016  & \GH & DeepAPI generates relevant API sequences starting from a natural language query. It employs an Encoder-Decoder RNN
		to encode words in context vectors. %used to train the model. %Given a corpus of annotated API	sequences, %\ie $<$API sequence, annotation$>$ pairs, 
		DeepAPI trains a model that encodes natural language annotations and API sequences. 
		Afterwards, it uses the model to compute a list of API sequences. \circledb{S} & An RNN bases also upon the notation of similarity, %DeepAPI learns from API sequence and textual annotation pairs, 
		thus a malicious user can forge API sequence and textual annotation pairs to spoil the recommendations. First, she can remove or change part of the textual annotation or even worst, mix annotations and API sequences. Second, she may inject malicious APIs into sequences. %The former deceptions impact the prediction performance, while the latter ones are even worst: they can compromise the outcoming API sequences with fake invocations. 
		&  \untick \\ \hline
		%As the corpus is collected from \GH projects, a hostile user can easily inject perturbations during the data gathering phase, \ie feeding the system with interfered projects. \\ \hline
%		\light
		PAM \cite{Fowkes:2016:PPA:2950290.2950319} & ESEC/ FSE & 2016 & \GH & %PAM %~\cite{Fowkes:2016:PPA:2950290.2950319} 
		%extracts relevant API patterns from client code by using the structural Expectation-Maximization (EM) algorithm to 
		%infer the most probable items. The mined API patterns are then ranked according to their probability. 
%		PAM consists of six building blocks, \ie probabilistic model, inference, learning, inferring new API patterns, candidate generation, and mining interesting API patterns. 
		%PAM uses a probability function to 
		PAM defines a distribution over all possible API patterns in client code, based on a set of patterns. It uses a generative model to infer the most probable patterns. The system generates candidates by relying on the highest support first rule.  \circledb{S}%, \ie searching for the best candidate. %earlier. %Due to these technical details, 
		&  PAM recommends API calls that commonly appear in different code snippets. Thus, push and nuke attacks could modify the final ranking obtained by the tool, \ie operating on terms' occurrences to favor or defame a certain API pattern. & \tick\\ \hline
%		\textsc{fine-GRAPE}~\cite{sawant_fine-grape_2017} 
		\textsc{fine-GRAPE} \cite{sawant_fine-grape_2017} & EMSE & 2017 & \GH & Relying on the history of the related files, \textsc{fine-GRAPE} parses \GH projects, discovers, and ranks the relevant API calls according to their history from every API version. \circledb{S} &  Manipulations that forge history of API calls in projects can pose a threat to the system. Another pitfall can be represented by the Java code that the tool parses to get relevant API patterns.& \untick \\ \hline
		\FC \cite{9359479,Nguyen:2019:FRS:3339505.3339636} & ICSE & 2019 & \GH, Maven, Google Play & \FC suggests APIs by encoding projects in a tensor and using a collaborative-filtering technique to deliver the list of APIs. Eventually, it mines APIs and snippets from similar projects with a graph representation. \circledb{S} & The system is susceptible to poisoning attacks, \ie an adversary can create fake similar projects containing toxic APIs and pose them as legitimate to deceiving \FC into recommending these calls/snippets. & \tick\\ \hline
		CodeKernel \cite{DBLP:conf/kbse/Gu0019} & ASE & 2019 & Java projects & A graph-based representation is used to cluster similar API calls. Then, the system computes graph similarity by means of kernel functions. Code is selected according to designed ranking metrics, \ie specificity and centrality. \circledb{S} & Since its kernel functions work on graph structure, CodeKernel can be fooled by copycat Java APIs that closely resemble normal ones. Attackers can insert fake code in the graph embedding process to disguise them as similar. & \untick \\ \hline
%		Quality-aware 
%<<<<<<< HEAD
		%=======================================
%		WebAPI~\cite{DBLP:conf/scc2/Fletcher19} & SCC  & 2019 & Programmable Web  & A matrix factorization technique is combined with a quality feature model to recommend accurate Web APIs. The Hierarchical Dirichlet Process and Jensen-Shannon divergence are used to compute the similarity and retrieve the final results. &  Similar to \UM, the similarity module can recommend malicious APIs if the tool is fed with %crafted projects, \ie those that contain manipulated code. As we are in the web domain, those attacks can affect sensitive information \eg authorization keys, personal data. & \untick\\ \hline
		%=======================================
		AuSearch \cite{DBLP:conf/wcre/AsyrofiT0J20} & SANER & 2020 & \GH, Maven & %Given a query, 
		AuSearch discovers API usages from \GH by converting the input query into a \GH query %to retrieve relevant files. 
		and searches for types of parameters that match with the ones contained in the query. It also relies on the Maven Package Search API algorithm to look for similar packages. \circledb{S} & The tool is prone to poisoning attack with project containing malicious packages. Furthermore, an attacker can use JAR files obtained from fake projects to spoil the package analyzer module which works on top of the Maven Package Search API algorithm.
 & \untick \\ \hline
		%=======================================		
%=======
%		WebAPI~\cite{DBLP:conf/scc2/Fletcher19} & SCC  & 2019 & Programmable Web  & The tool combines matrix factorization technique with a well-founded quality feature model to recommend accurate web APIs. The Hierarchical Dirichlet Process (HDP) and Jenssen-Shannon divergence have been employed to compute the similarity and retrieve the final results.  &  Similar to UP-miner, the similarity module can recommend malicious APIs if the tool is fed with fake projects. & No\\ \hline

%AuSearch \cite{DBLP:conf/wcre/AsyrofiT0J20} & SANER & 2020 & Github &AUSearch \cite{DBLP:conf/wcre/AsyrofiT0J20} has been conceived to discover API usages from Github repositories given an initial query. The tool turns such a query into a Github Query to retrieve relevant Java files. AUSearch eventually filters the outcomes by searching for types of parameters that match with the ones contained in the user query. & The tool is prone to poisoning attack if the malicious Github project are analyzed & No \\ \hline
%>>>>>>> e8f76db8e35dc19cd3f62b8c7a50adf98fb846a3
		 
%	 	PyART~\cite{he_pyart_2021} & ICSE  & 2021  & \GH &
%		PyART is a recommender system with the aim to suggest the next APIs for Python programs by inspecting the developer's context. Because Python programs are dynamically typed, it uses a light-weight analysis to derive the optimistic data-flow and infer an element's type. If the type inference is successful, all the callable methods of the inferred type are possible API candidates. Otherwise, API candidates are extracted from imported libraries and all the callable methods declared in the current context.  
%		Each candidate is represented by a feature vector consisting of optimistic data-flow hints, the token similarity, and the token co-occurrence hints. Similarly, the feature vectors are extracted from the projects in the training corpus. The feature vectors train a Random Forest recommendation model that is used to ranks all the extracted candidates.
%	 	% It recommends APIs for Python in real-time by excerpting three kinds of features from the developer's context. These features are eventually used to feed a Random Forest predictive model.  
%	 	&  PyART is less prone to the manipulation of the training data. First of all, it tries to infer the type of elements defined in the developer's context to compute the possible candidates. If the type is properly identified, the candidates are real APIs. Otherwise, PyART extracts possible candidates from imported libraries that are dynamically included from pip repositories. It makes the inject fake API as candidates difficult. Though mining projects with fake APIs can cheat the Random Forest recommendation models, it only impacts the candidates' rank. &  \\ \hline
		
%		\multicolumn{4}{|c|}{\textbf{Library migration recommendation}} \\  \hline 
%		Meditor \cite{xu_meditor_2019} & ICPC &2019 & \GH  \\ \hline
%		RAPIM \cite{alrubaye2019learning} & ASOC &2020 & \GH  \\ \hline        
		
%		\multicolumn{4}{|c|}{\textbf{Post recommendation}} \\  \hline 
%		PROMPTER~\cite{DBLP:journals/ese/PonzanelliBPOL16} & EMSE & 2014 &	Stack Overflow \\ \hline
		
		% 	     {\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{ML/DL}}}} & &  &	 &  & \\ \hline		
		%		 DeepTest~\cite{10.1145/3180155.3180220} & ICSE & 2018  &	 &	Software testing \\ \hline
		%		 Clone~\cite{7985645} & ICSE & 2017 &	 &	Software clone \\ \hline
	\end{tabular}
%
	\vspace{-.2cm}
	\label{tab:summary}
\end{table*}

%\end{landscape}


==> src/Approach2.tex <==
%\revised{%\subsection{Attack detection and countermeasures}
%Depending on the type of the consider RSSE, the literature is plenty of possible strategies to neutralize or reduce the negative effects of an adversarial attack. Mobasher \etal \cite{mobasher_attacks_2007} employ two different techniques to detect malicious attacks that involve recommended items \ie profile classification and anomaly detection. The former employs a classifier that makes use of attribute-reduction techniques to create a lower-dimensional training set. The underpinning model analyzes generic profile attributes as well as intra-profile and model-specific ones. The conducted evaluation shows that the proposed model can properly classify malicious users considering a well-defined set of metrics. Concerning anomaly detection problem, the work makes use of statistical process control (SPC) strategy to identify suspicious items trends. To this end, the model examines the items considering two parameters \ie the density of the distribution and the average ratings. The results demonstrate that detecting push attacks for popular items is more difficult while the SPC model correctly identifies attacks against low-density items. A recent work \cite{si_shilling_2020} highlights other possible countermeasures. Similar to supervised techniques, semi-supervised and unsupervised approaches have been developed with the aim of detecting attacks coming from pretended profiles. An alternative strategy could be the development of a robust recommendation algorithm that avoids possible attacks in advance. Several approaches employ matrix factorization or kernel distance even though trust-aware recommender systems are more robust than traditional ones \cite{DBLP:journals/corr/abs-1207-4525, 5428690}.
%Concerning shilling that exploits hubness, Hara \etal \cite{10.1145/2766462.2767823} propose an approach to increase the robustness of memory-based recommender system. To this end, the similarity measure exploited by the K-NN algorithm is transformed to reduce the bias that causes hubness. }


Both \LR and \CR suggest to active projects, \ie the ones under development, by searching for libraries from the most similar projects in the training data~\cite{NGUYEN2019110460}. For instance, the developer is searching for libraries for parsing JSON documents and the system should be able 
to suggest those that are used by similar projects. 
We simulate an attacker attempting 
to inject a library with malicious code (\eg by referring to the previous example, a malicious JSON parser), let it be $lib^{*}$, into the active projects. \revised{In practice, to avoid being detected, an attacker normally names $lib^{*}$ using a copycat name, aiming to disguise it. For instance, .}
Given that under the normal circumstances, the systems would never recommend $lib^{*}$ since the library has not been invoked anywhere.
To this end, we forcefully favor $lib^{*}$ using 
push attacks (cf. Section~\ref{sec:Classification}), so that, in the end,
the library will be suggested to projects.

% and to deceive developers
%ai.grakn:grakn-engine:2016-11-22
%To this end, w %that appear to be similar to the target ones. We exploit a 

%<<<<<<< HEAD
%When \LR and \CR learn from existing projects and when they provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}. This resembles ratings of a user profile in online shopping systems.
%%We craft a set of forged projects exploiting a well-known technique to populate their ratings~\cite{4216981}. By the original approach~\cite{BWMB06}, a profile is divided into four independent parts, \ie \emph{unrated}, \emph{filler}, \emph{selected}, and \emph{target}. 
%To attack a recommender system, there are various approaches to populate fake user profiles~\cite{BWMB06,4216981}. Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). \MAX{this part is unclear, I think those are 2 separate problems. I think here we can only say how we create a training set for the tools, then we have to explain that a project would fall in the training set if it has good ratings, and there are ways to fake the ratings, but we did not simulate this here to avoid violating github terms of service}
%Thus, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (cf. Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%=======

\revised{\subsection{Populating fake projects}}
When \LR and \CR learn from existing projects to %and when they 
provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}.
To attack a recommender system, there are various approaches to populate ratings for fake user profiles~\cite{BWMB06,4216981}. 
Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). 
Thus, to create a training set for the \LR and \CR tools, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (cf. 
Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.


We come across the following question: 
``\emph{Which libraries should be chosen as fillers, so that the fake project will be incorporated into the recommendation?}'' In fact, recommenders heavily rely on similarity~\cite{Schafer:2007:CFR:1768197.1768208}, thus we come up with the selection of popular libraries as fillers. Our intuition 
is that, a fake project with libraries widely used by other projects is likely to get attention from the recommendation engine. 
A list of libraries in the training projects is populated and sorted in descending order of the number of caller projects. A certain number of the most popular libraries is then randomly selected.

%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\gamma$ is the number of fillers. For \LR and \CR, \emph{k} is the number of similar projects and \emph{N} is the cut-off value for the ranked list of recommendations~\cite{6671293,NGUYEN2019110460}. We conducted experiments using ten-fold cross-validation on a dataset crawled from \GH consisting of 1,400 projects and 13,497 libraries. For a testing project, we randomly split its libraries into two equal parts, the first part is used as a query, while the second one is ground-truth data. To measure the effectiveness of the push attacks, we use \emph{Hit ratio} \emph{HR@N}, 
%defined as the ratio of projects being recommended with $lib^{*}$ to the total number of testing projects~\cite{10.1007/978-3-030-49461-2_18}. 
%To measure the accuracy, we use success rate \emph{SR@N}, \ie the ratio of projects getting at least a matched library (the size of the intersection of the recommended list with the ground-truth data is larger than 0) to the number of testing projects.
%We experimented with $\alpha$=$\{5\%,10\%\}$ as attack size; 
%$k$=$\{5,10,15,20\}$; $\gamma$=$\{3,4,6,8,10\}$ as fillers' size. The calibration of these parameters allows us to simulate \emph{stress tests}, aiming to investigate the systems' safeness under different working conditions. 


\begin{figure}[t!]
	\centering
	\vspace{-.3cm}
	\includegraphics[width=0.68\linewidth]{figs/FakeProject.pdf}
	\vspace{-.3cm}
	\caption{Manipulation of library usages for a fake project.}
	\label{fig:FakeProject}
%	\vspace{-.3cm}
\end{figure}



%\revised{\subsection{Detection and countermeasures}
%	Depending on the type of the consider RSSE, the literature is plenty of possible strategies to neutralize or reduce the negative effects of an adversarial attack. Mobasher \etal \cite{mobasher_attacks_2007} employ two different techniques to detect malicious attacks that involve recommended items \ie profile classification and anomaly detection. The former employs a classifier that makes use of attribute-reduction techniques to create a lower-dimensional training set. The underpinning model analyzes generic profile attributes as well as intra-profile and model-specific ones. The conducted evaluation shows that the proposed model can properly classify malicious users considering a well-defined set of metrics. Concerning anomaly detection problem, the work makes use of statistical process control (SPC) strategy to identify suspicious items trends. To this end, the model examines the items considering two parameters \ie the density of the distribution and the average ratings. The results demonstrate that detecting push attacks for popular items is more difficult while the SPC model correctly identifies attacks against low-density items. A recent work \cite{si_shilling_2020} highlights other possible countermeasures. Similar to supervised techniques, semi-supervised and unsupervised approaches have been developed with the aim of detecting attacks coming from pretended profiles. An alternative strategy could be the development of a robust recommendation algorithm that avoids possible attacks in advance. Several approaches employ matrix factorization or kernel distance even though trust-aware recommender systems are more robust than traditional ones \cite{DBLP:journals/corr/abs-1207-4525, 5428690}.
%	Concerning shilling that exploits hubness, Hara \etal \cite{10.1145/2766462.2767823} propose an approach to increase the robustness of memory-based recommender system. To this end, the similarity measure exploited by the K-NN algorithm is transformed to reduce the bias that causes hubness. }
%poisoning attacks that manipulate projects 

==> src/Countermeasures.tex <==
Something goes here.



==> src/Countermeasures2.tex <==
In the following, we first discuss the feasibility of the RSSE attacks.  Afterward, we overview possible defense mechanisms based on existing techniques, which are expected to be applicable for protecting RSSE against AML attacks.

%\smallskip

%\noindent
\subsection{Feasibility of the attacks} 
%\MAX{I would avoid the following question } A question that might arise at anytime is: ``\emph{How likely are the attacks in practice?}'' 
%Developers are increasingly using recommender systems  to support their daily tasks~\cite{10.1145/3183440.3195011}.
%, and for their convenience, various RSSE have been successfully integrated into the Eclipse IDE~\cite{9359479},\cite{DBLP:journals/ese/PonzanelliBPOL16}, providing recommendations -- \emph{on the fly} -- while they are programming. 
%that RSSE are fed with manipulated data. 
RSSE rely on third-party data sources, \ie they are usually fed with data from OSS repositories, which are open for changes including the phony ones. The probability that RSSE come across toxic sources cannot be ruled out.  There are precedents where thousands of repositories with malware apps have been unearthed in \GH~\cite{Rokon2020SourceFinderFM}, and they might be only \emph{the tip of the iceberg}. %, waiting. 

Though RSSE attempt to crawl training data from repositories considered to be \emph{credible}~\cite{NGUYEN2019110460}, \eg having a significant number of stars, forks, or watchers, unfortunately, this cannot help them completely evade toxic repositories. These metrics, however, can be falsified as attackers use fake accounts to star, fork, and watch the malicious repositories, making them appear more legitimate. Such a trick has been recently revealed, where several fake accounts are used to reciprocally endow their malicious repositories.\footnote{\url{https://zd.net/3bg3CK9}} To our knowledge, research conducted to fight this type of abuse is still in its initial phase~\cite{10.1145/3357384.3357971}. %,Rokon2020SourceFinderFM
Thus, techniques to conduct attacks are known, and there are at least examples of fake repositories, albeit being created for other purposes rather than for attacking RSSE. 

Adversaries may also have different ways to camouflage their hostile intent. Apart from wrapping malicious code in a single API call (see Section~\ref{sec:Example}), they might disguise it with a typosquatting name~\cite{10.1145/3463274.3463809}, \ie one that closely resembles a popular API. In this case, developers would adopt the disguised API/snippet without the least delay, once it is provided by the recommendation engine.

Finally, the results obtained in RQ$_2$ suggest that even with a small amount of artificial training data, hit ratios are always larger than 0, implying that clients are being provided with the fake APIs. Altogether, we see that API recommender systems are likely to be exploited, and in this way they inadvertently become a \emph{trojan horse}, causing havoc to software systems. 

%\MAX{the box below does not add much. I'd just say that techniques to conduct an attack are known, and there are at least examples of fake repositories, although created for purposes different than for attacking RSSE.}

%\vspace{.1cm}
%\begin{shadedbox}
%	\footnotesize{\textbf{Summary.} The probability that users of API/snippet RSSE are fooled by malicious data cannot be ruled out, leaving attacks substantially feasible.}
%\end{shadedbox}

%============================
%crime %misbehaviour
%, aiming to bait developers
%though developers trust their 
%Attackers may plant projects in OSS platforms and wait for their victims, like they go fishing.  
%and this is out of. As a matter of fact,
%. In this case, they only need to favor a handful of APIs instead of some, making attacks more feasible. Moreover, to avoid being detected
%In this case, an attacker may need to disguise a planted project by falsifying this information, \eg by starring and forking with forged accounts (\untick). 
%. Moreover, to increase their credibility/visibility,
%In fact, such an incident has been recently reported, where hundreds of \GH repositories promoting malware apps have been discovered. \ie they may rack up one day. They may increase the credibility of their planted projects by.
%
%Such a trick has been recently revealed, where 
%Moreover, to increase their credibility/visibility, attackers use fake accounts to star and watch malicious repositories.\footnote{\url{https://zd.net/3bg3CK9}} To our knowledge, research conducted to combat this type of misdeed is still in its infancy~\cite{Rokon2020SourceFinderFM}. 
%As a result, there is the need to favor a handful of APIs instead of some, making attacks more feasible. Moreover, to avoid being detected, they might disguise the code with a typosquatting name, \ie one that closely resembles a popular API. In this case, developers would adopt the disguised API without the least delay, once it is suggested by the recommendation engine. 
%abuse %crime %misbehaviour 
%\footnote{\url{https://zd.net/3bg3CK9}} 
%To our knowledge, research conducted to combat this type of misbehaviour is still in its initial phase~\cite{10.1145/3357384.3357971,Rokon2020SourceFinderFM}. 
%In case of a fake library, attackers may enclose all malicious code in a single API call (see Section~\ref{sec:Example}). 
%\emph{(i)} Android programming is becoming more popular, and developers are increasingly using recommender systems to assist their daily tasks~\cite{10.1145/3183440.3195011}; and \emph{(ii)} the adoption of intentionally manipulated APIs provided by recommender systems will infect apps with malicious code, causing probably disastrous consequences for mobile users.
%The second scenario is when the developer is provided with intentionally harmful APIs embedded in a fake third-party library, and disguising it in a legitimate snippet with a copycat name, \ie one that closely resembles a popular API. 
%To disguise the planted projects, attackers create fake accounts to star, fork, and watch malicious repositories to boost their credibility/visibility, thus exposing them better to search engines. 
%Referring back to the example in Listing~\ref{lst:ExampleSnippet}, attackers need to promote the following pattern: 
%\texttt{\hl{\small Socket\; socket\; =\; ...}} (Line~\ref{line:socket}), \texttt{\hl{\small OutputStream\; out\; =\; ...}} (Line~\ref{line:out}), and \texttt{\hl{\small out.write()}} (Line~\ref{line:code}). %, and then upload them to OSS platforms. 
%While this covers both the first and the second scenario, by the latter, as a prerequisite it is necessary to favor a fake library hosting malicious APIs to the developer. In our recent published work~\cite{EASE2021VP}, we succeeded in manipulating third-party library recommendation.
%To simplify the evaluation, we generated fake projects at the metadata level, \ie we assume that all projects have been successfully fetched from \GH.\footnote{We mined library usage directly from \emph{pom.xml} files.} In practice, it is necessary to plant these projects in \GH to make them appear as legitimate (\untick).
%============================
%for recommender systems in other domain to contextualize. We concentrate on analyzing 
%contextualizing 
%recommender systems in other domains,  to contextualize to RSSE.  
%Similarity, \ie marked with \circledb{S} in Table~\ref{tab:summary}. There have been some possible strategies proposed to neutralize or reduce the negative effects of an adversarial attack.
%collaborative-filtering recommender systems, 
%============================


%\smallskip
%\noindent
\subsection{On the quest for potential countermeasures}
While the topic of AML has been studied in different domains, there is no work dealing with adversarial attacks to RSSE (see Section~\ref{sec:RQ1}). Also, there exist no concrete countermeasures that can be instantly applied to protect RSSE against attacks. 

In the following, we discuss possible defense mechanisms from two perspectives, namely \emph{(i)} internal view, \ie design of recommender systems; and \emph{(ii)} external view, \ie techniques to detect and protect against hostile attempts. Concerning the former, we study counteractions proposed for generic recommender systems in the hope of customizing them for RSSE. Concerning the latter, we look for feasible ways to recognize and seize malicious APIs.% and protect RSSE. %API recommender systems.%anomaly detection techniques that can be used for API recommenders.

To \textbf{minimize the effect of manipulated profiles}, model-based algorithms are of great use as they can be applied to cluster similar profiles (OSS projects) into \emph{aggregate segments}~\cite{mobasher_attacks_2007}. Though these techniques cannot entirely isolate malicious projects, this aims to lessen the prevalence of projects with abnormal behaviors, \ie they will not be seen as similar to any active projects, \ie the ones under development. In this way, such a method reduces the possibility that RSSE select and incorporate bogus data, thereby avoiding attacks. The method can be applied to defend RSSE that work based on a similarity or collaborative-filtering technique, such as \UM \cite{Wang2013Mining}, MUSE \cite{Moreno:2015:IUT:2818754.2818860}, \FC~\cite{9359479}, or CodeKernel \cite{DBLP:conf/kbse/Gu0019}. Nevertheless, it requires the redesign of the whole systems' underpinning building blocks, and thus, it is not easy to conduct.  %Furthermore, it may not be applicable to other systems, such as MUSE, or.

Adversarial attacks can be counteracted using \textbf{anomaly detection techniques}, \ie recognizing malicious API patterns before they are recommended to developers. %There have been approaches conceived to detect malicious API sequences. 
For instance, a statistical process control strategy~\cite{mobasher_attacks_2007} has been used to identify suspicious items by examining two parameters, namely items' distribution density and average ratings. By referring to RSSE, we can think of detecting anomalies from the distributions of APIs in projects and declarations. This, however, necessitates careful analyses to avoid false positives and false negatives. As shown in Section~\ref{sec:rq2-design}, the distributions of APIs may span in a wide range, \ie there are not only extremely popular APIs but also rare ones. Thus, being based on a radical pattern, \eg a too popular or too rare one, the detection of malicious APIs may not succeed in every case. A more tailored approach is to tell malicious/benign API sequences apart by monitoring a certain set of third-party libraries using supervised classifiers~\cite{10.1109/COMPSAC.2015.241}. Such an approach, however, has its limitation as follows. Though it can detect malicious sequences consisting of APIs from a specific set of libraries, it may not be applicable to patterns with a few APIs coming from a less popular library. 

\textbf{Profile classification} can also help increase the resilience of RSSE against malicious attacks~\cite{10.1145/1097047.1097061}. First, it is necessary to build a training set consisting of both authentic projects and fake projects that are generated following an attack model. Attribute-reduction techniques may be used to reduce the number of features needed to represent the dataset. Afterward, supervised classifiers are trained on the resulting dataset to classify real and fake projects, aiming to detect the injection of malicious data. This technique works more effectively when we have enough training data by taking into consideration different ways of populating fake projects.

In conclusion, we believe that a hybrid security model, consisting of countermeasures pertaining to both an internal (design) and external view, is likely to contribute to the robustness and resilience of RSSE towards adversarial attacks. While internal countermeasures allow RSSE to avoid falsified or suspicious data sources, defense mechanisms based on external view help RSSE detect malicious intent hidden in API patterns before recommending them to developers.%, RSSE may check for its eligibility.

% a lower-dimensional training set is created, exploiting . Then, 
%The project each profile as being part of an attack or as coming from a genuine user. 
%Supervised classifiers can be used to create a lower-dimensional training set by means of attribute-reduction techniques. The underpinning model analyzes generic profile attributes as well as intra-profile and model-specific ones. 
%The conducted evaluation shows that the proposed model can properly classify malicious users considering a well-defined set of metrics.
% Statistics are computed over projects to create a 
%We use a supervised classification approach to detect and respond to profile injection attacks.
%The former employs a classifier that
%Two different techniques~\cite{mobasher_attacks_2007} have been used to detect malicious attacks that involve recommended items, \ie 
%A recent work \cite{si_shilling_2020} highlights other possible countermeasures. \MAX{for what? the previous sentence refers to malicious api sentences} Similar to supervised techniques, semi-supervised and unsupervised approaches have been developed with the aim of detecting attacks coming from pretended profiles. An alternative strategy could be the development of a robust recommendation algorithm that avoids possible attacks in advance.
%\MAX{the next sentence is a detail, just mention the related work.}
% Several approaches employ matrix factorization or kernel distance even though trust-aware recommender systems are more robust than traditional ones \cite{DBLP:journals/corr/abs-1207-4525, 5428690}.

%a, \ie that an 
%\MAX{the next paragraph can go away}
%The study has been conducted to secure machine learning algorithms by three golden rules. \textit{(i) Know your adversary}: attacker’s goal, knowledge, and strategy should be considered when a countermeasure is considered.  \textit{(ii) Be proactive}: simulating attacks (\eg injecting fake training data or mutating or manipulating testing inputs) is generally a good way to test machine learning algorithms' robustness. Finally, \textit{(iii) protect yourself}: how to react to past attacks and prevent future ones (\eg reactive or proactive defense).

%\MAX{I suggest the box below classifies the various countermeasures. But at this point I'm wondering whether a very small table couldn't be better.}



%==============================================================================
%Supervised classifiers are then trained and used to detect. 
%s. To this end, the model examines the items considering
%and monitored their constituent APIs to extract malicious/benign sequences
%Malicious API patterns can also be detected via the monitoring of 
%Fan \etal~\cite{10.1109/COMPSAC.2015.241} selected a
%The results demonstrate that detecting push attacks for popular items is more difficult while the SPC model correctly identifies attacks against low-density items. 
%==============================================================================
%\vspace{.1cm}
%\begin{shadedbox}
%	\footnotesize{\textbf{Summary.} Though there exist relevant methods that can be applied to protect RSSE, protecting . Thus, there is the need for decent countermeasures tailored to combat push attacks to API recommender systems.}% described in Section
%\end{shadedbox}
%==============================================================================
%Hara \etal  propose an approach . %Concerning shilling that exploits hubness, 
%Similarly, to increase the robustness of memory-based recommender system, the similarity measure exploited by the \emph{k-nn} algorithm is transformed to reduce the bias that causes hubness~\cite{10.1145/2766462.2767823}. 
%There are different studies conceived to detect anomalies. 
%==============================================================================
%Biggio \etal \cite{BIGGIO2018317} provided an overview of the evolution of AML in different lines of work (\eg image recognition, spam emails detection) over ten years of research. 
%In this respect, a segment manipulated projects are supposed to be. 
%Mobasher \etal \cite{mobasher_attacks_2007} employ 
%Mobasher \etal \cite{mobasher_attacks_2007} proposed using 
%==============================================================================
%We attempt to find feasible ways to detect malicious APIs and protect API recommender systems. 
%Nevertheless, this. However, This type of attack cannot be detected with conventional methods, which are based on grouping of API sequences. 
%\noindent
%$\rhd$~\textbf{\rqthird} 
%\textbf{Countermeasures:} 
%While we can inject the malicious library, the overall accuracy is not affected.
%\vspace{-.1cm}
%\subsection{Discussions} \label{sec:Discussions}
%\vspace{-.1cm}
%This section discusses the applicability of the attacks as well as countermeasures. 

%We consider the issue our future work.
%This subsection discusses the perspective of an attacker who wants to \textit{compromise the security of a system (marked with \untick)}, and that of an administrator who \textit{defends the system against hostile attempts (marked with \tick)}.

%While in the evaluation we performed only push attacks, the same methodology can be applied to conduct nuke attacks, \ie removing a useful library from the recommendations (\untick). Moreover, we tried with only one malicious library, however the evaluation can easily be extended to a set of libraries.

%We considered different settings for \LR and \CR, and this aims at studying the systems' capability in various conditions. In practice,  
%an attacker may not be aware of such internal design, 
%what matters is how she populates fake projects so that the malicious 
%library will be recommended (\untick), regardless of the systems' 
%configurations.

%To simplify the evaluation, we generated fake projects at the metadata level, \ie we assume that all projects have been successfully fetched from \GH.\footnote{We mined library usage directly from \emph{pom.xml} files.} In practice, it is necessary to plant these projects in \GH to make them appear as legitimate (\untick). Aiming for credible sources, a recommender usually chooses to crawl only from repositories with a considerably large number of stars and/or forks, or whatever criterion a recommender uses for selecting its training set (\tick)~\cite{NGUYEN2019110460}. 
%In this case, an attacker may need to disguise a planted project by falsifying this information, \eg by starring and forking with forged accounts (\untick). Thus, there is a need for mechanisms to detect this type of fabrication (\tick). 

%While in the scope of this paper, we addressed only RSSE for third-party libraries and API calls, we suppose that the same methodology can be generalized to other types of recommendations, such as post recommendation. Thus, we plan to investigate ... %We suppose that this type of attacks can be used to compromise many recommender systems in Software Engineering due to its efficacy. Thus, it essentially poses a threat to.

%To penetrate a system, the introduction of a library is just the first step. The second step is to trick developers into invoking the library by calling its functions.

%Thus, an adversary needs also to steer API or code recommenders (\untick), \eg the ones recently published~\cite{Fowkes:2016:PPA:2950290.2950319,Nguyen:2019:FRS:3339505.3339636,sawant_fine-grape_2017}.
%We conjecture that a technique similar to what described in Section~\ref{sec:Settings} can be used for injecting toxic APIs.

%\vspace{-.1cm}

%In the experiments, various internal settings were considered, and this aims at studying the systems' capability in different working conditions. In practice, an attacker may not be aware of such internal design, what matters is how she populates fake projects so that the malicious library will be recommended (\untick), regardless of the systems' configurations.





%Aiming for credible sources, a recommender usually chooses to crawl only from repositories with a considerably large number of stars and/or forks, or whatever criterion a recommender uses for selecting its training set (\tick)~\cite{NGUYEN2019110460}.



%In this case, an attacker may need to disguise a planted project by falsifying this information, \eg by starring and forking with forged accounts (\untick). In fact, such an incident has been recently reported, where hundreds of \GH repositories promoting malware apps have been discovered. Moreover, to increase their credibility/visibility, attackers use fake accounts to star and watch malicious repositories.\footnote{\url{https://zd.net/3bg3CK9}} To our knowledge, research conducted to combat this type of abuse %crime %misbehaviour 
%is still in its infancy~\cite{Rokon2020SourceFinderFM}. Thus, there is a need for mechanisms to detect this type of fabrication (\tick). 



%\revised{%\subsection{Detection and countermeasures}
%Depending on the type of the consider RSSE, the literature is plenty of 






%\begin{table*}[t!]
%	\centering
%	\vspace{-.3cm}
%	\footnotesize
%	%	\scriptsize	
%	\caption{Attacks and countermeasures.}
%	\begin{tabular}{| p{8.4cm} |p{8.4cm} |}	\hline
%		\textbf{Attacker} & \textbf{Defender}  \\ \hline
%		%We performed only push attacks in our evaluation, the same methodology can be applied to conduct nuke attacks, \ie expelling a useful API from the recommendations (\untick). Moreover, we tried with only one malicious library, however the evaluation can easily be extended to a set of libraries. 
%		&   \\ \hline
%		In the experiments, various internal settings were considered, and this aims at studying the systems' capability in different working conditions. In practice, an attacker may not be aware of such internal design, what matters is how she populates fake projects so that the malicious library will be recommended (\untick), regardless of the systems' configurations. & \\ \hline
%		To simplify the evaluation, we generated fake projects at the metadata level, \ie we assume that all projects have been successfully fetched from \GH.\footnote{We mined library usage directly from \emph{pom.xml} files.} In practice, it is necessary to plant these projects in \GH to make them appear as legitimate (\untick). &  Aiming for credible sources, a recommender usually chooses to crawl only from repositories with a considerably large number of stars and/or forks, or whatever criterion a recommender uses for selecting its training set (\tick)~\cite{NGUYEN2019110460}. \\ \hline
%		In this case, an attacker may need to disguise a planted project by falsifying this information, \eg by starring and forking with forged accounts (\untick). In fact, such an incident has been recently reported, where hundreds of \GH repositories promoting malware apps have been discovered. Moreover, to increase their credibility/visibility, attackers use fake accounts to star and watch malicious repositories.\footnote{\url{https://zd.net/3bg3CK9}} To our knowledge, research conducted to combat this type of abuse %crime %misbehaviour 
%			is still in its infancy~\cite{Rokon2020SourceFinderFM}. &  Thus, there is a need for mechanisms to detect this type of fabrication (\tick). \\ \hline  		
%	\end{tabular}
%	\vspace{-.2cm}
%	\label{tab:Countermeasures}
%\end{table*}


%============================
%Anomaly detection.
%\emph{What are the possible countermeasures, and how effective are they?} We conduct qualitative analyses to. 
%============================



%\vspace{.2cm}
%\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]
%	\small{\textbf{Summary.} There is the need for decent countermeasures for the attacks described in Section.}
%\end{tcolorbox}

==> src/Evaluation-old.tex <==
%\color{red}


%\color{black}

%The study is conducted on two library recommenders, \ie  \LR~\cite{6671293} and \CR~\cite{NGUYEN2019110460} (see Table~\ref{tab:summary}). 

%======================================
%\MAX{we can skip this paragraph, as the section follows the usual template for an empirical study}
%This section presents the methods and materials used to conduct an investigation into the existence of the research on %as well as implications of 
%adversarial Machine Learning in RSSE, as well as possible implications. Section~\ref{sec:ResearchQuestions} introduces three questions to address the research problems. 
%In Section~\ref{sec:Collection}, we define our strategy to search for papers from premier software engineering venues. We describe in Section \ref{sec:InjectingAPIs} the way in which projects with malicious APIs are populated. The datasets used and experimental settings are introduced in Section~\ref{sec:Settings}. Finally, Section \ref{sec:Metrics} gives a description for the evaluation metric.
%======================================

%To populate fake OSS projects, w
%a preliminary investigation into the implication of AML on two existing RSSE. We consider a scenario in which, developing new software, programmers rely on a recommender system to find and use in their code third-party libraries that offer the desired features. 

 
The \emph{goal} of this study is to investigate the relevance of AML attacks for RSSE, and in particular of API and code snippet recommenders. The \emph{quality focus} is the resilience of RSSE to AML attacks. The \emph{perspective} is of researchers interested to improve the RSSE they develop. The \emph{context} consists of state-of-the-art API and code snippet recommenders.
 

We aim to address the following research questions:


%\subsection{Research questions} \label{sec:ResearchQuestions}

%By means of a series of qualitative and quantitative evaluations, we aim at answering the following research questions:

% [--]
\begin{itemize}
	\item \rqfirst~We perform a literature analysis to investigate whether there is already any effort devoted to study and deal with threats to RSSE originating from malicious data. Although our purpose is not to perform a complete, detailed systematic literature review, we followed consolidated guidelines for this kind of study in software engineering \cite{KitchenhamBLBB11,MacDonellSKM10}.
	%\item \rqsecond~By studying the working mechanism of a set of representative API recommender systems, we analyze their risk of being influenced by hostile attempts.
	\item \rqsecond~First, we perform a qualitative analysis of the likely attack threats that could affect state-of-the-art API and code snippet recommenders. Then, based on their availability, 
	we select three systems for our empirical evaluation, \ie \UM~\cite{Wang2013Mining}, PAM~\cite{Fowkes:2016:PPA:2950290.2950319}, and \FC~\cite{9359479,Nguyen:2019:FRS:3339505.3339636}. These are among the state-of-the-art approaches for API recommendations as they emerge from premier software engineering venues. We conjecture that an evaluation on them will help shed light on the resilience of the majority of existing API recommenders.% systems.
%	\item \rqfourth~We are interested in understanding how the calibration of the systems' internal parameters of affects the attacks' efficiency. This is to find out how severe the possible consequences might be in practice.
%	\item \revised{\rqthird~We attempt to find feasible ways to detect malicious APIs and protect API recommender systems.}
\end{itemize}



\subsection{Literature analysis} \label{sec:Collection}



%\revised{To understand how well the AML in RSSE has been tackled with existing studies, we conduct a compact literature review on premier venues in Software Engineering,	including eight conferences and five journals. For the former, we investigate eight premier venues, among others, there are ICSE, ESEC/FSE, or ASE. Meanwhile, for the latter the following five journals are considered: TSE, TOSEM, EMSE, JSS, and IST. Table~\ref{tab:LiteratureReview} depicts the venues together with the number of papers for each annual edition.  From the \textit{Scopus}\footnote{\url{https://www.scopus.com/}} abstract and citation database, we extract all the papers published at a given edition (year) of a given venue (journal) by Scopus's advanced search and export features.  In the end, we collected 6,402 articles from these venues.	For each paper collected, we extract its title and abstract. First, we define a set of possible words we are interested in. Table \ref{tab:keywords} reports the terms-set we use to search for related papers. We use regular expressions for searching relevant papers (\eg we use or not of the ignore case sensitivity depending on the term we are searching for). In other words}

To achieve a good trade-off between the coverage of existing studies on AML in RSSE and efficiency, we defined the search strategy by answering the following four W-questions~\cite{zhang2011identifying} (``\emph{W}'' stands for Which?, Where?, What?, and When?). %, \ie Which?, Where?, What?, and When?~\cite{zhang2011identifying} as follows

%\revised{\textbf{Which:} \textbf{What:}  \textbf{Where:}   }
%\vspace{-.4cm}
%
%\begin{table}[t!]
%	\centering
%	\vspace{-.3cm}
%	\scriptsize	
%%	\footnotesize
%	\caption{Venues considered in the literature analysis.} %and their acronyms
%	\begin{tabular}{| p{0.2cm}|l | p{6cm} |}	\hline
%		& \textbf{Acronym} & \textbf{Name}  \\ \hline		
%		{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Conferences}}}} & ICSE & The IEEE/ACM International Conference on Software Engineering \\ \cline{2-3}
%		& ESEC/FSE & The ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering \\ \cline{2-3}
%		& ASE & The IEEE/ACM International Conference on Automated Software Engineering \\ \cline{2-3}
%		& ICSME & The International Conference on Software Maintenance and Evolution \\ \cline{2-3}
%		& ICST & The IEEE International Conference on Software Testing, Verification and Validation \\ \cline{2-3}
%		& ISSTA & The ACM SIGSOFT International Symposium on Software Testing and Analysis \\ \cline{2-3}
%		& ESEM & The ACM/IEEE International Symposium on Empirical Software Engineering and Measurement \\ \cline{2-3}
%		& MSR & The IEEE International Working Conference on Mining Software Repositories \\ \cline{2-3}
%		& SANER & The IEEE International Conference on Software Analysis, Evolution and Reengineering \\ \hline		
%		%		MSR & International Conference on Mining Software Repositories \\ \hline
%		{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Journals}}}} &	TSE & IEEE Transactions on Software Engineering \\ \cline{2-3}
%		& TOSEM & ACM Transactions on Software Engineering and Methodology \\ \cline{2-3}
%		& EMSE & Springer Empirical Software Engineering Journal \\ \cline{2-3}
%		& JSS & Elsevier Journal of Systems and Software \\ \cline{2-3}
%		& IST & Elsevier Information and Software Technology \\ \hline				
%	\end{tabular}
%	\vspace{-.2cm}
%	\label{tab:acronyms}
%\end{table}



%\color{blue}
\begin{itemize}
	\item \emph{Which?} Both automatic and manual searches were performed to look for relevant papers from conferences and journals.
	\item \emph{Where?} We conducted a literature analysis on premier venues in software engineering. 
	In particular, there are nine conferences as follows: ICSE, ESEC/FSE, ASE, ICSME, ICST, ISSTA, ESEM, MSR, and SANER. 
	Meanwhile, the following five journals were considered: TSE, TOSEM, EMSE, JSS, and IST.\footnote{We report the full name of all the venues as well as their corresponding acronyms in an online appendix \url{https://bit.ly/3vbAHhm}.} %\MAX{if space allows we expand names otherwise here we should refer to the appendix with the venue names}
	The selection of conferences and journals was performed so as to include mainstream venues, as well as specialized ones for which RSSE are relevant.
	The automatic search was done on the \textit{SCOPUS} database.\footnote{\url{https://www.scopus.com/}} We fetched all the papers published by a given edition (year) of a given venue (journal/conference) using the advanced search and export features.
	\item \emph{What?} For each paper collected, its title and abstract were extracted using a set of predefined keywords. %we are interested in. Table \ref{tab:keywords} reports the terms-set we 
	%	used to search for related papers. 
	To cover more possible results, we used regular expressions for searching, \eg depending on the terms we may use case sensitive queries. %, so as.
	%	\item \emph{Where?} We conduct a compact literature review on premier venues in Software Engineering, including eight conferences and five journals. For the former, we investigate eight premier venues, among others, there are ICSE, ESEC/FSE, or ASE. Meanwhile, for the latter the following five journals are considered: TSE, TOSEM, EMSE, JSS, and IST.
	\item \emph{When?} Since Adversarial Machine Learning is a recent research topic, we limit the search to the most five recent years, \ie from 2016 to 2020. %This also aims to limit.
\end{itemize}

The extraction process produced a corpus of \numPapers 
articles. 
Then, we performed various filtering steps to narrow down the search and look for those that meet our requirements. In particular, we are interested in studies 
dealing with recommender systems together with the relevant topics, \ie Adversarial Machine Learning, API mining, and malicious attempts.
Intermediate results, \eg number of downloaded papers per venue, number of candidate papers per venue, are available in our online appendix \cite{repo}. %\MAX{I added the sentence before, check if it makes sense}






%narrow down the search to. %The final results are goi

%	In the end, we collected 
%Our search strategy consists of an automatic search on Electronic Data Sources (EDS). We performed search on Electronic Data Sources (EDS). 

%\item \emph{Where?} We conduct a compact literature review on premier venues in Software Engineering, including eight conferences and five journals. For the former, we investigate eight premier venues, among others, there are ICSE, ESEC/FSE, or ASE. Meanwhile, for the latter the following five journals are considered: TSE, TOSEM, EMSE, JSS, and IST.

%from these venues.


%Our search strategy consists of an automatic search on Electronic Data Sources (EDS). 
%	We performed search on Electronic Data Sources (EDS). In particular, from the \textit{SCOPUS}\footnote{\url{https://www.scopus.com/}} abstract and citation database, we extracted all the papers published by a given edition (year) of a given venue (journal/conference) using the advanced search and export features. The extraction process culminated in a corpus of 
%	In the end, we collected 
%	6,402 articles. %from these venues.

%\color{black}
%\JDR{Summarizing mSLR papers}




%\revised{%\subsection{Attack detection and countermeasures}
%Depending on the type of the consider RSSE, the literature is plenty of possible strategies to neutralize or reduce the negative effects of an adversarial attack. Mobasher \etal \cite{mobasher_attacks_2007} employ two different techniques to detect malicious attacks that involve recommended items \ie profile classification and anomaly detection. The former employs a classifier that makes use of attribute-reduction techniques to create a lower-dimensional training set. The underpinning model analyzes generic profile attributes as well as intra-profile and model-specific ones. The conducted evaluation shows that the proposed model can properly classify malicious users considering a well-defined set of metrics. Concerning anomaly detection problem, the work makes use of statistical process control (SPC) strategy to identify suspicious items trends. To this end, the model examines the items considering two parameters \ie the density of the distribution and the average ratings. The results demonstrate that detecting push attacks for popular items is more difficult while the SPC model correctly identifies attacks against low-density items. A recent work \cite{si_shilling_2020} highlights other possible countermeasures. Similar to supervised techniques, semi-supervised and unsupervised approaches have been developed with the aim of detecting attacks coming from pretended profiles. An alternative strategy could be the development of a robust recommendation algorithm that avoids possible attacks in advance. Several approaches employ matrix factorization or kernel distance even though trust-aware recommender systems are more robust than traditional ones \cite{DBLP:journals/corr/abs-1207-4525, 5428690}.
%Concerning shilling that exploits hubness, Hara \etal \cite{10.1145/2766462.2767823} propose an approach to increase the robustness of memory-based recommender system. To this end, the similarity measure exploited by the K-NN algorithm is transformed to reduce the bias that causes hubness. }


% and to deceive developers
%ai.grakn:grakn-engine:2016-11-22
%To this end, w %that appear to be similar to the target ones. We exploit a 

%<<<<<<< HEAD
%When \LR and \CR learn from existing projects and when they provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}. This resembles ratings of a user profile in online shopping systems.
%%We craft a set of forged projects exploiting a well-known technique to populate their ratings~\cite{4216981}. By the original approach~\cite{BWMB06}, a profile is divided into four independent parts, \ie \emph{unrated}, \emph{filler}, \emph{selected}, and \emph{target}. 
%To attack a recommender system, there are various approaches to populate fake user profiles~\cite{BWMB06,4216981}. Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). \MAX{this part is unclear, I think those are 2 separate problems. I think here we can only say how we create a training set for the tools, then we have to explain that a project would fall in the training set if it has good ratings, and there are ways to fake the ratings, but we did not simulate this here to avoid violating github terms of service}
%Thus, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (see Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%=======






%together with the related calls, 
%to make it more convincing, and
%in a legitimate snippet 
%make their attempt more practical by 
%The second scenario is when the developer is provided with intentionally harmful APIs embedded in a fake third-party library. In this case, 

%We simulate an attacker attempting to inject a library with malicious code (\eg by referring to the previous example, a malicious JSON parser), let it be $lib^{*}$, into the active projects. 
%For instance, the developer is searching for libraries for parsing JSON documents and the system should be able to suggest those that are used by similar projects. 

%In practice, to avoid being detected, an attacker probably gives the library a copycat name, \ie one that closely resembles a popular library, aiming to disguise it better. For instance, a malicious library has been named as ``\emph{jeIlyfish}'' to deceive developers into believing it ``\emph{jellyfish},'' the authentic library.\footnote{\url{https://bit.ly/394uETI}} In this way, developers would adopt the disguised library without hesitation, once it has been suggested by the recommendation engine.

%In fact, typosquatting has been reported in recent work~\cite{10.1145/3196398.3196401}, and this indeed suggests an evident threat to the adoption of third-party libraries. 
%\ie a set of APIs, 



%\color{red}




%\revised{In practice, to avoid being detected, an attacker normally names $lib^{*}$ using a copycat name, aiming to disguise it. For instance, .}

%================================================
%When \LR and \CR learn from existing projects to %and when they 
%provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}.
%To attack a recommender system, there are various approaches to populate ratings for fake user profiles~\cite{BWMB06,4216981}. 
%Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). 
%Thus, to create a training set for the \LR and \CR tools, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (see 
%Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%================================================

%We come across the following question: ``\emph{Which libraries should be chosen as fillers, so that the fake project will be incorporated into the recommendation?}'' In fact, recommenders heavily rely on similarity~\cite{Schafer:2007:CFR:1768197.1768208}, thus we come up with the selection of popular libraries as fillers. Our intuition  is that, a fake project with libraries widely used by other projects is likely to get attention from the recommendation engine. A list of libraries in the training projects is populated and sorted in descending order of the number of caller projects. A certain number of the most popular libraries is then randomly selected.

\color{black}

%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\Omega$ is the number of fillers. For \LR and \CR, \emph{k} is the number of similar projects and \emph{N} is the cut-off value for the ranked list of recommendations~\cite{6671293,NGUYEN2019110460}. We conducted experiments using ten-fold cross-validation on a dataset crawled from \GH consisting of 1,400 projects and 13,497 libraries. For a testing project, we randomly split its libraries into two equal parts, the first part is used as a query, while the second one is ground-truth data. To measure the effectiveness of the push attacks, we use \emph{Hit ratio} \emph{HR@N}, 
%defined as the ratio of projects being recommended with $lib^{*}$ to the total number of testing projects~\cite{10.1007/978-3-030-49461-2_18}. 
%To measure the accuracy, we use success rate \emph{SR@N}, \ie the ratio of projects getting at least a matched library (the size of the intersection of the recommended list with the ground-truth data is larger than 0) to the number of testing projects.
%We experimented with $\alpha$=$\{5\%,10\%\}$ as attack size; 
%$k$=$\{5,10,15,20\}$; $\Omega$=$\{3,4,6,8,10\}$ as fillers' size. The calibration of these parameters allows us to simulate \emph{stress tests}, aiming to investigate the systems' safeness under different working conditions. 


%\begin{figure}[t!]
%	\centering
%	\vspace{-.3cm}
%	\includegraphics[width=0.68\linewidth]{figs/FakeProject.pdf}
%	\vspace{-.3cm}
%	\caption{Manipulation of library usages for a fake project.}
%	\label{fig:FakeProject}
%	%	\vspace{-.3cm}
%\end{figure}




\subsection{Performing push attacks to API and code snippet RSSE} \label{sec:InjectingAPIs}

As mentioned in Section~\ref{sec:Example}, though the code in Listing~\ref{lst:ExampleSnippet} is dangerous, it is unlikely that developers encounter something similar  under normal circumstances. 
Therefore, to expose the code to recommenders, attackers need to manipulate the training data by performing a \emph{push attack} (see Section~\ref{sec:Attacks}). In such a misdeed, they forcefully favor the targeted items by boosting their popularity. This will increase the possibility of being discovered and thus, recommended by search engines.

%==============================================
%Referring back to the example in Listing~\ref{lst:ExampleSnippet}, attackers need to promote the following pattern: 
%\texttt{\hl{\small Socket\; socket\; =\; ...}} (Line~\ref{line:socket}), \texttt{\hl{\small OutputStream\; out\; =\; ...}} (Line~\ref{line:out}), and \texttt{\hl{\small out.write()}} (Line~\ref{line:code}). %, and then upload them to OSS platforms. 
%In case of a fake library, attackers may enclose all malicious code in a single API call (see Section~\ref{sec:Example}). As a result, there is the need to favor a handful of APIs instead of some, making attacks more feasible. Moreover, to avoid being detected, they might disguise the code with a typosquatting name, \ie one that closely resembles a popular API. In this case, developers would adopt the disguised API without the least delay, once it is suggested by the recommendation engine.
%==============================================

 We encounter the following challenge: ``\emph{How should a fake API be planted, so that it will be incorporated by recommendation engines?}'' In fact, recommender systems rely heavily on similarity measures, \ie they employ algorithms to search for similar artifacts, which are used to deduce recommendations. This is the case not only for general-purpose recommender systems~\cite{Ricci2011}, but also for several RSSE~\cite{DBLP:conf/sigsoft/HolmesWM05,10.1145/1167473.1167508,Moreno:2015:IUT:2818754.2818860,Nguyen:2019:FRS:3339505.3339636,Zhong2009MAPO,Wang2013Mining}. For instance, library recommenders search for libraries from the most similar projects in the training data~\cite{NGUYEN2019110460,6671293}. Similarly, various systems for providing APIs and code also exploit a similarity measure~\cite{Fowkes:2016:PPA:2950290.2950319,9359479}, or a kernel~\cite{DBLP:conf/kbse/Gu0019} to retrieve similar projects and snippets. More importantly, to produce recommendations, RSSE need to rely on 
OSS forges, such as \GH, or Maven, which are subject to changes from the public. 



\begin{figure}[t]
	\centering
	\vspace{-.1cm}
	\includegraphics[width=0.86\linewidth]{figs/PushAttacks.pdf}
	\vspace{-.2cm}
	\caption{Manipulating \GH repositories.} %Performing push attacks
	\vspace{-.2cm}
	\label{fig:PushAttacks}
\end{figure}

Let us imagine a scenario in which one increases the popularity of malicious APIs\footnote{As stated in Section~\ref{sec:Example}, we consider an API malicious if it causes fatal errors, no matter where it comes from, \ie either a legitimate or a fake library.} by planting them to OSS projects, as many as possible. Fig.~\ref{fig:PushAttacks} illustrates the process in which attackers may exploit to plant malicious data. First, well-maintained repositories are forked from \GH, \eg those that have good indicators in terms of stars, forks, or watchers. Afterwards, the projects are injected with fake APIs, and then uploaded again to \GH. In fact, malicious repositories in \GH are not scarce, but \emph{dime a dozen}~\cite{Rokon2020SourceFinderFM}. To boost up the popularity of an API pattern, the APIs can be seeded into a significant number of declarations, for each training project. Attackers may create fake accounts to star, fork, and watch malicious repositories to increase their credibility/visibility, thus exposing them better to search engines.\footnote{Such a manipulation has been recently revealed \url{https://zd.net/3bg3CK9}.}

To this respect, there are the following parameters to consider, when it comes to populating artificial projects. 

%We illustrate in 
%Attackers may disguise the planted projects by starring and forking them with forged accounts. 
%making it more convincing, 
%=======================
%Such a trick has been recently revealed, where several \GH repositories hosting malware apps have been found~\cite{Rokon2020SourceFinderFM}.\footnote{\url{https://zd.net/3bg3CK9}} To our knowledge, research conducted to combat this type of abuse %crime %misbehaviour 
%is still in its initial phase~\cite{10.1145/3357384.3357971}. %,Rokon2020SourceFinderFM
%=======================
%Avoiding detection, 
%Since a project may consist of several declarations (see Section~\ref{sec:Definitions})
%To boost up the popularity of an API pattern, it is necessary to seed the APIs to not only one but more projects. 

\begin{itemize}
	\item $\alpha$ is the ratio of projects injected with fake APIs.% (\%).	
	\item $\beta$ is the ratio of methods in a project getting fake APIs.% (\%).
	\item $\Omega$ is the number of fake APIs injected to each declaration.
	\item \emph{N} is cut-off value for the ranked list of recommended items returned by a recommender system.
\end{itemize}

%It is worth noting that these parameters are under control of attackers, \ie they can be fined tune to make attacks more effective.
%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\Omega$ is the number of fillers. 
%In the evaluation, we experiment with different configurations by varying the parameters to analyze which settings bring more perturbed outcomes.

We experiment with the following sets of parameters: $\alpha$=$\{5\%,\-10\%,15\%,20\%\}$, $\beta$=$\{40\%,50\%,60\%\}$, $\Omega$=$\{1,2\}$. The rationale behind the selection of these values is as follows. Concerning $\alpha$, though having popular APIs is commonplace, 
it is difficult to rack up projects with malicious APIs, thus $\alpha$ is set to the following thresholds $\alpha$=$\{5\%,\-10\%,15\%,20\%\}$. In contrast, within a project, attackers have more freedom to embed APIs to declarations, therefore $\beta$ is varied from 40\%, 50\%, to 60\%. Finally, as explained in Section~\ref{sec:Example}, the number of fake APIs should be kept low to make attacks more feasible,  
\ie $\Omega$=$\{1,2\}$. We study how the calibration of the parameters affects the final efficiency, aiming to anticipate the extent to which the attacks are successful in the field. 








\subsection{Data extraction and curation} \label{sec:Settings} % and experimental settings

%Both \LR and \CR suggest to active projects, \ie the ones under development, by searching for libraries from the most similar projects in the training data~\cite{NGUYEN2019110460}. For instance, the developer is searching for libraries for parsing JSON documents and the system should be able 
%to suggest those that are used by similar projects. 
%We simulate an attacker attempting 
%to inject a library with malicious code (\eg by referring to the previous example, a malicious JSON parser), let it be $lib^{*}$, into the active projects. \revised{In practice, to avoid being detected, an attacker normally names $lib^{*}$ using a copycat name, aiming to disguise it. For instance, .}
%Given that under the normal circumstances, the systems would never recommend $lib^{*}$ since the library has not been invoked anywhere.
%To this end, we forcefully favor $lib^{*}$ using 
%push attacks (see Section~\ref{sec:Classification}), so that, in the end,
%the library will be suggested to projects.
%
%% and to deceive developers
%%ai.grakn:grakn-engine:2016-11-22
%%To this end, w %that appear to be similar to the target ones. We exploit a 
%
%%<<<<<<< HEAD
%%When \LR and \CR learn from existing projects and when they provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}. This resembles ratings of a user profile in online shopping systems.
%%%We craft a set of forged projects exploiting a well-known technique to populate their ratings~\cite{4216981}. By the original approach~\cite{BWMB06}, a profile is divided into four independent parts, \ie \emph{unrated}, \emph{filler}, \emph{selected}, and \emph{target}. 
%%To attack a recommender system, there are various approaches to populate fake user profiles~\cite{BWMB06,4216981}. Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). \MAX{this part is unclear, I think those are 2 separate problems. I think here we can only say how we create a training set for the tools, then we have to explain that a project would fall in the training set if it has good ratings, and there are ways to fake the ratings, but we did not simulate this here to avoid violating github terms of service}
%%Thus, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (see Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%%=======
%When \LR and \CR learn from existing projects to %and when they 
%provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}.
%To attack a recommender system, there are various approaches to populate ratings for fake user profiles~\cite{BWMB06,4216981}. 
%Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). 
%Thus, to create a training set for the \LR and \CR tools, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (see 
%Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%
%
%We come across the following question: 
%``\emph{Which libraries should be chosen as fillers, so that the fake project will be incorporated into the recommendation?}'' In fact, recommenders heavily rely on similarity~\cite{Schafer:2007:CFR:1768197.1768208}, thus we come up with the selection of popular libraries as fillers. Our intuition 
%is that, a fake project with libraries widely used by other projects is likely to get attention from the recommendation engine. 
%A list of libraries in the training projects is populated and sorted in descending order of the number of caller projects. A certain number of the most popular libraries is then randomly selected.
%
%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\Omega$ is the number of fillers. For \LR and \CR, \emph{k} is the number of similar projects and \emph{N} is the cut-off value for the ranked list of recommendations~\cite{6671293,NGUYEN2019110460}. We conducted experiments using ten-fold cross-validation on a dataset crawled from \GH consisting of 1,400 projects and 13,497 libraries. For a testing project, we randomly split its libraries into two equal parts, the first part is used as a query, while the second one is ground-truth data. To measure the effectiveness of the push attacks, we use \emph{Hit ratio} \emph{HR@N}, 
%defined as the ratio of projects being recommended with $lib^{*}$ to the total number of testing projects~\cite{10.1007/978-3-030-49461-2_18}. 
%To measure the accuracy, we use success rate \emph{SR@N}, \ie the ratio of projects getting at least a matched library (the size of the intersection of the recommended list with the ground-truth data is larger than 0) to the number of testing projects.
%We experimented with $\alpha$=$\{5\%,10\%\}$ as attack size; 
%$k$=$\{5,10,15,20\}$; $\Omega$=$\{3,4,6,8,10\}$ as fillers' size. The calibration of these parameters allows us to simulate \emph{stress tests}, aiming to investigate the systems' safeness under different working conditions. 
%
%
%\begin{figure}[t!]
%	\centering
%	\vspace{-.3cm}
%	\includegraphics[width=0.68\linewidth]{figs/FakeProject.pdf}
%	\vspace{-.3cm}
%	\caption{Manipulation of library usages for a fake project.}
%	\label{fig:FakeProject}
%	\vspace{-.3cm}
%\end{figure}



%The following research questions are addressed to study the performance: \emph{(i)} ``\rqfirst'' and \emph{(ii)} ``\rqsecond''.

%employed a curated dataset composed of 3,000 Android projects crawled from the Apkpure platform\footnote{\url{https://apkpure.com/it/}} employed by an existing work \cite{9359479}. 

To address RQ$_2$, we looked at the same venues considered in RQ$_1$ to identify, over the period 2010-2020, API recommender systems as well as RSSE suggesting API code example snippets. We then qualitatively discuss, for each recommender,   the working mechanism and its potential risks. 



%From the papers in \textbf{RQ$_1$} that match with two sets of keywords, \ie REC and API, we carefully read and selected 
%RSSE that support the development of software projects by delivering API calls and/or snippets. We also searched earlier venues for additional tools being considered to be among the first and thus, the most influential API recommender systems. Eventually, we included two more tools, namely 
%Strathcona \cite{DBLP:conf/sigsoft/HolmesWM05}, 
%XSnippet~\cite{10.1145/1167473.1167508}, 
%MAPO~\cite{Zhong2009MAPO}, 
%\UM~\cite{Wang2013Mining} and MUSE~\cite{Moreno:2015:IUT:2818754.2818860}. Table~\ref{tab:summary} lists in chronological order, and analyzes the set consisting of 9 API/snippet RSSE.

Then, based on the tool availability as well as the characteristics of the tools, we select three of them,  \ie \UM~\cite{Wang2013Mining}, PAM~\cite{Fowkes:2016:PPA:2950290.2950319}, and \FC~\cite{Nguyen:2019:FRS:3339505.3339636}.
To evaluate the resilience of \UM, PAM, and \FC, we use a dataset containing Android apps' source code. We focused on Android apps because they entail a typical scenario in which an infection can cause unwanted consequences such as data leaks.
%Such a dataset has been chosen due to the following reasons: \emph{(i)} Android programming is becoming more popular, and developers are increasingly using recommender systems to assist their daily tasks~\cite{10.1145/3183440.3195011}; and \emph{(ii)} the adoption of intentionally manipulated APIs provided by recommender systems will infect apps with malicious code, causing probably disastrous consequences for mobile users. 

%\begin{figure}[h!]
%	\centering
%	\vspace{-.2cm}
%	\includegraphics[width=\linewidth]{figs/DataExtraction2.pdf}
%	\vspace{-.3cm}
%	\caption{Collecting data from \GH and Google Play.}
%	\vspace{-.2cm}
%	\label{fig:DataExtraction}
%\end{figure}

%Since the systems considered in \textbf{RQ$_3$}, \ie \UM~\cite{Wang2013Mining}, PAM \cite{Fowkes:2016:PPA:2950290.2950319}, and \FC~\cite{Nguyen:2019:FRS:3339505.3339636} cannot work directly on raw data collected from \GH, it is necessary to perform preprocessing steps to convert the input data into a processable format. 

To mine data for the experiments, we made use of a process conceived in a recent work~\cite{9359479}. %, depicted in Fig.~\ref{fig:DataExtraction}. 
First, we searched for open source projects using the \emph{AndroidTimeMachine} platform~\cite{8595172}, which retrieves apps and their source code from Google Play\footnote{\url{https://play.google.com/}} and \GH. Second, APK files are fetched from the Apkpure platform,\footnote{\url{https://apkpure.com/}} using a Python script. 
Third, the \emph{dex2jar} tool \cite{dex2jar} is used to convert the APK files into the JAR format. The JAR files were then fed as input for Rascal to convert them into the M$^3$ format~\cite{Basten2015M3}. We obtained a set of \numApps apps with full source code. To simplify the evaluation, %using the \textsc{API Seeder} component 
we inject APIs at the metadata level, \ie after the data that has been parsed to a processable format. This is for experimental purposes only, since in reality we need to seed data directly to projects and upload them to \GH\footnote{This requires extra effort, which is not the focus of this paper, thus we consider this our future work.} as shown in Fig.~\ref{fig:PushAttacks}.

We then inserted fake APIs to random projects and declarations, attempting to simulate real-world scenarios where APIs are dispersed across several declarations. Finally, the resulting data is parsed in two formats, \ie ARFF files to be fed to \UM and PAM, and a special file format for providing input to \FC. By an empirical evaluation, we realized that \UM and PAM suffer from scalability issues, \ie they cannot work on large datasets. Thus for evaluating them, we could only consider a subset consisting of 500 apps. For \FC, the whole \numApps apps are used since the system is capable of handling well a large amount of data.


%, after all the projects have been obtained from OSS platforms
%Since the examined tools take as input ARFF file format, we extracted such a format starting from the decompiled version of each project. 


%The process culminated in the final corpus consisting of 2,600 APK binary files (mined from Apkpure) together with additional metadata (mined from Google Play), including authors, categories, star rating, price, and the number of downloads. By carefully inspecting the data, we realized that most of the apps are highly rated and they have a high number of downloads. 
%As Rascal can parse certain programming languages, from the initial dataset we filtered out irrelevant projects to select only the Java and Kotlin ones, which account for the majority of the apps. % \MAX{does this depend on the analysis capability? clarify.
%Afterwards, we 
%Figure~\ref{fig:StarsAndDownloads} depicts a map of the apps with respect to the number of stars and downloads. As can be seen, the apps are scattered across the map: there are apps that locate on the lower part of the figure, indicating a low rating as well as a low number of downloads. 
%locate on the upper part of the figure
%We consider a larger dataset rather than the two original ones to examine carefully the potentially disruptive effect of malicious attacks. Moreover, we are capable of experimenting with different adversarial settings to investigate to what extend the robustness is compromised.
%\FC is dependent on Rascal M$^3$~\cite{Basten2015M3} to function. Rascal M$^3$ is an intermediate model that performs static analysis on source code to extract method declarations and invocations from a set of projects. This model is an extensible and composable algebraic data type that captures both language-agnostic and Java-specific facts in immutable binary relations. These relations represent program information such as existing \textit{declarations}, \textit{method invocations}, \textit{field accesses}, \textit{interface implementations}, \textit{class extensions}, among others~\cite{Basten2015M3}. To gather relevant data, Rascal M$^3$ leverages the Eclipse JDT Core Component\footnote{\url{https://www.eclipse.org/jdt/core/}} to build and traverse the abstract syntax trees of the target Java projects.

%The x-Axis represents the number of declarations that have the number of of invocations in the y-Axis. 


We inspected the dataset and counted 26,852 unique APIs in all the apps. Fig.~\ref{fig:NumOfDeclarations} depicts the distribution of APIs in projects and declarations. The x-Axis and the y-Axis specify the number of projects and the number of declarations in which an invocation is seen, respectively. The dense cluster of points on the lower left corner suggests that most of the APIs appear in less than 250 projects and 200 declarations. Meanwhile, a small fraction of them are invoked by a large number of projects and declarations, \ie more than 2,000 and 10,000, respectively. Such a distribution has an impact on the $\alpha$ and $\beta$ parameters as we mentioned in Section~\ref{sec:InjectingAPIs}. 

\begin{figure}[t]
	\centering
	\vspace{-.2cm}
	\includegraphics[width=0.680\linewidth]{figs/ProjectDeclarations3.png}
	\vspace{-.1cm}
	\caption{Frequency of APIs in projects and declarations.} %Summary of the main words
	\vspace{-.2cm}
	\label{fig:NumOfDeclarations}
\end{figure}

%relationship between projects and declarations. 


%The top ten most popular APIs are shown in Table~\ref{tab:TopTenInvocations}, whose the second column specifies the frequency of appearance of an API in all the projects. Overall, the table


The figure indicates that some APIs are extremely frequent. By looking inside the dataset, we see that \texttt{\hl{\small java/lang/String\-Builder/append(java.l\-ang.String)}} is the most popular API as it appears in 96.61\% of the projects. Other invocations specific to Android apps, such as \texttt{\hl{\small android/view/View/get\-Right()}}, are also very common in the dataset. The presence of very popular APIs gives us some hints on how to inject malicious APIs having the same names. We conjecture that, even if we embed an artificial API to a large number of projects, this can be seen as normal and thus, does not arouse developers' suspicion. 

%It is evident that all of them are very popular. 
%catch developers' attention.%normal and thus. %, and thus. %does not cause any.
%imperceptible
% impacts on the way we plant fake APIs. 
%We call \textbf{F$_p$} and \textbf{F$_d$}

%\begin{table}[h!]
%%	\vspace{-.2cm}
%%	\footnotesize
%	\scriptsize
%	\caption{Top ten most frequent APIs.}
%	\vspace{-.2cm}
%	\begin{tabular}{|p{6.8cm}|l|} \hline
%		\textbf{API} & \textbf{Freq. (\%)}  \\ \hline
%		java/lang/StringBuilder/append(java.lang.String) & 96.61  \\ \hline
%		java/lang/IllegalStateException/IllegalStateException(java.lang.String)	 & 89.70 \\ \hline
%		android/util/Log/w(java.lang.String,java.lang.String) & 88.30 \\ \hline
%		java/util/Iterator/hasNext() & 86.92  \\ \hline
% 		android/view/View/getRight() & 86.00   \\ \hline
%		android/view/View/getLayoutParams()	 & 85.96 \\ \hline
% 		java/util/Map/put(java.lang.Object,java.lang.Object) & 78.30 \\ \hline 		 	 
% 		java/util/ArrayList/ArrayList() & 77.15 \\ \hline
% 		java/lang/Integer/intValue() & 75.88 \\ \hline
% 		java/lang/String/valueOf(java.lang.Object) 	 & 49.88 \\ \hline
%	\end{tabular}
%	\label{tab:TopTenInvocations}
%	\vspace{-.2cm}
%\end{table}




%\begin{table}[h!]
%	\vspace{-.2cm}
%	\footnotesize
%	\caption{Top ten most frequent APIs.}
%	\vspace{-.2cm}
%	\begin{tabular}{|l|p{6.8cm}|l|} \hline
%		\textbf{API} & \textbf{F$_p$} & \textbf{F$_d$} \\ \hline
%		\texttt{\footnotesize java/lang/StringBuilder/append(java.lang.String)}	 & &  \\ \hline
%		\texttt{\footnotesize java/util/Iterator/hasNext()} & & \\ \hline
%		\texttt{\footnotesize android/view/View/getLayoutParams()}	 &  & \\ \hline
%		\texttt{\footnotesize android/util/Log/w(java.lang.String,java.lang.String)} &  & \\ \hline
%		\texttt{\footnotesize java/lang/Illegal\-StateException/Illegal\-StateException(java.lang.String)}	 &  & \\ \hline
%		\texttt{\footnotesize android/view/View/getRight()} &  & \\ \hline
%		\texttt{\footnotesize java/util/ArrayList/ArrayList()} &  & \\ \hline
%		\texttt{\footnotesize java/util/Map/put(java.lang.Object,java.lang.Object)} & &  \\ \hline 		 	 
%		\texttt{\footnotesize java/lang/String/valueOf(java.lang.Object)} 	 &  & \\ \hline
%		\texttt{\footnotesize java/lang/Integer/intValue()} &  & \\ \hline
%	\end{tabular}
%	\label{tab:TopTenInvocations}
%	\vspace{-.2cm}
%\end{table}





%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\Omega$ is the number of fillers. 
%For \LR and \CR, \emph{k} is the number of similar projects and \emph{N} is the cut-off value for the ranked list of recommendations~\cite{6671293,NGUYEN2019110460}. 


%To measure the effectiveness of the push attacks, we use \emph{Hit ratio} \emph{HR@N}, 
%defined as the ratio of projects being recommended with $lib^{*}$ to the total number of testing projects~\cite{10.1007/978-3-030-49461-2_18}. 

%\color{red}
%To measure the accuracy, we use success rate \emph{SR@N}, \ie the ratio of projects getting at least a matched library (the size of the intersection of the recommended list with the ground-truth data is larger than 0) to the number of testing projects. We experimented with $\alpha$=$\{5\%,10\%\}$ as attack size; $k$=$\{5,10,15,20\}$; $\Omega$=$\{3,4,6,8,10\}$ as fillers' size. The calibration of these parameters allows us to simulate \emph{stress tests}, aiming to investigate the systems' safeness under different working conditions. 
%\color{black}





%\subsection{Injecting APIs} \label{sec:InjectingAPIs}

%\revised{\subsection{Populating fake projects}}
%both scenarios appear to be unrealistic since 
%Given that under the normal circumstances, the systems would never recommend $lib^{*}$ since the library has not been invoked anywhere. To this end, we forcefully favor $lib^{*}$ using push attacks (see Section~\ref{sec:Classification}), so that, in the end, the library will be suggested to projects.
%of encountering such a snippet 

%For each declaration, we extract its method name, a list of types of the parameters, and a list of API function calls. In this way, a project is represented as a set of declarations from its constituent classes.

%The second scenario is when the developer is provided with intentionally harmful APIs embedded in a fake library. In this case, attackers may make their attempt more practical by wrapping all malicious code in a single API, and disguise it in a legitimate snippet.
%We insert malicious APIs
%In other words, when using recommender systems the developer would hardly encounter the snippet. 






\subsection{Settings and metric} \label{sec:Metrics}

%To this end, the hit ratio metric HR@N is defined as follows. 
% on a dataset crawled from \GH consisting of 3,200 Android apps. 
%For a testing project, we randomly split its libraries into two equal parts, the first part is used as a query, while the second one is ground-truth data.

We conducted experiments using the ten-fold cross-validation meth\-odology, \ie the dataset with $\left| P \right|$  projects is divided into ten equal parts, and each experiment is done in ten times. For each round of execution, one part is used for testing, while the other nine remaining parts are fed as training.% data. 

To measure the effectiveness of push attacks, we employ \emph{Hit ratio} \emph{HR@N}~\cite{10.1007/978-3-030-49461-2_18,mobasher_attacks_2007}, which is defined as the ratio of projects being provided with a fake API $\left| T \right|$ to the total number of testing projects $\left| P \right|$, \ie $HR@N = \left| T \right| / \left| P \right|$, with N as the cut-off value for the ranked list. The metric is computed over the results of all the ten folds. %\MAX{summing or computing the hit ratio over the results of all ten folds? Otherwise it will no longer be a ratio}



%
%\begin{equation}
%HR@N = \frac{ \emph{API*@N}}{\left| P \right|}
%\end{equation}
%where $T$ is the number of projects recommended with the fake APIs with N as the cut-off value for the ranked list, and $\left| P \right|$ is the total number of projects. 

%We use a set of 1,200 projects collected from \GH. To fill the ratings, 
%there is a set of parameters that need to be considered, and let us call them \emph{internal parameters}.
%There are the following parameters to consider:
%\begin{itemize}
%	\item Attack size is defined as the ratio of fake projects to the total number of training projects $\alpha$; 
%	\item The number of libraries for a fake projects;
%	\item The number of most popular libraries considered for generating.
%\end{itemize}
%\begin{table}[h]
%	\centering
%	\vspace{-.3cm}
%	\scriptsize
%	\caption{Parameters.}
%	\begin{tabular}{|p{0.5cm} | p{3.1cm} | p{0.5cm} | p{3.1cm} |} \hline
%		\multicolumn{2}{|c|}{\textbf{External parameters}} & \multicolumn{2}{c|}{\textbf{Internal parameters}} \\  \hline
%		\textbf{Name} & \textbf{Description} & \textbf{Name} & \textbf{Description}  \\ \hline
%		$\alpha$ & Attack size  & k & Number of neighbour projects \\ \hline
%		$\beta$ & Number of most popular libraries  & N & Cut-off value \\ \hline
%		$\lambda$ & Number of filler libraries  &  &  \\ \hline
%	\end{tabular}
%	%	\vspace{-.4cm}
%	\label{tab:parameters}
%\end{table}


%\subsection{Metrics}

%To measure the effectiveness of the push attack, we use
%\emph{Prediction shift} and 
%Moreover, we also measure \emph{accuracy}.
%The experiment results are shown in 



==> src/Evaluation2.tex <==
%\color{red}


%\color{black}

%The study is conducted on two library recommenders, \ie  \LR~\cite{6671293} and \CR~\cite{NGUYEN2019110460} (see Table~\ref{tab:summary}). 

%======================================
%\MAX{we can skip this paragraph, as the section follows the usual template for an empirical study}
%This section presents the methods and materials used to conduct an investigation into the existence of the research on %as well as implications of 
%adversarial Machine Learning in RSSE, as well as possible implications. Section~\ref{sec:ResearchQuestions} introduces three questions to address the research problems. 
%In Section~\ref{sec:Collection}, we define our strategy to search for papers from premier software engineering venues. We describe in Section \ref{sec:InjectingAPIs} the way in which projects with malicious APIs are populated. The datasets used and experimental settings are introduced in Section~\ref{sec:Settings}. Finally, Section \ref{sec:Metrics} gives a description for the evaluation metric.
%======================================

%To populate fake OSS projects, w
%a preliminary investigation into the implication of AML on two existing RSSE. We consider a scenario in which, developing new software, programmers rely on a recommender system to find and use in their code third-party libraries that offer the desired features. 

 
The \emph{goal} of this study is to investigate the relevance of AML attacks for RSSE, and in particular of API and code snippet recommenders. The \emph{quality focus} is the resilience of RSSE to AML attacks. The \emph{perspective} is of researchers interested to improve the RSSE they develop. The \emph{context} consists of state-of-the-art API and code snippet recommenders.
 

We aim to address the following research questions:


%\subsection{Research questions} \label{sec:ResearchQuestions}

%By means of a series of qualitative and quantitative evaluations, we aim at answering the following research questions:

% [--]
\begin{itemize}
	\item \rqfirst~We perform a literature analysis to investigate whether there is already any effort devoted to study and deal with threats to RSSE originating from malicious data. Although our purpose is not to perform a complete, detailed systematic literature review, we followed consolidated guidelines for this kind of study in software engineering \cite{KitchenhamBLBB11,MacDonellSKM10}.
	%\item \rqsecond~By studying the working mechanism of a set of representative API recommender systems, we analyze their risk of being influenced by hostile attempts.
	\item \rqsecond~First, we perform a qualitative analysis of the likely attack threats that could affect state-of-the-art API and code snippet recommenders. Then, based on their availability, 
	we select three systems for our empirical evaluation, \ie \UM~\cite{Wang2013Mining}, PAM~\cite{Fowkes:2016:PPA:2950290.2950319}, and \FC~\cite{9359479,Nguyen:2019:FRS:3339505.3339636}. These are among the state-of-the-art approaches for API recommendations as they emerge from premier software engineering venues. We conjecture that an evaluation on these systems will help to shed light on the resilience of the majority of existing API recommenders.% systems.
%	\item \rqfourth~We are interested in understanding how the calibration of the systems' internal parameters of affects the attacks' efficiency. This is to find out how severe the possible consequences might be in practice.
%	\item \revised{\rqthird~We attempt to find feasible ways to detect malicious APIs and protect API recommender systems.}
\end{itemize}



\subsection{Addressing RQ$_1$: Literature analysis} \label{sec:Collection}




To achieve a good trade-off between the coverage of existing studies on AML in RSSE and efficiency, we defined the search strategy by answering the following four W-questions~\cite{zhang2011identifying} (``\emph{W}'' stands for Which?, Where?, What?, and When?).


 %, \ie Which?, Where?, What?, and When?~\cite{zhang2011identifying} as follows

%\revised{\textbf{Which:} \textbf{What:}  \textbf{Where:}   }
%\vspace{-.4cm}
%
%\begin{table}[t!]
%	\centering
%	\vspace{-.3cm}
%	\scriptsize	
%%	\footnotesize
%	\caption{Venues considered in the literature analysis.} %and their acronyms
%	\begin{tabular}{| p{0.2cm}|l | p{6cm} |}	\hline
%		& \textbf{Acronym} & \textbf{Name}  \\ \hline		
%		{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Conferences}}}} & ICSE & The IEEE/ACM International Conference on Software Engineering \\ \cline{2-3}
%		& ESEC/FSE & The ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering \\ \cline{2-3}
%		& ASE & The IEEE/ACM International Conference on Automated Software Engineering \\ \cline{2-3}
%		& ICSME & The International Conference on Software Maintenance and Evolution \\ \cline{2-3}
%		& ICST & The IEEE International Conference on Software Testing, Verification and Validation \\ \cline{2-3}
%		& ISSTA & The ACM SIGSOFT International Symposium on Software Testing and Analysis \\ \cline{2-3}
%		& ESEM & The ACM/IEEE International Symposium on Empirical Software Engineering and Measurement \\ \cline{2-3}
%		& MSR & The IEEE International Working Conference on Mining Software Repositories \\ \cline{2-3}
%		& SANER & The IEEE International Conference on Software Analysis, Evolution and Reengineering \\ \hline		
%		%		MSR & International Conference on Mining Software Repositories \\ \hline
%		{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Journals}}}} &	TSE & IEEE Transactions on Software Engineering \\ \cline{2-3}
%		& TOSEM & ACM Transactions on Software Engineering and Methodology \\ \cline{2-3}
%		& EMSE & Springer Empirical Software Engineering Journal \\ \cline{2-3}
%		& JSS & Elsevier Journal of Systems and Software \\ \cline{2-3}
%		& IST & Elsevier Information and Software Technology \\ \hline				
%	\end{tabular}
%	\vspace{-.2cm}
%	\label{tab:acronyms}
%\end{table}



%\color{blue}
\begin{itemize}
	\item \emph{Which?} Both automatic and manual searches were performed to look for relevant papers from conferences and journals.
	\item \emph{Where?} We conducted a literature analysis on premier venues in software engineering. 
	In particular, there are nine conferences as follows: ICSE, ESEC/FSE, ASE, ICSME, ICST, ISSTA, ESEM, MSR, and SANER. 
	Meanwhile, the following five journals were considered: TSE, TOSEM, EMSE, JSS, and IST.\footnote{We report the full name of all the venues as well as their corresponding acronyms in an online appendix \url{https://bit.ly/3jUey4K}.} %\MAX{if space allows we expand names otherwise here we should refer to the appendix with the venue names}
	The selection of conferences and journals was performed so to include mainstream venues, as well as specialized ones for which RSSE are relevant.
	The automatic search was done on the \textit{SCOPUS} database.\footnote{\url{https://www.scopus.com/}} We fetched all the papers published by a given edition (year) of a given venue (journal/conference) using the advanced search and export features.
	\item \emph{What?} For each paper collected, its title and abstract were extracted using a set of predefined keywords. %we are interested in. Table \ref{tab:keywords} reports the terms-set we 
	%	used to search for related papers. 
	To cover more possible results, we used regular expressions for searching, \eg depending on the terms we may use case sensitive queries. %, so as.
	%	\item \emph{Where?} We conduct a compact literature review on premier venues in Software Engineering, including eight conferences and five journals. For the former, we investigate eight premier venues, among others, there are ICSE, ESEC/FSE, or ASE. Meanwhile, for the latter the following five journals are considered: TSE, TOSEM, EMSE, JSS, and IST.
	\item \emph{When?} Since Adversarial Machine Learning is a recent research topic, we limit the search to the most five recent years, \ie from 2016 to 2020. %This also aims to limit.
\end{itemize}

The extraction process produced a corpus of \numPapers 
articles. 
Then, we performed various filtering steps to narrow down the search and look for those that meet our requirements. In particular, we are interested in studies 
dealing with recommender systems together with the relevant topics, \ie Adversarial Machine Learning, API mining, and malicious attempts.
Intermediate results, \eg number of downloaded papers per venue, number of candidate papers per venue, are available in our online appendix \cite{phuong_t_nguyen_2021_5105955}. %\MAX{I added the sentence before, check if it makes sense}






%narrow down the search to. %The final results are goi

%	In the end, we collected 
%Our search strategy consists of an automatic search on Electronic Data Sources (EDS). We performed search on Electronic Data Sources (EDS). 

%\item \emph{Where?} We conduct a compact literature review on premier venues in Software Engineering, including eight conferences and five journals. For the former, we investigate eight premier venues, among others, there are ICSE, ESEC/FSE, or ASE. Meanwhile, for the latter the following five journals are considered: TSE, TOSEM, EMSE, JSS, and IST.

%from these venues.


%Our search strategy consists of an automatic search on Electronic Data Sources (EDS). 
%	We performed search on Electronic Data Sources (EDS). In particular, from the \textit{SCOPUS}\footnote{\url{https://www.scopus.com/}} abstract and citation database, we extracted all the papers published by a given edition (year) of a given venue (journal/conference) using the advanced search and export features. The extraction process culminated in a corpus of 
%	In the end, we collected 
%	6,402 articles. %from these venues.

%\color{black}
%\JDR{Summarizing mSLR papers}




%\revised{%\subsection{Attack detection and countermeasures}
%Depending on the type of the consider RSSE, the literature is plenty of possible strategies to neutralize or reduce the negative effects of an adversarial attack. Mobasher \etal \cite{mobasher_attacks_2007} employ two different techniques to detect malicious attacks that involve recommended items \ie profile classification and anomaly detection. The former employs a classifier that makes use of attribute-reduction techniques to create a lower-dimensional training set. The underpinning model analyzes generic profile attributes as well as intra-profile and model-specific ones. The conducted evaluation shows that the proposed model can properly classify malicious users considering a well-defined set of metrics. Concerning anomaly detection problem, the work makes use of statistical process control (SPC) strategy to identify suspicious items trends. To this end, the model examines the items considering two parameters \ie the density of the distribution and the average ratings. The results demonstrate that detecting push attacks for popular items is more difficult while the SPC model correctly identifies attacks against low-density items. A recent work \cite{si_shilling_2020} highlights other possible countermeasures. Similar to supervised techniques, semi-supervised and unsupervised approaches have been developed with the aim of detecting attacks coming from pretended profiles. An alternative strategy could be the development of a robust recommendation algorithm that avoids possible attacks in advance. Several approaches employ matrix factorization or kernel distance even though trust-aware recommender systems are more robust than traditional ones \cite{DBLP:journals/corr/abs-1207-4525, 5428690}.
%Concerning shilling that exploits hubness, Hara \etal \cite{10.1145/2766462.2767823} propose an approach to increase the robustness of memory-based recommender system. To this end, the similarity measure exploited by the K-NN algorithm is transformed to reduce the bias that causes hubness. }


% and to deceive developers
%ai.grakn:grakn-engine:2016-11-22
%To this end, w %that appear to be similar to the target ones. We exploit a 

%<<<<<<< HEAD
%When \LR and \CR learn from existing projects and when they provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}. This resembles ratings of a user profile in online shopping systems.
%%We craft a set of forged projects exploiting a well-known technique to populate their ratings~\cite{4216981}. By the original approach~\cite{BWMB06}, a profile is divided into four independent parts, \ie \emph{unrated}, \emph{filler}, \emph{selected}, and \emph{target}. 
%To attack a recommender system, there are various approaches to populate fake user profiles~\cite{BWMB06,4216981}. Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). \MAX{this part is unclear, I think those are 2 separate problems. I think here we can only say how we create a training set for the tools, then we have to explain that a project would fall in the training set if it has good ratings, and there are ways to fake the ratings, but we did not simulate this here to avoid violating github terms of service}
%Thus, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (see Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%=======






%together with the related calls, 
%to make it more convincing, and
%in a legitimate snippet 
%make their attempt more practical by 
%The second scenario is when the developer is provided with intentionally harmful APIs embedded in a fake third-party library. In this case, 

%We simulate an attacker attempting to inject a library with malicious code (\eg by referring to the previous example, a malicious JSON parser), let it be $lib^{*}$, into the active projects. 
%For instance, the developer is searching for libraries for parsing JSON documents and the system should be able to suggest those that are used by similar projects. 

%In practice, to avoid being detected, an attacker probably gives the library a copycat name, \ie one that closely resembles a popular library, aiming to disguise it better. For instance, a malicious library has been named as ``\emph{jeIlyfish}'' to deceive developers into believing it ``\emph{jellyfish},'' the authentic library.\footnote{\url{https://bit.ly/394uETI}} In this way, developers would adopt the disguised library without hesitation, once it has been suggested by the recommendation engine.

%In fact, typosquatting has been reported in recent work~\cite{10.1145/3196398.3196401}, and this indeed suggests an evident threat to the adoption of third-party libraries. 
%\ie a set of APIs, 



%\color{red}




%\revised{In practice, to avoid being detected, an attacker normally names $lib^{*}$ using a copycat name, aiming to disguise it. For instance, .}

%================================================
%When \LR and \CR learn from existing projects to %and when they 
%provide recommendations, they treat a project's library usage as a vector, where each entry corresponds to a library: 1 means that the library is included in the project, 0 otherwise~\cite{6671293,NGUYEN2019110460}.
%To attack a recommender system, there are various approaches to populate ratings for fake user profiles~\cite{BWMB06,4216981}. 
%Unfortunately, they cannot be directly applied to forge projects, since they deal with multi-level ratings, while in library recommendation there are only two \emph{ratings} (0 and 1). 
%Thus, to create a training set for the \LR and \CR tools, we have to devise a new method to produce fake projects as follows. A project's vector is divided into two independent parts, namely \emph{filler libraries} and \emph{target library} (see 
%Fig.~\ref{fig:FakeProject}). We fill in the former with a set of libraries from training data; while the latter is set to $lib^{*}$. The manipulation aims to achieve two goals: \emph{(i)} making the fake project be similar to active projects; and \emph{(ii)} boosting the presence of $lib^{*}$.
%================================================

%We come across the following question: ``\emph{Which libraries should be chosen as fillers, so that the fake project will be incorporated into the recommendation?}'' In fact, recommenders heavily rely on similarity~\cite{Schafer:2007:CFR:1768197.1768208}, thus we come up with the selection of popular libraries as fillers. Our intuition  is that, a fake project with libraries widely used by other projects is likely to get attention from the recommendation engine. A list of libraries in the training projects is populated and sorted in descending order of the number of caller projects. A certain number of the most popular libraries is then randomly selected.

%\color{black}

%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\Omega$ is the number of fillers. For \LR and \CR, \emph{k} is the number of similar projects and \emph{N} is the cut-off value for the ranked list of recommendations~\cite{6671293,NGUYEN2019110460}. We conducted experiments using ten-fold cross-validation on a dataset crawled from \GH consisting of 1,400 projects and 13,497 libraries. For a testing project, we randomly split its libraries into two equal parts, the first part is used as a query, while the second one is ground-truth data. To measure the effectiveness of the push attacks, we use \emph{Hit ratio} \emph{HR@N}, 
%defined as the ratio of projects being recommended with $lib^{*}$ to the total number of testing projects~\cite{10.1007/978-3-030-49461-2_18}. 
%To measure the accuracy, we use success rate \emph{SR@N}, \ie the ratio of projects getting at least a matched library (the size of the intersection of the recommended list with the ground-truth data is larger than 0) to the number of testing projects.
%We experimented with $\alpha$=$\{5\%,10\%\}$ as attack size; 
%$k$=$\{5,10,15,20\}$; $\Omega$=$\{3,4,6,8,10\}$ as fillers' size. The calibration of these parameters allows us to simulate \emph{stress tests}, aiming to investigate the systems' safeness under different working conditions. 


%\begin{figure}[t!]
%	\centering
%	\vspace{-.3cm}
%	\includegraphics[width=0.68\linewidth]{figs/FakeProject.pdf}
%	\vspace{-.3cm}
%	\caption{Manipulation of library usages for a fake project.}
%	\label{fig:FakeProject}
%	%	\vspace{-.3cm}
%\end{figure}







\subsection{Addressing RQ$_2$: Qualitative analysis and experiment on three RSSE} 
\label{sec:rq2-design}

To address RQ$_2$, we looked at the same venues considered in RQ$_1$ to identify, over the period 2010--2020, API recommender systems as well as RSSE suggesting API code example snippets. We then qualitatively discuss, for each recommender,   the working mechanism, and its potential risks. 

Then, based on the tool availability as well as the characteristics of the tools, we select three of them,  \ie \UM~\cite{Wang2013Mining}, PAM~\cite{Fowkes:2016:PPA:2950290.2950319}, and \FC~\cite{Nguyen:2019:FRS:3339505.3339636}.
To evaluate the resilience of \UM, PAM, and \FC, we use a dataset containing Android apps' source code. We focused on Android apps because they entail a typical scenario in which an infection can cause unwanted consequences such as data leaks.


%To mine data for the experiments, 
We made use of a dataset which was curated through our recent work~\cite{9359479}, and the collection process is summarized as follows. First, we searched for open source projects using the \emph{AndroidTimeMachine} platform~\cite{8595172}, which retrieves apps and their source code from Google Play\footnote{\url{https://play.google.com/}} and \GH. Second, APK files are fetched from the Apkpure platform,\footnote{\url{https://apkpure.com/}} using a Python script. 
Third, the \emph{dex2jar} tool \cite{dex2jar} is used to convert the APK files into the JAR format. The JAR files were then fed as input for Rascal to convert them into the M$^3$ format~\cite{Basten2015M3}. We obtained a set of \numApps apps with full source code. To simplify the evaluation, 
we inject APIs at the metadata level, \ie after the data that has been parsed to a processable format. This is for experimental purposes only since, in reality, attackers need to seed data directly to projects and upload them to \GH as shown in Fig.~\ref{fig:PushAttacks}. However, in our evaluation we refrained from doing this to carefully follow ethical boundaries, as well as to avoid adversely impacting real-world systems. %, and infringing their terms of use 

%This is outside the focus of this paper, and we leave it for future work. 

%

We then inserted fake APIs into random projects and declarations, attempting to simulate real-world scenarios where APIs are dispersed across several declarations. Finally, the resulting data is parsed in two formats, \ie ARFF files to be fed to \UM and PAM, and a special file format for providing input to \FC. By an empirical evaluation, we realized that \UM and PAM suffer from scalability issues, \ie they cannot work on large datasets. Thus for evaluating them, we could only consider a subset consisting of 500 apps. For \FC, the whole \numApps apps are used since the system is capable of handling well a large amount of data.


There are the following parameters to consider when it comes to populating artificial projects. 

%We illustrate in 
%Attackers may disguise the planted projects by starring and forking them with forged accounts. 
%making it more convincing, 
%=======================
%Such a trick has been recently revealed, where several \GH repositories hosting malware apps have been found~\cite{Rokon2020SourceFinderFM}.\footnote{\url{https://zd.net/3bg3CK9}} To our knowledge, research conducted to combat this type of abuse %crime %misbehaviour 
%is still in its initial phase~\cite{10.1145/3357384.3357971}. %,Rokon2020SourceFinderFM
%=======================
%Avoiding detection, 
%Since a project may consist of several declarations (see Section~\ref{sec:Definitions})
%To boost up the popularity of an API pattern, it is necessary to seed the APIs to not only one but more projects. 

\begin{itemize}
	\item $\alpha$ is the ratio of projects injected with fake APIs (in percent, \%).	
	\item $\beta$ is the ratio of methods in a project getting fake APIs (in percent, \%).
	\item $\Omega$ is the number of fake APIs injected to each declaration.
	\item \emph{N} is cut-off value for the ranked list of recommended items returned by a recommender system.
\end{itemize}

%It is worth noting that these parameters are under control of attackers, \ie they can be fined tune to make attacks more effective.
%On the attacker's side, $\alpha$ is the ratio of fake projects to the total number of projects (in \%); $\Omega$ is the number of fillers. 
%In the evaluation, we experiment with different configurations by varying the parameters to analyze which settings bring more perturbed outcomes.

We experiment with the following sets of parameters: $\alpha$=$\{5\%,\-10\%,15\%,20\%\}$, $\beta$=$\{40\%,50\%,60\%\}$, $\Omega$=$\{1,2\}$. The rationale behind the selection of these values is as follows. Concerning $\alpha$, though having popular APIs is commonplace, it is difficult to rack up projects with malicious APIs, thus $\alpha$ is set a small percentage, \ie %the following thresholds 
$\alpha$=$\{5\%,\-10\%,15\%,20\%\}$. In contrast, within a project, attackers have more freedom to embed APIs to declarations, therefore $\beta$ is varied from 40\%, 50\%, to 60\%. Finally, as explained in Section~\ref{sec:Example}, the number of fake APIs should be kept low to make attacks more feasible,  
\ie $\Omega$=$\{1,2\}$. We study how the calibration of the parameters affects the final efficiency, aiming to anticipate the extent to which the attacks are successful in the field. 



We inspected the dataset produced as explained above, and counted 26,852 unique APIs in all the apps. Fig.~\ref{fig:NumOfDeclarations} depicts the distribution of APIs in projects and declarations. The x-Axis and the y-Axis specify the number of projects and the number of declarations in which an invocation is seen, respectively. The dense cluster of points on the lower-left corner suggests that most of the APIs appear in less than 250 projects and 200 declarations. Meanwhile, a small fraction of them are invoked by a large number of projects and declarations, \ie more than 2,000 and 10,000, respectively. Such a distribution has an impact on the $\alpha$ and $\beta$ parameters.

\begin{figure}[t]
	\centering
	%\vspace{-.1cm}
	\includegraphics[width=0.86\linewidth]{figs/ProjectDeclarations3.png}
	%\vspace{-.1cm}
	\caption{Frequency of APIs in projects and declarations.} %Summary of the main words
	\vspace{-.3cm}
	\label{fig:NumOfDeclarations}
\end{figure}



The figure indicates that some APIs are extremely frequent. By looking inside the dataset, we see that \texttt{\hl{\small java/lang/String\-Builder/append(java.l\-ang.String)}} is the most popular API as it appears in 96.61\% of the projects. Other invocations specific to Android apps, such as \texttt{\hl{\small android/view/View/get\-Right()}}, are also very common in the dataset. The presence of very popular APIs gives us some hints on how to inject malicious APIs having the same names. We conjecture that, even if we embed an artificial API on a large number of projects, this can be seen as normal and thus, does not arouse developers' suspicion. 



We conducted experiments using the ten-fold cross-validation meth\-odology, \ie the dataset with $\left| P \right|$  projects is divided into ten equal parts, and each experiment composed of ten train/test tasks. For each round of execution, one part is used for testing, while the other nine remaining parts are fed as training.% data. 

To measure the effectiveness of push attacks, we employ \emph{Hit ratio} \emph{HR@N}~\cite{10.1007/978-3-030-49461-2_18,mobasher_attacks_2007}, which is defined as the ratio of projects being provided with a fake API $\left| T \right|$ to the total number of testing projects $\left| P \right|$, \ie $HR@N = \left| T \right| / \left| P \right|$, with N being the cut-off value for the ranked list. The metric is computed over the results of all the ten folds.






==> src/Introduction2.tex <==

%In recent years, software projects have reached a higher degree of complexity due to the heterogeneous resources involved in the development process. 

%When dealing with certain coding tasks, rather than 
%implementing a new system from scratch, developers usually 
%make use of third-party libraries (TPLs) that provide the 
%desired functionalities. Third-party libraries offer a wide range of 
%operations, \eg database management, file utilities, Website 
%connection, to name a few. Employing existing third-party 
%libraries allows developers to re-use a well-founded 
%infrastructure, without reinventing the wheel, which 
%eventually helps save time as well as increase productivity. 
%However, TPLs evolve over the course of time 
%and API functions can be added, and many others can be 
%removed, e.g., to make the library more efficient or to 
%fix some security issues. 
%%
%Migrating clients code from one library release to a target 
%one can be difficult and time-consuming especially when the 
%API being upgraded introduce breaking changes that make the 
%client fail to compile or introduce  behavioral changes into 
%it \cite{7884616}. However, managing TPLs and keeping them 
%up-to-date becomes a critical practice, so as to minimize the technical debt~\cite{avgeriou_et_al:DR:2016:6693}. %to do not make the technical debt growing \cite{avgeriou_et_al:DR:2016:6693}.
%
%are employed to realize complex functionalities without wasting precious time. 
%Most of them offer utilities to perform 
%Even though they are very powerful software components, TPLs require a lot of effort in the initial integration within the project as well as in the maintenance over time. 
%In this way, it is necessary to migrate an old library to a 
%new one, so as to enforce the new functionalities on the 
%project. 
%In general, there are two main 
%categories of migration as follows: \emph{(i)} replacement of 
%a library with a 
%different one with similar functionalities; and \emph{(ii)} 
%upgrading the same 
%library to a newer version. The former impacts negatively on 
%coupling 
%\cite{alrubaye_how_nodate}, as the migration can break many 
%mutual dependencies 
%of the different libraries. Meanwhile, the latter affects 
%instead the internal 
%relationships of a certain library measured by various 
%cohesion metrics. 
%\cite{alrubaye_how_nodate}. 
%Several approaches already face both of the migration categories even though the room of improvements are still available, \ie retrieving and storing migration data or clearly identify the intermediate steps to make two concrete examples. 

%In order to migrate a client $C$ from an initial library 
%version $l_{v_i}$ to a target one $l_{v_t}$, the developer 
%needs to understand very well the documentation of both 
%versions as well as to choose the right matching between 
%corresponding methods. 
%%Given the circumstances, the lack of 
%%knowledge about how to migrate the client $C$ to the library 
%%$l_{v_t}$ may impede the development process. 
%Things are even more complicated when several subsequent 
%versions of the library of interest $l$ have been released 
%from $v_i$  to  $v_t$. 
%In such cases, developers that want to reduce the technical 
%debts, which have been accumulated due to libraries 
%that have not been upgraded yet, have first to decide the 
%\textit{upgrade plan} that has to be applied, i.e., how to go 
%from $l_{v_i}$  to  $l_{v_t}$ since many possible paths might 
%be 
%followed. In such cases, it is essential to have proper 
%machinery to assist developers in choosing suitable upgrade 
%plans to reduce the efforts that are needed to migrate the 
%client project  $C$ 
%under development. It is possible to minimize migration 
%efforts, by identifying the upgrade plan, which minimizes the 
%errors on the client $C$ that need to be fixed, and by 
%providing developers with supporting material, e.g., 
%documentation, and snippets of code examples, which can be 
%considered during the migration phases.


%, although minimize the issues that arise during the actual adaptation is a real challenge to be faced.
%The literature is plenty of studies that analyze the problem from different perspectives \ie users' awareness \cite{kula_developers_2018} or releases' documentation \cite{lamothe_exploring_2018}.
%A source code project that contains API calls coming from an old version of a library cannot work when it is integrated with a new version of the library. 
%libraries' 
%In this sense, depending software clients of a library need to be migrated in order to make use of a new library version, and this is understood as \emph{API migration}. However, the manual migration process between different library version is time-consuming and prone to error~\cite{DBLP:journals/corr/abs-1812-04894}. 
%Concerning migration, %it can fall into 
%==============================================================================
%In recent years, software development activity has reached a high degree of 
%complexity, led by the heterogeneity of the components, data sources, and 
%tasks. To address such challenges, suitable mechanisms are needed to transform 
%raw data into practical knowledge that in turn helps developers with their 
%programming tasks. 
%==============================================================================
%The introduction of recommender systems in software engineering \cite{robillard_recommendation_2014} permits to assist developers in navigating large information spaces and getting instant recommendations that might be helpful to solve the particular development problem at hand. Thus, a recommender system in software engineering (RSSE) aims at giving developers recommendations, which can consist of different items including code examples, issue reports, reusable source code, possible third-party components, documentation, to name a few~\cite{robillard_recommendation_2014}.
%With the aim of proposing a recommender system \cite{robillard_recommendation_2014} tailored for this domain, 


%In this work, we introduce \tool, a novel approach to recommend
%upgrade plans for third-party libraries. By exploiting the 
%experience of other projects that have already performed similar 
%upgrades and migrations, \tool recommends the upgrade plan 
%that should be performed to migrate from the current library 
%version to the desired one. Recommendations are inferred by 
%analyzing  \GH repositories that are similar to the project 
%under development. In particular, by considering 
%\emph{pom.xml} files, a graph-based representation is built to 
%represent the upgrade plans that existing repositories have 
%already performed.
%
%support the the 
%upgrade of TPLs: %given an initial version of a certain 
%%library. 
%by analyzing \GH repositories' commits, \tool is able to 
%infer relevant data from commits that affect the 
%\emph{pom.xml} file(s) of the project. Afterwards, a graph is 
%built using this data to create relationships between two 
%versions. 
%During the graph creation phase, \tool assigns weights that 
%represent the number of clients projects performing a specific 
%upgrade. In the recommendation phase, a shortest-path 
%algorithm is employed to minimize the number of upgrade steps, 
%taking into consideration the aforementioned weights. As 
%output, \tool delivers an upgrade plan to the user with the 
%target version as well as all the intermediate passages. 
%%Though several tools are already in place, they cannot 
%%provide a replication package for a suitable comparison. 
%%Thus, w
%To the best of our knowledge, there exists no tool that 
%provides this type of recommendations. Thus, we evaluate \tool 
%by using metrics commonly used in information retrieval 
%applications, \ie precision, recall, and F-measure. 
%Furthermore, we limit ourselves to recommend just an ideal 
%plan rather than apply directly the suggested upgrades in the 
%source code of the project. %Nevertheless, we believe that

%========================================================================
%To cope with their everyday programming tasks,  developers access and browse
%various information sources~\cite{Dagenais:2010:MNS:1806799.1806842}. %, often in a short time \cite{Dagenais:2010:MNS:1806799.1806842}. 
%Given the wide availability of sources of formal and informal documentation, %In such a context, 
%the problem is not a lack but instead, information overload \cite{Murphy09,Murphy-HillMG10}.
%========================================================================

%Recently, many studies have been conducted to develop methods and tools --- 

%===============================
	%In Computer Vision, a non-random noise added to images is imperceptible to humans, however it may steer ML models to perform wrong prediction~\cite{conf/cvpr/NguyenYC15}. For example, a panda was recognized as a ribbon by state-of-the-art deep neural networks after the input image had been padded with noise, meanwhile humans still correctly perceived the panda from the forged image~\cite{DBLP:journals/corr/GoodfellowSS14}.	
%===============================	
	

In recent years, several recommender systems for software engineering (RSSE) have been conceptualized to support developers in their task and, possibly, reduce the increasing information overload originating from the availability of data from various sources~\cite{di_rocco_development_2021,Gu2016DeepAPI,Murphy09,Murphy-HillMG10,NGUYEN2019110460,DBLP:journals/ese/PonzanelliBPOL16}. A relevant example of RSSE is represented by API recommender systems, which provide developers with function calls and/or code snippets being beneficial to their coding
tasks~\cite{Moreno:2015:IUT:2818754.2818860,Nguyen:2019:FRS:3339505.3339636,robillard_recommendation_2014}. Such systems learn their recommendations (of code snippets or APIs) from external sources such as code bases, \eg \GH or communication channels, \eg Stack Overflow. Since these sources are open for changes and contributions by the crowd, the recommenders' learning material might be exposed to malicious attacks~\cite{zhang_cyber-guided_2020}. In other words, these sources can be exploited to fool API recommender systems.

%In fact, data from these sources contains noise, as this has been already reported~\cite{KalliamvakouGBSGD14}. 

Adversarial attempts generate perturbations to deceive and disrupt systems by causing a malfunction, compromising their recommendation capabilities. For instance, an adversarial attack to recommender systems, depending on the intent, can favor or defame an item, thus creating a negative impact on the final recommendations~\cite{10.1007/s10462-012-9364-9}. Similarly, by manipulating training data available in OSS platforms, hostile users may render recommender systems vulnerable to harmf\-ul artifacts. If a recommender is trained to provide malicious APIs or snippets, this can trigger disruptions to a software system. For example, a recent work~\cite{DBLP:conf/ndss/WuGCHCD19} shows that there have been attempts using toxic code to secretly force Android apps to open ports, allowing for unauthorized access.

%a malicious snippet may 
%In this way, attackers may try to manipulate the open data. 
% used to train recommenders can be 
%As a consequence, the outcome of the provided recommendation depends very much on the quality of the input data. 
%However, data used to feed API recommender systems generally comes from open source platforms, such as the Maven Central Repository, SourceForge, Microsoft Codebase, or the most popular one, \GH. 
%. RSSE provide developers with automated assistance 

%\revised{Though a lot of improvements have been obtained so far, there is still the need to make RSSE more effective and robust. More importantly, while a large number of attempts have been made 
%	to improve the recommendation accuracy, little attention has been paid to make systems robust and resilient to malicious data. In fact, by manipulating training data available in open source software platforms, a hostile user can render recommender systems vulnerable to adversarial attacks. Thus, we come across two additional questions: ``\emph{What causes harm to RSSE?}'' and ``\emph{How can we defend them against adversarial attempts?}''}

%existing code bases or informal documentation. 
%The development of RSSE encompasses several phases including the design of the underpinning algorithms or the reuse of existing ones. Machine Learning (ML) techniques are amongst the natural choices that developers take when new recommender systems have to be conceived

%\MAX{cite here the most relevant ones from our table}

%to the domain of software development 
%A recommender system in software engineering is defined as \emph{``... a  software application that provides information items estimated to be valuable for a software engineering task in a given context''}~\cite{robillard_recommendation_2014}. 

%%============================The following paragraph needs to be completely rephrased==========================================
%%Deep Learning is the driving force of recent developments and breakthroughs in the field of Artificial Intelligence (AI). 
%%the most successful approach to the way machines learn as well as improving the way to function independently and without human intervention. 
%The proliferation of disruptive Machine Learning (ML) and especially Deep Learning (DL) algorithms %techniques %deep neural networks 
%in recent years has enabled a plethora of applications across several domains. Such techniques work on the basis of complex artificial neural networks, which are capable of effectively learning from data by means of a large number of hyper-parameters distributed in different network layers.
%%Neural networks - artificial abstraction models in the human brain - are trained using modern learning algorithms and huge datasets. The result is that speech recognition systems improve independently; cars drive autonomously based on environmental sensor information; medical applications exceed a physician's performance.
%%==============================================================================
%%thereby culminating in Deep Learning. 
%% In recent years
%%Recently, the intensive use of Recommender systems in Software Engineering has brought in benefits. 
%%Different AI techniques to deploy in Software Engineering. 
%%In Software Engineering
%In a nutshell, DL techniques are %deemed to be 
%an advanced paradigm that brings in substantial improvement in performance compared to conventional learning algorithms. %In recent years, 
%Recently, there is an increasingly number of applications of ML/DL techniques %. The deployment of Deep Learning techniques 
%to address challenging issues in Software Engineering, with the aim of improving the synergy between the two domains~\cite{10.1145/3172871.3172891,Shafiq2020MachineLF,DBLP:conf/icse/AmershiBBDGKNN019}.


%attempts to fuse 
%============================Adversarial Machine Learning in Recommender Systems============================


Research on Adversarial Machine Learning~\cite{10.1145/2046684.2046692,6015575} (AML) studies security issues in Machine Learning systems as well as general-purpose recommender systems~\cite{10.1145/3439729}. So far, AML has been investigated in different domains, \eg online systems~\cite{4216981}, image classification~\cite{conf/cvpr/NguyenYC15}, and addresses both threats and countermeasures~\cite{10.1007/978-3-030-49461-2_18,wang_adversarial_2020}. However, to the best of our knowledge, the issue of AML in recommender systems remains unexplored in software engineering.


%=========================
%\MAX{I think this text can be dropped because it is somewhat repetitive of what said before and later.}
%To be concrete, through a careful observation, we realize that no studies have been conducted to investigate the abuse of deliberately forged data to spoil API recommender systems' outcomes, as well as to conceive suitable counteractions. In fact, while the research community either underestimates or ignores it, the possibility of using falsified data to trick RSSE is always present, posing a potential danger to software systems. In this sense, there is the need to perceive the likely threats, with the ultimate aim of conceptualizing countermeasures to increase the resilience of RSSE. 

%=========================
%\MAX{I know these are motivating questions, however I'm afraid the reader would seek answers to these questions}
%Thus, we come across two motivating questions: ``\emph{What may cause harm to API recommender systems?}'' and ``\emph{How can we defend them against adversarial attempts?}'' 
%=========================

%And it is time to wake up and smell the coffee.

%, but it is ignored by the community
%conceiving counteractions to increase the resilience of RSSE.
%=========================
%while there are some initial efforts to, 
%=========================
%=========================
%Though a lot of improvements have been obtained so far, there is still the need to make RSSE more effective and robust.
%According to our observation, while a large number of attempts have been made to improve the recommendation accuracy, little attention has been paid to make systems robust and resilient to malicious data. 
%=========================
%=========================



%in a way that it will be falsely classified by 
%, whilst still being imperceptible recognized by humans
%manipulate target items, either to aiming to 
%Adversarial attacks 
%Depending on the attacker's intention 

% However, to the best of our knowledge, AML has not been investigated in the context of SE applications of ML yet.

%The ultimate aim of these attacks is to

%For example, Anelli \etal~\cite{10.1007/978-3-030-49461-2_18} use shilling attack~\cite{DBLP:journals/air/SiL20} to manipulate a collaborative-filtering recommender system operated with Linked Data. Also, Wang and Han \cite{wang_adversarial_2020} propose an improvement of the Bayesian personalized ranking (BPR) technique by exploiting the adversarial training-based mean strategy (AT-MBPR) in the domain of collaborative filtering-based recommender systems.

% to protect systems against attacks
%Adversarial Machine Learning (AML) is an emerging research topic that is a combination of the best practices in various fields, including Machine Learning, robust statistics, and computer security~\cite{DDM20a,10.1145/2046684.2046692}. %[115, 134] %Tommaso Di Noia. %Adversarial machine learning 

%A main way to achieve this is to feed systems with malicious data~\cite{DDM20a}.


%image is still seen as the same panda 
%Adversarial examples: ML models misclassify examples that are only slightly different from correctly classified .... ~\cite{43405}.
%The learned model slightly differs from the true data distribution.
%============================Limitations of existing work===============================================================
%and how to synergically integrate machine intelligence and human intelligence (e.g., domain knowledge or insight) to effectively tackle challenging software engineering problems


%Most RSSE heavily rely on open data sources, such as \GH, the Maven Central Repository, or Stack Overflow, which can be easily steered by adversaries \cite{zhang_cyber-guided_2020}. In other words, these systems are vulnerable to attacks equipped with forged input data. %Therefore, there is the need for comprehending the likely threats, with the ultimate aim of 
%\color{red}
%===================================================The aim of this paper===============================================
%We first provide an overview of state-of-the-art API recommenders, discussing  how they could be potentially affected by AML. Through a literature search from premier venues in Software Engineering for adversarial techniques, we show that there are considerably evident threats to RSSE.
%\color{black}

%To defend a system against threats, in the first place, it is necessary to be knowledgeable of various types of adversary activities~\cite{4216981}. 

%with the existing RSSE, there are %considerably 
%highly evident risks of being manipulated by adversarial techniques.
%adversarial attacks. 

%\MAX{see if you like how I state the papers' contribution here}

In this paper, we provide a first empirical investigation into the relevance and effects of AML in RSSE. First, through a literature analysis on 14 premier venues in software engineering, we show that there has been no work to study the issue of AML in RSSE. Afterwards, we present a qualitative analysis of state-of-the-art API recommenders, underlining their risk of being manipulated by adversarial techniques. Then, we perform an empirical evaluation on three API recommenders using  data seeded in real OSS projects. The results reveal a worrisome outcome: by crafting input data to feed the systems, we can manipulate the recommendations, successfully promoting fake/toxic API calls. Last but not least, we devise some possible countermeasures to cope with this type of manipulations. 
%
%In summary, our paper makes the following contributions: 
%\MAX{said before}
%Altogether, our work is novel as it is the first one to study threats that cause harm 
%to RSSE providing API calls and code snippets, as well as to evaluate on real API recommender systems to perturb their recommendation capability. 
%a simple manipulation, we can seamlessly
%In this respect, our work is the first one that brings in the issue of AML in RSSE.

The preliminary idea of studying attacks to RSSE has been outlined in our previous short paper~\cite{10.1145/3463274.3463809}, which has been thoroughly extended in this work under different dimensions including the analysis of code snippet seeding scenario. In particular, this paper makes the following contributions: 
\begin{itemize}
	\item[--] A literature review on major software engineering venues to show that the topic of AML in RSSE has not been properly studied by existing research.
	\item[--] A comprehensive qualitative analysis of relevant, state-of-the-art API recommender systems and their risk of being affected by bogus data. 
	\item[--] An empirical study on three state-of-the-art API recommenders, evaluating their resilience to adversarial attacks.
	\item[--] A replication package has been made available to facilitate future research~\cite{phuong_t_nguyen_2021_5105955}.
\end{itemize}

The paper is structured as follows: Section \ref{sec:Background} provides a motivating example and background of adversarial attacks. Section \ref{sec:Evaluation} details the study definition and planning.  The results are reported and discussed in Section~\ref{sec:Results}. Section~\ref{sec:Countermeasures}, outlines possible countermeasures to AML for API recommenders. Section~\ref{sec:RelatedWork} reviews related work. Finally, Section~\ref{sec:Conclusion} outlines future work and concludes the paper. 






%, putting software clients at risk
%risk on the learning models. 
%have suggested it is due to extreme nonlinearity of deep neural networks.
%\begin{itemize}
%\item A condensed literature review on recommender systems in Software Engineering;%applications of ML/DL in Software Engineering;
%	\item A summary of most notable RSSE to provide third-party libraries and API function calls; \MAX{I wouldn't call this a contribution, I suggest to merge this with the next, saying ``A discussion fo the possible adversarial attacks on state-of-the-art RSSE for third-party libraries and API calls''}
%\vspace{.4cm}
%\noindent
%$\rhd$~
%\end{itemize}

%\vspace{.05cm}
%\noindent
%$\rhd$~\emph{A review}: 
%
%\vspace{-.05cm}
%\noindent
%$\rhd$~\emph{Possible implications on the Software Engineering domain}: 

%\vspace{.05cm}


==> src/Introduction_temp.tex <==

%In recent years, software projects have reached a higher degree of complexity due to the heterogeneous resources involved in the development process. 

%When dealing with certain coding tasks, rather than 
%implementing a new system from scratch, developers usually 
%make use of third-party libraries (TPLs) that provide the 
%desired functionalities. Third-party libraries offer a wide range of 
%operations, \eg database management, file utilities, Website 
%connection, to name a few. Employing existing third-party 
%libraries allows developers to re-use a well-founded 
%infrastructure, without reinventing the wheel, which 
%eventually helps save time as well as increase productivity. 
%However, TPLs evolve over the course of time 
%and API functions can be added, and many others can be 
%removed, e.g., to make the library more efficient or to 
%fix some security issues. 
%%
%Migrating clients code from one library release to a target 
%one can be difficult and time-consuming especially when the 
%API being upgraded introduce breaking changes that make the 
%client fail to compile or introduce  behavioral changes into 
%it \cite{7884616}. However, managing TPLs and keeping them 
%up-to-date becomes a critical practice, so as to minimize the technical debt~\cite{avgeriou_et_al:DR:2016:6693}. %to do not make the technical debt growing \cite{avgeriou_et_al:DR:2016:6693}.
%
%are employed to realize complex functionalities without wasting precious time. 
%Most of them offer utilities to perform 
%Even though they are very powerful software components, TPLs require a lot of effort in the initial integration within the project as well as in the maintenance over time. 
%In this way, it is necessary to migrate an old library to a 
%new one, so as to enforce the new functionalities on the 
%project. 
%In general, there are two main 
%categories of migration as follows: \emph{(i)} replacement of 
%a library with a 
%different one with similar functionalities; and \emph{(ii)} 
%upgrading the same 
%library to a newer version. The former impacts negatively on 
%coupling 
%\cite{alrubaye_how_nodate}, as the migration can break many 
%mutual dependencies 
%of the different libraries. Meanwhile, the latter affects 
%instead the internal 
%relationships of a certain library measured by various 
%cohesion metrics. 
%\cite{alrubaye_how_nodate}. 
%Several approaches already face both of the migration categories even though the room of improvements are still available, \ie retrieving and storing migration data or clearly identify the intermediate steps to make two concrete examples. 

%In order to migrate a client $C$ from an initial library 
%version $l_{v_i}$ to a target one $l_{v_t}$, the developer 
%needs to understand very well the documentation of both 
%versions as well as to choose the right matching between 
%corresponding methods. 
%%Given the circumstances, the lack of 
%%knowledge about how to migrate the client $C$ to the library 
%%$l_{v_t}$ may impede the development process. 
%Things are even more complicated when several subsequent 
%versions of the library of interest $l$ have been released 
%from $v_i$  to  $v_t$. 
%In such cases, developers that want to reduce the technical 
%debts, which have been accumulated due to libraries 
%that have not been upgraded yet, have first to decide the 
%\textit{upgrade plan} that has to be applied, i.e., how to go 
%from $l_{v_i}$  to  $l_{v_t}$ since many possible paths might 
%be 
%followed. In such cases, it is essential to have proper 
%machinery to assist developers in choosing suitable upgrade 
%plans to reduce the efforts that are needed to migrate the 
%client project  $C$ 
%under development. It is possible to minimize migration 
%efforts, by identifying the upgrade plan, which minimizes the 
%errors on the client $C$ that need to be fixed, and by 
%providing developers with supporting material, e.g., 
%documentation, and snippets of code examples, which can be 
%considered during the migration phases.

 
%, although minimize the issues that arise during the actual adaptation is a real challenge to be faced.
%The literature is plenty of studies that analyze the problem from different perspectives \ie users' awareness \cite{kula_developers_2018} or releases' documentation \cite{lamothe_exploring_2018}.
%A source code project that contains API calls coming from an old version of a library cannot work when it is integrated with a new version of the library. 
%libraries' 
%In this sense, depending software clients of a library need to be migrated in order to make use of a new library version, and this is understood as \emph{API migration}. However, the manual migration process between different library version is time-consuming and prone to error~\cite{DBLP:journals/corr/abs-1812-04894}. 
%Concerning migration, %it can fall into 
%==============================================================================
%In recent years, software development activity has reached a high degree of 
%complexity, led by the heterogeneity of the components, data sources, and 
%tasks. To address such challenges, suitable mechanisms are needed to transform 
%raw data into practical knowledge that in turn helps developers with their 
%programming tasks. 
%==============================================================================
%The introduction of recommender systems in software engineering \cite{robillard_recommendation_2014} permits to assist developers in navigating large information spaces and getting instant recommendations that might be helpful to solve the particular development problem at hand. Thus, a recommender system in software engineering (RSSE) aims at giving developers recommendations, which can consist of different items including code examples, issue reports, reusable source code, possible third-party components, documentation, to name a few~\cite{robillard_recommendation_2014}.
%With the aim of proposing a recommender system \cite{robillard_recommendation_2014} tailored for this domain, 


%In this work, we introduce \tool, a novel approach to recommend
%upgrade plans for third-party libraries. By exploiting the 
%experience of other projects that have already performed similar 
%upgrades and migrations, \tool recommends the upgrade plan 
%that should be performed to migrate from the current library 
%version to the desired one. Recommendations are inferred by 
%analyzing  \GH repositories that are similar to the project 
%under development. In particular, by considering 
%\emph{pom.xml} files, a graph-based representation is built to 
%represent the upgrade plans that existing repositories have 
%already performed.
%
%support the the 
%upgrade of TPLs: %given an initial version of a certain 
%%library. 
%by analyzing \GH repositories' commits, \tool is able to 
%infer relevant data from commits that affect the 
%\emph{pom.xml} file(s) of the project. Afterwards, a graph is 
%built using this data to create relationships between two 
%versions. 
%During the graph creation phase, \tool assigns weights that 
%represent the number of clients projects performing a specific 
%upgrade. In the recommendation phase, a shortest-path 
%algorithm is employed to minimize the number of upgrade steps, 
%taking into consideration the aforementioned weights. As 
%output, \tool delivers an upgrade plan to the user with the 
%target version as well as all the intermediate passages. 
%%Though several tools are already in place, they cannot 
%%provide a replication package for a suitable comparison. 
%%Thus, w
%To the best of our knowledge, there exists no tool that 
%provides this type of recommendations. Thus, we evaluate \tool 
%by using metrics commonly used in information retrieval 
%applications, \ie precision, recall, and F-measure. 
%Furthermore, we limit ourselves to recommend just an ideal 
%plan rather than apply directly the suggested upgrades in the 
%source code of the project. %Nevertheless, we believe that

To cope with their everyday programming tasks,  developers access and browse
various information sources~\cite{Dagenais:2010:MNS:1806799.1806842}. %, often in a short time \cite{Dagenais:2010:MNS:1806799.1806842}. 
Given the wide availability of sources of formal and informal documentation,
%In such a context, 
the problem is not a lack but instead, information overload \cite{Murphy09,Murphy-HillMG10}. Recently, many studies have been conducted to develop methods and tools --- recommender systems for software engineers (RSSE) --- to provide developers with automated assistance~\cite{Gu2016DeepAPI,DBLP:journals/ese/PonzanelliBPOL16,NGUYEN2019110460}. %\MAX{cite here the most relevant ones from our table}



The development of RSSE %recommender systems 
encompasses several phases including the 
design of the underpinning algorithms or the reuse of existing ones. Machine 
Learning (ML) techniques are amongst the natural choices that developers take 
when new recommender systems have to be conceived 
~\cite{robillard_recommendation_2014}. This means, for example, that the recommendation of code elements (\eg snippets or APIs) is learned from existing code bases or informal documentation. As a result, %consequence, 
the quality of the provided recommendation depends on the quality of such data, whose noisiness has been previously reported %in previous research 
\cite{KalliamvakouGBSGD14}.

%to the domain of software development 
%A recommender system in software engineering is defined as \emph{``... a  software application that provides information items estimated to be valuable for a software engineering task in a given context''}~\cite{robillard_recommendation_2014}. 



%%============================The following paragraph needs to be completely rephrased==========================================
%%Deep Learning is the driving force of recent developments and breakthroughs in the field of Artificial Intelligence (AI). 
%%the most successful approach to the way machines learn as well as improving the way to function independently and without human intervention. 
%The proliferation of disruptive Machine Learning (ML) and especially Deep Learning (DL) algorithms %techniques %deep neural networks 
%in recent years has enabled a plethora of applications across several domains. Such techniques work on the basis of complex artificial neural networks, which are capable of effectively learning from data by means of a large number of hyper-parameters distributed in different network layers.
%%Neural networks - artificial abstraction models in the human brain - are trained using modern learning algorithms and huge datasets. The result is that speech recognition systems improve independently; cars drive autonomously based on environmental sensor information; medical applications exceed a physician's performance.
%%==============================================================================
%%thereby culminating in Deep Learning. 
%% In recent years
%%Recently, the intensive use of Recommender systems in Software Engineering has brought in benefits. 
%%Different AI techniques to deploy in Software Engineering. 
%%In Software Engineering
%In a nutshell, DL techniques are %deemed to be 
%an advanced paradigm that brings in substantial improvement in performance compared to conventional learning algorithms. %In recent years, 
%Recently, there is an increasingly number of applications of ML/DL techniques %. The deployment of Deep Learning techniques 
%to address challenging issues in Software Engineering, with the aim of improving the synergy between the two domains~\cite{10.1145/3172871.3172891,Shafiq2020MachineLF,DBLP:conf/icse/AmershiBBDGKNN019}.




%attempts to fuse 
%============================Adversarial Machine Learning in Recommender Systems============================


Even worse, online data used to train recommenders can be exploited for malicious purposes.
Adversarial Machine Learning~\cite{6015575,10.1145/2046684.2046692} (AML) is a field of study that focuses on security issues in ML systems and, specifically, in (general-purpose) recommender systems too~\cite{DDM20a}. Research has been done to identify probable threats and seek out adequate countermeasures~\cite{10.1007/978-3-030-49461-2_18,wang_adversarial_2020}.
For example, Anelli \etal~\cite{10.1007/978-3-030-49461-2_18} use shilling attack~\cite{DBLP:journals/air/SiL20} to manipulate a collaborative-filtering recommender system operated with Linked Data. Also, Wang and Han \cite{wang_adversarial_2020} propose an improvement of the Bayesian personalized ranking (BPR) technique by exploiting the adversarial training-based mean strategy (AT-MBPR) in the domain of collaborative filtering-based recommender systems.

 % to protect systems against attacks
%Adversarial Machine Learning (AML) is an emerging research topic that is a combination of the best practices in various fields, including Machine Learning, robust statistics, and computer security~\cite{DDM20a,10.1145/2046684.2046692}. %[115, 134] %Tommaso Di Noia. %Adversarial machine learning 
To defend a system against threats, in the first place, it is necessary to be knowledgeable of 
various types of adversary activities~\cite{4216981}.
Such activities generate perturbations to deceive and 
disrupt systems by causing a malfunction, compromising their 
recommendation capabilities. 
%A main way to achieve this is to feed systems with malicious data~\cite{DDM20a}.

The ultimate aim of these attacks is to manipulate target items, thus creating 
either a negative or positive influence on the final 
recommendations~\cite{10.1007/s10462-012-9364-9}, depending on the attacker's 
intention. For instance, in image classification, an attacker crafts an input 
image by adding non-random noise in a way that it will be falsely classified by 
ML models, whilst still being properly recognized by 
humans~\cite{conf/cvpr/NguyenYC15}. As an example, a panda was recognized as a 
ribbon by cutting-edge deep neural networks once the input image had been 
padded with noise, meanwhile humans still correctly perceived the panda from 
the forged image~\cite{DBLP:journals/corr/GoodfellowSS14}.



%image is still seen as the same panda 
%Adversarial examples: ML models misclassify examples that are only slightly different from correctly classified .... ~\cite{43405}.
%The learned model slightly differs from the true data distribution.
%============================Limitations of existing work===============================================================
%and how to synergically integrate machine intelligence and human intelligence (e.g., domain knowledge or insight) to effectively tackle challenging software engineering problems
AML has been studied in a wide range of domains, \eg online shopping systems~\cite{4216981} or image classification~\cite{conf/cvpr/NguyenYC15}, and addresses both  
risks and countermeasures. However, to the best of our knowledge, AML has not been investigated in the context of SE applications of ML yet.

In this paper, we report  the first study 
on threats that cause harm or danger to RSSE suggesting third-party libraries 
and API function calls. We select these two types of recommendations as they 
are representative of scenarios in which \emph{(i)}  the recommendation is 
learned from OSS repositories; and \emph{(ii)} the outcome of a malicious 
recommendation, \eg the usage of a library or an API, can result in severe 
security holes~\cite{10.1145/2976749.2978333}. 

Based on a thorough observation and by analyzing existing literature, we realized that most of the efforts to improve RSSE 
have been made to enhance their prediction accuracy. To the best of our knowledge, no work has been dedicated 
to investigate 
the problem of using intentionally falsified data to compromise recommender systems' capabilities, as well as conceptualizing the corresponding countermeasures. 
In this respect, our work is the first one that brings in the issue of AML in RSSE. 

Most RSSE 
heavily rely on open data sources, such as \GH, 
the Maven Central Repository, or Stack Overflow, 
which can be easily steered by adversaries \cite{zhang_cyber-guided_2020}. In other words, these systems are 
vulnerable to attacks equipped with forged input data.
Therefore, 
there is the need for comprehending the likely threats, with the ultimate aim of 
conceiving counteractions to increase the resilience
of RSSE.

%===================================================The aim of this paper===============================================
We first provide an overview of state-of-the-art API and third-party library recommenders, discussing  how they could be potentially affected by AML.
Through a literature search from premier venues in Software Engineering for adversarial techniques, 
we show that there are considerably evident threats to RSSE. 
Then, we perform a preliminary examination of two existing systems for recommending third-party libraries. The experimental results reveal a worrying 
outcome: by a simple manipulation, we can seamlessly spoil the final recommendations, putting software clients at risk.

The present paper makes the following contributions: 

%risk on the learning models. 
%have suggested it is due to extreme nonlinearity of deep neural networks.
%\begin{itemize}
	%\item A condensed literature review on recommender systems in Software Engineering;%applications of ML/DL in Software Engineering;
%	\item A summary of most notable RSSE to provide third-party libraries and API function calls; \MAX{I wouldn't call this a contribution, I suggest to merge this with the next, saying ``A discussion fo the possible adversarial attacks on state-of-the-art RSSE for third-party libraries and API calls''}
%\vspace{.05cm}
%\noindent
%$\rhd$~
\begin{itemize}
	%	\noindent
	\item[--] A discussion on the possible adversarial attacks to state-of-the-art RSSE for third-party libraries and API calls; 
	\item[--] A preliminary evaluation on two library recommender systems to perturb their recommendations.
\end{itemize}
%\end{itemize}

%\vspace{.05cm}
%\noindent
%$\rhd$~\emph{A review}: 
%
%\vspace{-.05cm}
%\noindent
%$\rhd$~\emph{Possible implications on the Software Engineering domain}: 

%\vspace{.05cm}
The paper is structured as follows. Section \ref{sec:Background} provides  background notions about adversarial attacks and their effects on RSSE. Section \ref{sec:ProofOfConcept} reports an initial evaluation on two RSSE, while Section~\ref{sec:Conclusion} outlines future work and concludes the paper. 


==> src/ProposedApproach2.tex <==


In the scope of this work, we limited ourselves mainly to supporting the first 
phase of the migration process, \ie inferring migration. We also propose an 
upgrade plan without proposing a direct integration of the delivered 
recommendations at the source code level. Although this can be seen as a 
limitation, we put the effort into investigating new methodologies to cope with 
the challenges stated in the previous section. The overall structure of the 
envisioned approach is depicted in Fig.~\ref{fig:approach} and consists of main 
four components, \ie \emph{Migration Tracker}, \emph{Data Extractor}, 
\emph{Graph Builder}, and \emph{Plan Calculator}. \emph{Migration Tracker} 
extracts migration information from heterogeneous data sources, \ie \GH 
repositories, Stack Overflow posts, or API documentations, to name a few. Then, 
the collected information is encoded in CSV files by means of \emph{Data 
Extractor}. Using the encoded data, \emph{Graph Builder} constructs a migration 
graph with multiple weights. Finally, \emph{Plan Calculator} delivers the 
upgrade plan by relying on an aggregation function for multiple weights and 
shortest path algorithms provided by \emph{Neo4j}. In this work, we partially 
implemented the components, in the next subsections, we describe \tool, by 
focusing on the implemented features. %of the tool.
 


% whose functionalities are explained below

\smallskip
\noindent
\emph{A. Migration Tracker:} \label{sec:tracker} In Fig.~\ref{fig:approach}, we 
could have potential heterogeneous resources to deal with in the first step. 
For instance, relevant migration data could be found in \GH repositories and 
their corresponding metadata such as issues, commits, or stars. Additionally, 
we can extract other valuable information from Stack Overflow, bug reports, and 
API documentation. Intuitively, in case of alternative upgrade plans, 
developers might prefer those that have been followed most to migrate other 
projects and for which there is the availability of related posts and 
supporting documentation that can be examined during migrations. In this paper, 
we focus on the analysis of the 
resources mined from \GH using \emph{Crawler}, a sub-component of the 
\emph{Migration Tracker} component. It downloads a list of \GH projects that 
have at least one \emph{pom.xml} file using the JGit 
library.\footnote{\url{https://www.eclipse.org/jgit/}} In case there are 
multiple \emph{pom.xml} files, they will be analyzed separately to avoid 
information loss. Then, \emph{Migration Tracker} analyzes all the repository's 
commits that affect the \emph{pom.xml} to find added and removed TPLs. 

\smallskip
\noindent
\emph{B. Data Extractor:} \label{sec:dataEx}
Once valuable data has been excerpted, \emph{Data Extractor} aggregates the 
migration data in CSV files and calculates weights according to the type of the 
root sources, as heterogeneous resources need to be considered in a different 
manner during the recommendation phase. Concerning the CSV format, each row of 
these files contains the name of the library, the corresponding version, the 
sign, and the date. In particular, the sign can be '+' or '-' in case of added 
or removed version, respectively. By exploiting such kind of data, \tool is 
able to deduce the number of clients that perform a certain migration step from 
a version to a another. The idea is to count the number of clients that made 
this migration and report it as a weight on the edges of the graph. The 
definition of the weight might also take into account the availability of 
additional material that can support the migration phase \eg 
documentation, and Stack Overflow posts.

\smallskip
\noindent
\emph{C. Graph Builder:} The \emph{Graph Builder} component creates nodes and 
relationships by considering the date and weights computed in the previous 
phase. To do this, \tool exploits the Cypher query language 
\footnote{\url{https://neo4j.com/developer/cypher-query-language/}} to store 
data into a \emph{Neo4j} graph. For instance, we extract from CSV files two 
pair library-version \emph{(l,v1)} and \emph{(l,v2)} with signs '-' and '+', 
respectively. In this way, the component creates an oriented edge from 
\emph{(l,v1)} to \emph{(l,v2)}. The date value contained in the CSV record is 
used to avoid duplicated edges or loops. Furthermore, each edge is weighted 
according to the number of clients as described in \textit{Data Extractor} 
phase.
Thus, the final outcome of %the implemented version of 
this component is a migration graph that considers the community's interests as the only weight. 

\begin{figure}[h!]
	\centering
	\vspace{-.2cm}
	\includegraphics[width=\linewidth]{figs/graph.png}
	\vspace{-.6cm}
	\caption{The \emph{slf4j} migration graph.}
	\vspace{-.5cm}
	\label{fig:graph}
\end{figure}


\smallskip
\noindent
\emph{D. Plan Calculator:} By relying on a candidate project as the input, 
\emph{Plan Calculator} analyzes \emph{pom.xml} file(s) to get TPLs' history 
used by the project. Then, it 
retrieves the upgrade plan by exploiting %two main strategies, \ie 
the aggregation function and the shortest path algorithm. The former combines 
all the possible weights belonging to the graph. The latter simply applies the 
implemented shortest path algorithm offered by Neo4j considering these weights. 
As mentioned before, we consider only the number of clients as the weight to 
minimize the number of steps to perform the proposed upgrading. Thus, the 
implemented version of \tool recommends the upgrade plan for a certain library 
by evaluating the community's decisions. To be concrete, Fig.~\ref{fig:graph} 
represents the extracted migration graph for the \emph{slf4j-api} library. 
Starting from version \emph{1.5.8}, \tool recommends a possible upgrade plan 
depicted in Fig.~\ref{fig:path}. Considering the aforementioned weights, the 
suggested steps involve upgrading to \emph{1.6.1}, \emph{1.6.4}, and 
\emph{1.7.5} to reach the final version considered in the example, \ie 
\emph{1.7.25}. For the tool the majority of developers prefer to perform such 
the upgrade plan, rather than directly update the library to the newest 
version. 

%=======
%By relying on a candidate project as the input, the \emph{Plan calculator} analyzes POM file(s) to get TPLs' history used by the project. Then, it 
%retrieves the upgrade plan by exploiting two main strategies, \ie the aggregation function and the shortest path algorithm. The former combines all the possible weights belonging to the graph. The latter simply applies the implemented shortest path algorithm offered by the Neo4j \cite{neo4j_942_2020} considering these weights. As mentioned before, we consider only the number of clients as the weight to minimize the number of steps to perform the proposed upgrading. Thus, the implemented version of \tool recommends the upgrade plan for a certain library by evaluating the community's decisions. A possible upgrade plan for \emph{slf4-api} library is depicted in Figure \ref{fig:path} while Figure \ref{fig:graph} represents the corresponding whole migration graph.

\begin{figure}[h]
	\centering
	\vspace{-.4cm}
	\includegraphics[width=\linewidth]{figs/slf4j_path.png}
	\caption{A recommended upgrade plan for \emph{slf4j}.}
	\vspace{-.4cm}
	\label{fig:path}
\end{figure}

%>>>>>>> db42d17e3d25a49b6b15af8a0b2c4191fd9e478a






==> src/RelatedWork2.tex <==
%Adversarial Machine Learning 

%==============================
%The topic of AML has garnered attention from the research community in recent years. In image classification, several adversarial techniques have been introduced to add perturbations to images~\cite{DBLP:journals/corr/GoodfellowSS14,conf/cvpr/NguyenYC15}, which are then correctly recognized by humans. However, DNNs are prone to these attacks as they fail to classify the crated images. 
%==============================
%by crafting images 
%Nguyen \etal~\cite{conf/cvpr/NguyenYC15} presents an approach to deceive DNNs %deep neural networks 
%have been %shown to be 
%, but not by cutting-edge deep neural networks (DNNs). %believe to be recognizable objects with over 99\% confidence. 
%For instance, in image classification, an attacker crafts an input image by adding noise in a way that it will not be correctly classified by ML models, while still being properly recognized by humans' eyes~\cite{conf/cvpr/NguyenYC15}.

This section describes \emph{(i)} a case of RSSE robust to AML; \emph{(ii)} applications of AML in SE; and \emph{(iii)} studies about AML attacks to recommender systems belonging to other domains.

PyART~\cite{he_pyart_2021} is a recommender system for Python developers.
It mines developers' context to suggest the next APIs to be included. PyART uses a lightweight analysis to derive an optimistic data flow and infer an element's type. If the type inference is successful, all the callable methods of the inferred type are possible API candidates. Otherwise, API candidates are extracted from libraries and all the callable methods declared in the current context. For this reason, PyART is less prone to manipulation of training data, but this comes at a price since at the same time, it is unable to recommend APIs from unseen libraries/code.


Chen \etal~\cite{chen_adversarial_2017} explored the impact of AML on malware detection and implemented two techniques to detect and defend against attacks. \textit{EvnAttack} is an evasion attack model to assess the security of classifiers, and \textit{SecDefender} is a secure-learning paradigm against evasion attacks in malware detection. Bielik and Vechev~\cite{bielik_adversarial_2020} proposed a similar approach that uses adversarial training techniques to achieve both robust and accurate models of code. %The tool was applied to predict types for two dynamically typed languages JavaScript and TypeScript. %The evaluation shows that all the 5 neural networks architectures involved in the experiment benefit from the usage of adversarial training techniques.
Shriver \etal~\cite{Shriver:ICSE:2021} explored	the use of existing adversarial attack techniques for the falsification of deep neural networks (DNN) safety properties. They transform a correctness problem into a set of robustness problems (property reduction) that employ a set of falsifiers (adversarial attacks). 
%Shriver \etal also showed that property reduction yields advantageous violations of general DNN correctness problems.
 Their work focuses on how AML can hinder a DNN correctness, and not on RSSE recommendations.

There are various studies about AML for general-purpose recommender systems~\cite{4216981,10.1007/s10462-012-9364-9}. Anelli \etal~\cite{10.1007/978-3-030-49461-2_18} introduced an attempt to use a shilling attack to manipulate a collaborative-filtering recommender system operated with linked data. However, they do not propose any concrete countermeasures to fight against this type of attack. Deldjoo \etal~\cite{10.1145/3439729} reported a comprehensive survey on recent developments on AML for the security of recommender systems. Among others, their work reviews various attacking and defense models for generic recommender systems. Such techniques could be possibly adapted to RSSE that follow the same design methodology of generic recommender systems. %We consider this our future work.

%Concerning defense techniques, various approaches have been~\cite{4216981}. 
Cao \etal~\cite{cao_adversarial_2020} proposed an attack-agnostic detection model to support recommender systems using reinforcement learning (RL). The model is based on an attention classifier that distinguishes adversarial examples from legitimate ones by measuring the probability that input data suffer from perturbations. % introduced using a constructed attack model. 
We assume that this technique can be customized to protect RSSE, as it is able not only to learn from good samples but also to learn to avoid hostile patterns.


%=======================================================
%PyART
%Each candidate is represented by a feature vector consisting of optimistic data-flow hints, the token similarity, and the token co-occurrence hints. Similarly, the feature vectors are extracted from the projects in the training corpus. The feature vectors train a Random Forest recommendation model that is used to ranks all the extracted candidates.
% It recommends APIs for Python in real-time by excerpting three kinds of features from the developer's context. These features are eventually used to feed a Random Forest predictive model.  
%PyART is less prone to the manipulation of the training data. First of all, it tries to infer the type of elements defined in the developer's context to compute the possible candidates. If the type is properly identified, the candidates are real APIs. Otherwise, PyART extracts possible candidates from imported libraries that are dynamically included from pip repositories. It makes the inject fake API as candidates difficult. Though mining projects with fake APIs can cheat the Random Forest recommendation models, it only impacts the candidates' rank. %\\ \hline
%=======================================================
%and (ii) to show another successful application of AML in generative adversarial networks (GANs) for generative applications, thanks to their ability for learning (high-dimensional) data distributions.
%In our work, we performed similar push attacks on three RSSE which work on data from \GH. %However, we need to devise our own method to curate fake projects. 
%Wang and Han~\cite{wang_adversarial_2020} propose an improvement of the Bayesian personalized ranking technique by exploiting the adversarial training-based mean strategy in the domain of collaborative filtering-based recommender systems. By exploiting user's ratings, the underpinning MBPR model extract and classify user's feedback into three categories. After, the algorithm injects adversarial perturbations in the initial training data to construct a noisy dataset. An iterative process then optimizes the objective function. 
%To defend against attacks, there have been several.

%Strathcona \cite{DBLP:conf/sigsoft/HolmesWM05}, Local repositories, Strathcona suggests relevant API usages by searching in a local code repository. It employs six different heuristics that compute the similarity at the structural level to increase the quality of the retrieved code snippets. The system uses a local repository which is automatically generated from existing source code examples. Attackers can easily inject malicious APIs into such a knowledge-base to fool the developed heuristics. 

%XSnippet~\cite{10.1145/1167473.1167508}, Eclipse projects, Relevant API snippets are retrieved by invoking different queries that consider both the parents of the class and the lexical visible type. A graph-based mining algorithm is then used to deliver the final recommendations by employing a breadth-first search algorithm. As the underpinning algorithm mines common tree paths, a poisoning attack may succeed in altering the outcomes of the system by adding similar tree branches, \ie XSnippet can be deceived with fake projects containing bad classes and methods. 

%MAPO~\cite{Zhong2009MAPO}, SourceForge, API patterns are recommended by extracting related information from developers' context using the BIDE mining algorithm~\cite{1319986}. The resulting data is clustered and ranked according to their similarity with the client code. Since BIDE~\cite{1319986} works by mining from common patterns, MAPO can be steered by malicious code inserted into projects with popular API sequences. The clustering engine also contributes to the introduction of fake code to users. %& \untick\\ \hline%\cline{2-6}



%\subsection{Robust API Recommender system}


%Shilling attacks~\cite{DBLP:journals/air/SiL20}.
%. In this paper, we show another way that DNN and human
%vision differ: 

%
%\begin{table}[]	
%	\caption{Selected research on AML for API recommender systems}
%	\label{tab:mini-SLR}
%	\begin{tabular}{|l|l|l|l|l|l|}
%		\hline
%		& \textbf{REC}                                     & \textbf{ADV}              & \textbf{ML}                & \textbf{API}              & \textbf{MAL} \\ \hline
%		\textbf{REC} & \textbf{429}                                     &                           &                            &                           &              \\ \hline
%		\textbf{ADV} & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0} & \textbf{45}               &                            &                           &              \\ \hline
%		\textbf{ML}  & \cellcolor[HTML]{009901}27                       & \cellcolor[HTML]{036400}5 & \textbf{311}               &                           &              \\ \hline
%		\textbf{API} & \cellcolor[HTML]{009901}45                       & \cellcolor[HTML]{036400}2 & \cellcolor[HTML]{009901}27 & \textbf{323}              &              \\ \hline
%		\textbf{MAL} & \cellcolor[HTML]{FFCCC9}0                        & 1                         & \cellcolor[HTML]{009901}7  & \cellcolor[HTML]{009901}9 & \textbf{80}  \\ \hline
%	\end{tabular}
%
%\end{table}


==> src/Results2.tex <==


%\vspace{-.3cm}

%\subsection{Result analysis}

%In the following, w
%We answer \textbf{RQ$_1$} (Section~\ref{sec:RQ1})  by means of qualitative analyses on the existing literature. Then, we answer \textbf{RQ$_2$} (Section~\ref{sec:RQ2}) by analyzing  
%the results obtained from the empirical experiments.% on the datasets described in Section~\ref{sec:Settings}. 

This section reports the study results, addressing the research questions formulated in Section~\ref{sec:Evaluation}.

\subsection{\rqfirst} \label{sec:RQ1}

%A mini literature survey

%\JDR{this paragraph has to be restructured}We selected three of them however they are about detecting malware application or code as a security issue rather than malicious API in the code. three papers refer to the identification of malware in android applications by ml approaches, one refers to code plagiarism, and the last one refers to the detection of malicious software by analyzing the behavioral artifacts. 
%\vspace{.1cm}
%\begin{shadedbox}
%	\small{\textbf{Observation 2.} The issue of adversarial attacks to API recommender systems has not been adequately studied so far.}
%\end{shadedbox}
%%\vspace{-.4cm}



%Fig.~\ref{fig:BubbleChart} lists 


% (see Section~\ref{sec:Collection}). In total, the final corpus .
%\begin{table}[h!]
%	\centering
%	\vspace{-.3cm}
%	\footnotesize
%	%	\scriptsize	
%	\caption{Number of papers emerging from premier SE venues in the most five recent years (2016 -- 2020).}
%	\begin{tabular}{| p{0.2cm}|l | p{0.8cm} | p{0.8cm} | p{0.8cm} | p{0.8cm} | p{0.8cm} |} \hline
%		{\multirow{2}{*}{}}	&	{\multirow{2}{*}{\textbf{Venue}}}	& \multicolumn{5}{c|}{\textbf{Year}} \\  \cline{3-7} 
%		&  & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020}  \\ \hline
%		{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Conferences}}}} & ICSE & 101 & 67 & 153 & 109 & 129 \\ \cline{2-7} %WRCE\footnote{WRCE was the former edition of SANER}
%		& ESEC/FSE & 146 & 81 & 117 & 77 & 169 \\ \cline{2-7}
%		& ASE & 112 & 116 & 109 & 154 &  159\\ \cline{2-7}
%		& ICSME & 79 & 79 & 88 & 95 & 108 \\ \cline{2-7}
%		%		\rowcolor{verylightgray}
%		& ICST &  49 & 74 & 70 & 56 & 81 \\ \cline{2-7}
%		& ISSTA & 44 &  57 & 40  & 55  & 57  \\ \cline{2-7}
%		%		& MSR &  &  &  &  & 77  \\ \cline{2-7}
%		& ESEM & 145 & 165 & 187 & 195 & 188 \\ \cline{2-7}
%		& MSR & 61 & 67 & 79 & 81 & 77 \\ \cline{2-7}
%		& SANER & 19 & 83 & 77 & 72 & 79 \\ \hline
%		{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Journals}}}} & TSE & 62 & 57 & 73 & 119 & 112 \\ \cline{2-7} %WRCE\footnote{WRCE was the former edition of SANER}
%		& TOSEM & 18 & 12 & 26 & 28 & 32 \\ \cline{2-7}
%		& EMSE & 145 & 165 & 187 & 195 & 188 \\ \cline{2-7}
%		& JSS & 256 & 238 & 259 &222  & 217 \\ \cline{2-7}
%		%		\rowcolor{verylightgray}
%		& IST & 125 & 110 & 172 & 170 & 122 \\ \hline
%	\end{tabular}
%	\vspace{-.2cm}
%	\label{tab:LiteratureReview}
%\end{table}

%\begin{figure}[h!]
%	\centering
%	\vspace{-.2cm}
%	\includegraphics[width=0.88\linewidth]{figs/BubbleChart3.png}
%	\vspace{-.3cm}
%	\caption{Number of papers from premier SE venues from 2016 to 2020.} %Summary of the main words
%	\label{fig:BubbleChart}
%	\vspace{-.2cm}
%\end{figure}

%\MAX{IMHO the following paragraph can be dropped, we don't want to discuss the conferences/journals healthiness}
%Top-tier conferences such as ICSE or ESEC/FSE normally attract a large number of submissions and thus, they also have more articles, ranging from 67 papers with ICSE in 2017 to 169 papers with ESEC/FSE in 2020, though the acceptance rate is low, \ie generally below 20\%.\footnote{\url{https://dl.acm.org/doi/proceedings/10.5555/3339505}} 
%ranging from 67 papers with ICSE in 2017 to 169 papers. Other conferences such as ICST, MSR, ESEM, or SANER have less, \ie in average around 80 papers for one edition. 
%\eg larger for JSS and ICSE, smaller for others. 

%, as they receive more submissions, \ie more than one thousand of papers every year, even though the acceptance rate is also lower than 20\%.\footnote{\url{https://bit.ly/2PHXiTn}}


Following the process in Section~\ref{sec:Collection}, we collected a corpus consisting of \numPapers documents coming from the considered conferences and journals in the five most recent years, \ie from 2016 to 2020. By inspecting the corpus, we see that the number of papers varies among different venues, ranging from less than 20 to around 250 papers. 
%Concerning conferences, while some venues have more than a hundred, the others have less than 80 articles in one edition. Similarly, journals such as TSE or TOSEM also feature a small quantity of papers, annually. Only by JSS, we see a significant number of accepted papers, \ie more than 200 by all the considered years.

% shown in Table~\ref{tab:keywords}

%In particular, we are interested in studies about recommender systems (REC) and the related topics, \ie adversarial Machine Learning (ADV, ML), API mining (API), and malicious attempts (MAL).
%From the resulting collection,
%' 

%
%\begin{table}[h!]
%	\vspace{-.2cm}
%%	\footnotesize
%	\scriptsize
%	\caption{Keywords.}
%	\vspace{-.2cm}
%	\begin{tabular}{|l|p{6.6cm}|} \hline
%		\textbf{Acronym} & \textbf{Set of terms} \\ \hline
%		REC & recommendation, recommender, recommendation systems \\ \hline
%		API & API \\ \hline
%		ADV & AML, adversarial \\ \hline%\cline{2-2} 
%%		& AML  \\ \hline
%		ML & ML, Machine Learning, machine learning \\ \hline%\cline{2-2} , machine-learning
%%		& ML  \\ \hline
%		MAL & Malicious, malicious \\ \hline
%	\end{tabular}
%	\label{tab:keywords}
%	\vspace{-.2cm}
%\end{table}




\begin{table}[h!]
	\footnotesize
	\caption{Keywords}
	\begin{tabular}{|l|p{4.8cm}|c|} \hline
		\textbf{Acronym} & \textbf{Set of terms} & \textbf{Case-sensitive} \\ \hline
		REC & recommendation, recommender, recommendation systems & \untick \\ \hline
		API & API & \tick \\ \hline
		\multirow{2}{*}{ADV} & adversarial & \untick \\ \cline{2-3} 
		& AML & \tick \\ \hline
		\multirow{2}{*}{ML} & machine learning, machine-learning & \untick \\ \cline{2-3}
		& ML & \tick \\ \hline
		MAL & malicious & \untick \\ \hline
	\end{tabular}
	\label{tab:keywords}
\end{table}


We are interested in studies about recommender systems and the related topics, \ie Adversarial Machine Learning, API mining, and malicious attempts. From the collected corpus we narrowed down the scope by using five sets of keywords as shown in Table~\ref{tab:keywords}. For instance, for the REC set, there are the following keywords: ``\emph{recommendation},'' ``\emph{recommender},'' or ``\emph{recommender systems},'' which are popular terms used to refer to a system for providing recommendations. %\emph{(ii)} API: ``\emph{API},'' \emph{(iii)} ADV: ``\emph{AML},'' ``\emph{adversarial},'' \emph{(iv)} ML: ``\emph{ML},'' ``\emph{Machine Learning},'' ``\emph{machine learning},'' and \emph{(v)} MAL: ``\emph{Malicious},'' ``\emph{malicious}.'


\begin{figure}[h!]
	\centering
	\vspace{-.6cm}
	\includegraphics[width=0.680\linewidth]{figs/LiteratureSummary.pdf}
%	\vspace{-.3cm}
	\caption{Number of papers for the related topics.} %Summary of the main words
	\label{fig:mini-SLR}
	\vspace{-.1cm}
\end{figure}

Fig.~\ref{fig:mini-SLR} depicts a matrix whose each cell reports the number of papers that contain both the keywords in the corresponding column and row. Since it is a symmetric matrix, we list the numbers on the lower left part and leave the upper right part blank, for the sake of clarity. 
%We got 506 papers related to the keyword set REC, 33 papers with ML, and 82 articles with MAL. We discarded all these papers as they are not closely related to the topics of interest.
%
%\begin{table}[h!]	
%	\footnotesize
%	\caption{Selected research on AML for API recommender systems}
%	\begin{tabular}{|l|l|l|l|l|l|}
%		\hline
%		& \textbf{REC}                                     & \textbf{ADV}              & \textbf{ML}                & \textbf{API}              & \textbf{MAL} \\ \hline
%		\textbf{REC} & \textbf{429}                                     &                           &                            &                           &              \\ \hline
%		\textbf{ADV} & \cellcolor[HTML]{FFCCC9}{\color[HTML]{000000} 0} & \textbf{45}               &                            &                           &              \\ \hline
%		\textbf{ML}  & \cellcolor[HTML]{009901}27                       & \cellcolor[HTML]{036400}5 & \textbf{311}               &                           &              \\ \hline
%		\textbf{API} & \cellcolor[HTML]{009901}45                       & \cellcolor[HTML]{036400}2 & \cellcolor[HTML]{009901}27 & \textbf{323}              &              \\ \hline
%		\textbf{MAL} & \cellcolor[HTML]{FFCCC9}0                        & 1                         & \cellcolor[HTML]{036400}7  & \cellcolor[HTML]{009901}8 & \textbf{80}  \\ \hline
%	\end{tabular}
% 	\label{tab:mini-SLR}
%\end{table}
%
%the scope of our study. 
%It is also worth noting that no forward snowballing steps are required since no papers fits the mini.
%There are two papers which contain both ``\emph{API}'' and ``\emph{adversarial}.'' 
%\revised{Then, we collect the papers that use at least two of the selected terms. Fig.~\ref{fig:mini-SLR} shows the results of our queries: in the diagonal, we report the number of papers that match with one term (\eg we collected 429 papers including \textit{REC} term-set) while the other cells show the number of papers that contain column and row term-sets together.}
%
%In Fig.~\ref{fig:mini-SLR}, we highlight with different colours (\ie dark green, green and pink) the cells. The dark green cells report the closest term-sets to our scopes, the green ones count the papers that can be related to the topics of this paper, while the pink ones are strictly close to the survey that we are conducting. It is worth noting that the pink cells count 0 papers that match our term-sets intersection.%For instance, articles like the one proposed by Gao \etal~\cite{10.1145/3368089.3409745} have been discarded because they are very unrelated to our study. In particular, such a paper studies the}
%In the rest of this section, we are interested in the papers in the green cells. 
%
Our search targets papers containing one of the following five combinations: either \emph{(i)} REC and ADV; or \emph{(ii)} ADV and ML; or \emph{(iii)} ADV and API; or \emph{(iv)} REC and MAL; or \emph{(v)} API and MAL. %\MAX{make sure the previous thing is already said in the design}
We mark the associated cells using the green color, and carefully examine these papers. None of them matches with both sets of keywords REC and ADV, or REC and MAL. %, \ie the corresponding cells are 0. 
For the combinations REC and ML, ADV and API, API and MAL, we found six, three, and nine articles, respectively. By reading the abstract, we filtered out the ones being completely out of our interest. We ended up with only seven %relevant 
papers~\cite{bao_mining_2018,garcia_lightweight_2018,koch_semi-automated_2017,lee_adlib_2019,narayanan_multi-view_2018,singh_detection_2020,wu_effective_2016}, discussed as follows.

Most of the resulting studies investigate API-based malware detection in the context of Android applications. For instance, Wu \etal \cite{wu_effective_2016} proposed an approach that relies on dataflow-related API-level features to detect malicious samples. 
Similarly, \textsc{RevealDroid} \cite{garcia_lightweight_2018} exploits a scalable, light-weight classification and regression tree classifiers (CART) to discover Android malware. API features are extracted directly from source code, \ie by mining security-sensitive API calls. \textsc{MKLDroid}~\cite{narayanan_multi-view_2018} is a framework for detecting malware and malicious code localization, and it integrates different semantic perspectives of apps, \eg security-sensitive APIs, system calls, control-flow structures, information flows, in conjunction with ML classifiers. A recent work~\cite{lee_adlib_2019} analyzes vulnerabilities caused by the usage of advertising platform SDKs. Moreover, a static analysis tool named \textsc{Adlib} has been developed to analyze advertising platform SDKs and detect vulnerable patterns that can be abused by advertisements. Bao \etal \cite{bao_mining_2018} proposed a study for detecting malicious behavior of malware that infects benign apps by mining sandboxes. 

%\begin{figure}[t!]
%	\centering
%	\vspace{-.3cm}
%	\includegraphics[width=0.99\linewidth]{figs/Wordcloud2.png}
%	\vspace{-.3cm}
%	\caption{Word cloud for the set of collected papers.} %Summary of the main words
%	\label{fig:Wordcloud}
%	\vspace{-.3cm}
%\end{figure}

%In a more general context, 
Singh \etal~\cite{singh_detection_2020} proposed an approach to detection of behavior-based malware. Cuckoo sandboxes are inspected to extract three different primary features. After dedicated preprocessing steps, \eg NLP, or decomposition, all the resulting features are integrated in the training set to develop malware classifiers using different machine learning algorithms, \eg Random Forest, Decision Tree, or Support Vector Machines. %, K-Nearest Neighbors, Na\"{i}ve Bayes, Gradient Boosting, and ADA Boosting. 
Being conceived to automatically identify Server-based InFormation OvershariNg (SIFON) vulnerabilities, the Hush tool \cite{koch_semi-automated_2017} employs a heuristic to analyze sensitive information excerpted from server-side mobile APIs. As a preliminary study, the system makes use of static program analysis to discover potential software vulnerabilities in the analyzed applications.

In summary, by thoroughly investigating the papers that match the keywords used to filter out irrelevant studies, we realize that all of them deal with malware detection in Android apps. Instead, we did not find any work related to potential threats and implications of adversarial attacks to API RSSE.%recommender systems.
%RSSE in general, and 
% in particular.



%=============================================
%Eventually, we depict in Fig.~\ref{fig:Wordcloud} the word cloud populated from the original corpus with 6,402 documents using their titles and abstracts. Such a diagram shows the frequency of occurrence of a word, \ie the more it appears in the text, the bigger it is depicted in the cloud. From the figure, it is evident that ``\emph{software}'' and ``\emph{code}'' are the most frequent terms in the corpus. Moreover, ``\emph{developers}'' and ``\emph{test}'' are also among the most popular terms. However, we do not see terms such as ``\emph{recommender}'' or ``\emph{adversarial}'' in the cloud.
%=============================================





\vspace{.1cm}
\begin{shadedbox}
	\textbf{Answer to RQ$_1$.} So far, the issue of adversarial attacks to APIs and code snippet recommenders has not been adequately studied in major software engineering venues.
\end{shadedbox}



\input{src/APIRecSys}

\subsection{\rqsecond} \label{sec:RQ2}

We answer \textbf{RQ$_2$} by discussing a qualitative analysis of existing API recommender systems, and by presenting the results of the empirical evaluation, which has been performed by analyzing notable RSSE for mining APIs and code snippets.

\smallskip
\subsubsection{Qualitative analysis}\label{sec:rq2_qualitative_analysis}

From the premier software engineering venues considered in \textbf{RQ$_1$} we selected work presenting techniques and tools recommending APIs and code snippets. Table~\ref{tab:summary} lists in chronological order the set of analyzed approaches. 
%
% that match with two sets of keywords, \ie REC and API, we carefully read and selected RSSE that support the development of software projects by delivering API calls and/or snippets. We also searched earlier venues for additional tools being considered to be among the first and thus, the most influential API recommender systems. Eventually, we included two more tools, namely 
%Strathcona \cite{DBLP:conf/sigsoft/HolmesWM05}, 
%XSnippet~\cite{10.1145/1167473.1167508}, 
%MAPO~\cite{Zhong2009MAPO}, 
%\UM~\cite{Wang2013Mining} and MUSE~\cite{Moreno:2015:IUT:2818754.2818860}. Table~\ref{tab:summary} lists in chronological order, and analyzes the set consisting of 9 API/snippet RSSE.
%
For each system, %in Table~\ref{tab:summary}, %we report the publication (\textbf{Venue}) and the (\textbf{Year}). 
by studying the used approach (\textbf{Working mechanism} column), we discuss its possible vulnerabilities  (\textbf{Poten\-tial risks} column). 
The last column, namely \textbf{Avail.}, specifies the availab\-ility of the replication package by each tool, \ie either available (\tick) or not available (\untick).

Besides what is reported in the \textbf{Potential risks} column of Table~\ref{tab:summary}, this section summarizes their main charact\-eristics to highlight the risk of being exploited. Two features that make a system vulnerable to malicious attempts are namely \emph{(i)} relying on data from the open-source for training, \eg \GH or Android markets; and \emph{(ii)} the application of a similarity measure (marked with \circledb{S}) or a clustering technique (marked with \circled{C}) to recommend APIs or code, as we detail below. 



\begin{itemize}
	\item All the systems leverage public data sources to function. While in principle RSSE can also be trained on closed-source, trusted repositories, in all those cases a realistic, broad learning makes it unavoidable to leverage large, open-source forges.
	 Most of the considered RSSE are trained with repositories from \GH, Maven, or the Microsoft Code Base, including %MAPO~\cite{Zhong2009MAPO}, 
	\UM~\cite{Wang2013Mining}, DeepAPI~\cite{Gu2016DeepAPI}, PAM \cite{Fowkes:2016:PPA:2950290.2950319}, \textsc{fine-GRAPE}~\cite{sawant_fine-grape_2017}, AuSearch \cite{DBLP:conf/wcre/AsyrofiT0J20}. Since these sources are freely open for changes by the crowd, they are also exposed to malicious purposes. Other systems supporting Android apps, such as SALAD \cite{DBLP:conf/icse/NguyenPVN16} or \FC~\cite{9359479} normally obtain data from Google Play, which enforces mechanisms to control submissions. Nevertheless, such a platform is not immune from manipulation, as this has been previously reported~\cite{7403546}.
	\item Most of the approaches are based on a similarity measure/kernel to mine APIs and/or code snippets. In this way, an adversary can insert malicious APIs into similar projects, and pose them as legitimate to trick the systems into using the disguised project and eventually recommendi\-ng API calls. In particular, the following systems work on the basis of a similarity algorithm: %Strathcona \cite{DBLP:conf/sigsoft/HolmesWM05}, XSnippet \cite{10.1145/1167473.1167508}, 
	MUSE~\cite{Moreno:2015:IUT:2818754.2818860}, \textsc{fine-GRAPE}~\cite{sawant_fine-grape_2017}, \FC~\cite{9359479,Nguyen:2019:FRS:3339505.3339636}, and CodeKernel \cite{DBLP:conf/kbse/Gu0019}. %Two other systems, \ie MAPO~\cite{Zhong2009MAPO} and 
	\UM~\cite{Wang2013Mining} is not directly based on similarity, however, it relies on the BIDE algorithm~\cite{1319986}, which works by mining from common patterns. Thus, it is prone to malicious code concealed in popular sequences. 
	\item Similarly, the other systems that work on clustering techniq\-ues are also susceptible to adversarial attacks. In fact, besides the BIDE algorithm~\cite{1319986}, MAPO and \UM additionally employ clustering to group similar code sequences. In this way, attackers may populate fake projects to favor a particul\-ar code pattern containing malicious APIs. 
	Lastly, approach\-es like \textsc{fine-GRAPE} are prone to manipulations forging an artificial history of API calls in \GH projects.
\end{itemize}


%. the system can be fooled with malicious code intentionally inserted
%Thus, they are exposed to perturbations with malicious content hidden in OSS projects. We therefore conjecture that, by fabricating projects with bogus data, attackers can favor (push attack) or defame (nuke attack) a library~\cite{10.1007/978-3-030-49461-2_18,DBLP:journals/air/SiL20,DDM20a}.

Altogether, it is evident that all the systems in Table~\ref{tab:summary} are potentially exposed to push attacks. 
%In other words, 
They can be manipulated to favor a malicious API or	 snippet, so that it will be suggested by the recommendation engine. As such, the systems in which the recommended code is embedded will suffer. 

 
%
%\vspace{.1cm}
%\begin{shadedbox}
%	\footnotesize{\textbf{Answer to RQ$_2$.} The analysis shows that malicious training data can pose a prominent threat to the resilience of state-of-the-art RSSE which, as a consequence, could recommend malicious APIs or code snippets.}
%\end{shadedbox}
%
%\subsection{\rqthird} \label{sec:RQ3}

%\smallskip
\subsubsection{Empirical evaluation}\label{sec:rq2_empirical_evalutation}

To quantitatively investigate the extent to which the threats outlined in the previous qualitative analysis can actually occur, we perform an empirical evaluation on three among the systems in Table~\ref{tab:summary}, \ie \UM~\cite{Wang2013Mining}, PAM~\cite{Fowkes:2016:PPA:2950290.2950319}, and \FC~\cite{Nguyen:2019:FRS:3339505.3339636} using the collected dataset (see Section~\ref{sec:rq2-design}).

We selected these tools due to the following reasons. \emph{First}, \UM is a well-established recommender system, which has shown to outperform \MP~\cite{Zhong2009MAPO}, one of the first systems for suggesting APIs. PAM has been proven to be more effective compared to MAPO and \UM~\cite{Fowkes:2016:PPA:2950290.2950319}. Meanwhile, \FC is the most recent approach and it obtains the best prediction performance if compared to both \UM and PAM~\cite{9359479}. \emph{Second}, the considered systems are also representative in terms of working mechanism (see Table \ref{tab:summary}).  \UM works based on clustering, while PAM mines API patterns that commonly appear in different snippets, and finally \FC exploits a collaborative-filtering technique, \ie also based on a similarity algorithm, to retrieve APIs from similar projects. In this respect, we conjecture that an evaluation on the three systems could be generalizable to the remaining ones in Table~\ref{tab:summary}. \emph{Third}, 
the three tools have evaluation replication package available, \ie being specified with (\tick) in the \textbf{Avail.} column of Table~\ref{tab:summary}. Such implementations enable us to run the experiments according to our needs.

The number of ranked items $N$ is %considered as 
internal, \ie it can be customized by developers. In contrast, $\alpha$,  $\beta$, and $\Omega$ are external since they can be tuned by adversaries to make their attacks more effective. The increase of $\alpha$, $\beta$, and $\Omega$ is related to the extent to which attackers add fake APIs to more projects. In the evaluation, we experiment with different configurations by varying these parameters to analyze which settings bring more perturbed outcomes.
%, if they are inclined. \MAX{what does it mean ``if they are inclined''?}

%We experiment with the following sets of parameters: $\alpha$=$\{5\%,\-10\%,15\%,20\%\}$, $\beta$=$\{40\%,50\%,60\%\}$, $\Omega$=$\{1,2\}$. The rationale behind the selection of these values is as follows. Concerning the ratio of infected projects, though having popular APIs is commonplace (see Section~\ref{sec:Settings}), it is difficult to curate a large number of projects with malicious APIs, thus $\alpha$ is set to the following thresholds $\alpha$=$\{5\%,\-10\%,15\%,20\%\}$. In contrast, within a project, attackers have more freedom to embed APIs to declarations, therefore we vary $\beta$ from 40\%, 50\%, and to 60\%. Finally, as we explained in Section~\ref{sec:Example}, the number of fake APIs $\Omega$ should be kept low to make attacks more feasible,  
%\ie $\Omega$=$\{1,2\}$. We study how the calibration of the parameters affects the final efficiency, aiming to anticipate the extent to which the attacks are successful in the field. 
%
%\MAX{I'm wondering whether the text up to here shouldn't go in the design. On the one hand, I understand, because this concerns systems which we discovered based on the RQ2 analysis. On the other hand here we mix design and result, but maybe in this case is fine.}
%



\begin{table}[t!]
	\centering
%	\vspace{-.2cm}
	\scriptsize
	\caption{Hit ratio for the recommendations by \UM.}
%	\vspace{-.2cm}
	\begin{tabular}{|p{0.15cm}|p{0.75cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|}
		%	\begin{tabular}{|p{0.2cm}|p{0.8cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|}
		\hline
		%		& & \multicolumn{10}{c|}{\textbf{FOCUS}} & \multicolumn{10}{c|}{\textbf{\CR}} \\  \hline 		
		& & \multicolumn{4}{c|}{\textbf{$\Omega$=1}} & \multicolumn{4}{c|}{\textbf{$\Omega$=2}}  \\ \hline %\hline		
		%		& & \textbf{$\alpha$=10\%} & \textbf{$\alpha$=20\%} & \textbf{$\alpha$=30\%} & \textbf{$\alpha$=40\%} & \textbf{$\beta$=10\%} & \textbf{$\beta$=20\%} & \textbf{$\beta$=30\%} & \textbf{$\beta$=40\%}  \\ \hline %\hline		
		& $\alpha$ & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} \\ \hline %\hline		
		%		& & \multicolumn{10}{c|}{\textbf{$\alpha=5\%$}} \\  \hline 
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=40\%$}}} & 
		\textbf{HR@5} & 0.078 & 0.141 & 0.200 & 0.262 & 0.005 & 0.094  & 0.021 & 0.032    \\ \cline{2-10}
		& \textbf{HR@10} & 0.088 & 0.179 & 0.252 & 0.336  & 0.031 & 0.518 & 0.073 & 0.110  \\ \cline{2-10}
		& \textbf{HR@15} & 0.119 & 0.221 & 0.313 & 0.397 & 0.072 & 0.990 & 0.139  & 0.192   \\ \cline{2-10}
		& \textbf{HR@20} & 0.119 & 0.226 & 0.317 & 0.401 & 0.104 & 0.169 & 0.247  & 0.327  \\ \hline
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=50\%$}}} &
		 \textbf{HR@5}  & 0.098 &  0.169 & 0.213 & 0.266 & 0.000 & 0.047 & 0.017  & 0.032 \\ \cline{2-10}
		& \textbf{HR@10} & 0.114 &  0.188  &  0.256  & 0.331 & 0.031 & 0.424 & 0.065 & 0.106 \\ \cline{2-10}
		& \textbf{HR@15} & 0.130 &  0.235 & 0.326 & 0.409 & 0.083 & 0.115  &  0.156 & 0.209  \\ \cline{2-10}
		& \textbf{HR@20} & 0.130 & 0.235 & 0.326 &  0.409 & 0.109 & 0.193 & 0.273  & 0.336  \\ \hline
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=60\%$}}} &
		 \textbf{HR@5} & 0.093 & 0.174 & 0.239 & 0.295  & 0.015 & 0.014  & 0.021  & 0.028   \\ \cline{2-10}
		& \textbf{HR@10} & 0.193 & 0.356 & 0.282 & 0.356 & 0.041 & 0.056 & 0.065  & 0.102   \\ \cline{2-10}
		& \textbf{HR@15} & 0.231 & 0.401 & 0.321 & 0.401 & 0.078 & 0.127 & 0.147 & 0.196   \\ \cline{2-10}
		& \textbf{HR@20} & 0.235 & 0.409 & 0.326 & \textbf{0.409} & 0.098 & 0.193 & 0.265 & 0.331    \\ \hline
	\end{tabular}
	\label{tab:ResultsUPMiner}
	%	\vspace{-.2cm}
\end{table}

\begin{table}[t!]
	\centering
	%	\vspace{-.2cm}
	%	\footnotesize
	\scriptsize
	\caption{Hit ratio for the recommendations by PAM.}
	%	\vspace{-.2cm}
	\begin{tabular}{|p{0.15cm}|p{0.75cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|}
		%	\begin{tabular}{|p{0.2cm}|p{0.8cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|p{0.62cm}|}
		\hline
		%		& & \multicolumn{10}{c|}{\textbf{FOCUS}} & \multicolumn{10}{c|}{\textbf{\CR}} \\  \hline 		
		& & \multicolumn{4}{c|}{\textbf{$\Omega$=1}} & \multicolumn{4}{c|}{\textbf{$\Omega$=2}} \\ \hline %\hline		
		%		& & \textbf{$\alpha$=10\%} & \textbf{$\alpha$=20\%} & \textbf{$\alpha$=30\%} & \textbf{$\alpha$=40\%} & \textbf{$\beta$=10\%} & \textbf{$\beta$=20\%} & \textbf{$\beta$=30\%} & \textbf{$\beta$=40\%}  \\ \hline %\hline		
		& $\alpha$ & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} \\ \hline %\hline		
		%		& & \multicolumn{10}{c|}{\textbf{$\alpha=5\%$}} \\  \hline 
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=40\%$}}} &
		\textbf{HR@5} & 0.048 & 0.098 & 0.148 & 0.198 & 0.044 & 0.090  & 0.140 & 0.198  \\ \cline{2-10}
		& \textbf{HR@10} & 0.050 & 0.100 & 0.150 & 0.200  & 0.048 & 0.098 & 0.148  & 0.198  \\ \cline{2-10}
		& \textbf{HR@15} & 0.050 & 0.100 & 0.150 & 0.200 & 0.050 & 0.100 & 0.150  & 0.200 \\ \cline{2-10}
		& \textbf{HR@20} & 0.050 & 0.100 & 0.150 & 0.200 & 0.050 & 0.100 & 0.150  & 0.200 \\ \hline
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=50\%$}}} &
		\textbf{HR@5}  & 0.048 &  0.098 & 0.148 & 0.198 & 0.048 & 0.098 & 0.148  & 0.198   \\ \cline{2-10}
		& \textbf{HR@10} & 0.500 & 0.100 & 0.150 & 0.200 & 0.048 & 0.098 & 0.148 & 0.198 \\ \cline{2-10}
		& \textbf{HR@15} & 0.500 & 0.100 & 0.150 & 0.200 & 0.050 & 0.100  &  0.150 & 0.200  \\ \cline{2-10}
		& \textbf{HR@20} & 0.050 & 0.100 & 0.150 & 0.200 & 0.050 & 0.100 & 0.150  & 0.200  \\ \hline
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=60\%$}}} &
		\textbf{HR@5} & 0.048 & 0.098 & 0.148 & 0.198  & 0.048 & 0.096  & 0.146  & 0.196  \\ \cline{2-10}
		& \textbf{HR@10} & 0.050  & 0.100 & 0.150 & 0.200 & 0.048 & 0.098 & 0.148  & 0.198\\ \cline{2-10}
		& \textbf{HR@15} & 0.050 & 0.100 & 0.150 & 0.200 & 0.050 & 0.100 & 0.150  & 0.200   \\ \cline{2-10}
		& \textbf{HR@20} & 0.050 & 0.100 & 0.150 & 0.200 & 0.050 & 0.100 & 0.150 & \textbf{0.200}  \\ \hline
	\end{tabular}
	\label{tab:ResultsPAM}
	\vspace{-.2cm}
\end{table}


\begin{table}[t!]
	\centering
	%	\vspace{-.2cm}
	\scriptsize
	\caption{Hit ratio for the recommendations by \FC.}
	\label{tab:ResultsFOCUS}
	%	\vspace{-.2cm}
	\begin{tabular}{|p{0.15cm}|p{0.75cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|p{0.45cm}|}
		\hline
		%		& & \multicolumn{10}{c|}{\textbf{FOCUS}} & \multicolumn{10}{c|}{\textbf{\CR}} \\  \hline 		
		& & \multicolumn{4}{c|}{\textbf{$\Omega$=1}} & \multicolumn{4}{c|}{\textbf{$\Omega$=2}} \\ \hline %\hline		
		& $\alpha$ & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} \\ \hline %\hline		
		%		& & \multicolumn{10}{c|}{\textbf{$\alpha=5\%$}} \\  \hline 
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=40\%$}}} & \textbf{HR@5} & 0.012 & 0.021 & 0.028 & 0.039 & 0.009 & 0.025 & 0.034 & 0.034 \\ \cline{2-10}
		& \textbf{HR@10} & 0.029 & 0.053 & 0.078 & 0.115 & 0.026 & 0.055 & 0.087 & 0.106 \\ \cline{2-10}
		& \textbf{HR@15} & 0.032 & 0.068 & 0.101 & 0.145 & 0.031  & 0.070 & 0.106 & 0.141 \\ \cline{2-10}
		& \textbf{HR@20} & 0.038 & 0.081 & 0.119 & 0.173 & 0.037 & 0.083 & 0.119 & 0.168 \\ \hline
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=50\%$}}} & \textbf{HR@5} & 0.014 & 0.036 & 0.050  & 0.067 & 0.017	 & 0.036 & 0.048 & 0.063 \\ \cline{2-10}
		& \textbf{HR@10} & 0.033 & 0.073 & 0.105  & 0.140 & 0.033 & 0.073 & 0.105 & 0.139 \\ \cline{2-10}
		& \textbf{HR@15} & 0.040 & 0.081 & 0.126 & 0.164 & 0.038 & 0.083 & 0.123 & 0.164 \\ \cline{2-10}
		& \textbf{HR@20} & 0.046 & 0.089 & 0.138 & 0.192 & 0.044 & 0.090 & 0.136 & 0.181 \\ \hline
		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\beta=60\%$}}} & \textbf{HR@5} & 0.023 & 0.051 & 0.072 & 0.028 & 0.094 & 0.047 & 0.070 & 0.097 \\ \cline{2-10}
		& \textbf{HR@10} & 0.040 & 0.083 & 0.123 & 0.171 & 0.038  & 0.080 & 0.120 & 0.160  \\ \cline{2-10}
		& \textbf{HR@15} & 0.045 & 0.093 & 0.138 & 0.190 & 0.041 & 0.088 & 0.131 & 0.173  \\ \cline{2-10}
		& \textbf{HR@20} & 0.048 & 0.099 & 0.149 & \textbf{0.203} & 0.047 & 0.096 & 0.139 & 0.185  \\ \hline
	\end{tabular}
	
	\vspace{-.2cm}
\end{table}


Table \ref{tab:ResultsUPMiner} shows the hit ratio HR@N obtained by the recommendati\-on results of \UM. It is evident that the system is considerably affected by the crafted training data, \ie it recommends the fake APIs to several projects, depending on the input parameters $\alpha$, $\beta$, and $\Omega$. Even with a small ratio of infected projects \eg $\alpha$=$5\%$, \UM recommends the artificial APIs to hundreds of projects. For instance, considering $\Omega$=1, the hit ratio HR@5 is $0.078$ and it increases to $0.119$ when N=20. When the fake API is injected to more declarations (increasing $\beta$), the hit ratio gradually improves: given that $\alpha$=20\%, $\beta$=40\%, we get HR@5=0.262, while with $\beta$=60\% HR@5 is $0.295$. The same trend can be seen with other values of $\alpha$ and $\beta$.  The hit ratio is proportional to $\alpha$ -- the ratio of infected projects. In particular, the attacks become most successful when $\alpha$=20\% and $\beta$=60\%, \ie HR@20=0.409. Given that $\Omega$=2, we obtain a comparable outcome to that with $\Omega$=1. To summarize, we conclude that \emph{\UM is prone to adversarial attacks since it suggests malicious APIs to developers.} 

%\MAX{something also from the ICSE NIER comments: does it make sense to show and discuss very high values of alpha?}

%We notice that increasing the number of projects injected with fake APIs leads to higher hit ratio values. In particular, the maximum value is reached with $\beta$ = 60 and $\alpha$ = 40 for each cut-off value \ie $N$=$\{5,10,15,20\}$. Such results are achieved by injecting only one fake API. In contrast, adding an additional malicious API decrease all the reported values even though they demonstrate that the system is still prone to malicious attacks. Generally speaking, more recommendations increase the probability to encounter a fake API in the outcomes. 




%\emph{We conclude that even with a simple fabrication, the resilience of both 
%\LR and \CR is considerably compromised.}

%\begin{table*}[t!]
%	\centering
%	\vspace{-.2cm}
%	\footnotesize
%	\caption{Hit ratio @N for different configurations.}
%	\vspace{-.2cm}
%	\begin{tabular}{|p{0.2cm}|p{0.5cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|p{0.42cm}|}
%		\hline
%		& & \multicolumn{10}{c|}{\textbf{\LR}} & \multicolumn{10}{c|}{\textbf{\CR}} \\  \hline 		
%		& & \multicolumn{5}{c|}{\textbf{HR@10}} & \multicolumn{5}{c|}{\textbf{HR@15}} & \multicolumn{5}{c|}{\textbf{HR@10}} & \multicolumn{5}{c|}{\textbf{HR@15}} \\ \hline %\hline		
%		& & \textbf{$\Omega$=3} & \textbf{$\Omega$=4} & \textbf{$\Omega$=6} & \textbf{$\Omega$=8} & \textbf{$\Omega$=10} & \textbf{$\Omega$=3} & \textbf{$\Omega$=4} & \textbf{$\Omega$=6} & \textbf{$\Omega$=8} & \textbf{$\Omega$=10} & \textbf{$\Omega$=3} & \textbf{$\Omega$=4} & \textbf{$\Omega$=6} & \textbf{$\Omega$=8} & \textbf{$\Omega$=10} & \textbf{$\Omega$=3} & \textbf{$\Omega$=4} & \textbf{$\Omega$=6} & \textbf{$\Omega$=8} & \textbf{$\Omega$=10} \\ \hline %\hline		
%		%		& & \multicolumn{10}{c|}{\textbf{$\alpha=5\%$}} \\  \hline 
%		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\alpha=5\%$}}} & \textbf{k=5} & --- & 0.154 & 0.177 & 0.242 & 0.219 & --- & 0.154 & 0.189 & 0.252 & 0.237 & 0.159 & 0.158 & 0.145 & 0.113 & 0.103  & 0.178  & 0.177 & 0.163 & 0.138 & 0.120 \\ \cline{2-22}
%		& \textbf{k=10} & --- & 0.198 & 0.273 & 0.428 & 0.410 & --- & 0.198 & 0.317 & 0.455 & 0.442 & 0.140 & 0.141 & 0.165 & 0.149 & 0.140 & 0.184  & 0.190 & 0.201 & 0.185 & 0.174  \\ \cline{2-22}
%		& \textbf{k=15} & --- & 0.199 & 0.307 & 0.541 & 0.546 & --- & 0.199 & 0.368 & 0.580 & 0.580 & 0.154 & 0.163 & 0.188 & 0.198 & 0.189 & 0.200  & 0.227 & 0.235 & 0.250 & 0.229 \\ \cline{2-22}
%		& \textbf{k=20} & --- & 0.177 & 0.316 & 0.608 & 0.637 & --- & 0.177 & 0.388 & 0.658 & 0.670 & 0.112 & 0.135 & 0.207 & 0.188 & 0.194 & 0.168  & 0.191 & 0.268 & 0.235 & 0.250 \\ \hline	
%		%		& & \multicolumn{10}{c|}{\textbf{$\alpha=10\%$}} \\  \hline 
%		{\multirow{4}{*}{\rotatebox[origin=c]{90}{$\alpha=10\%$}}} & \textbf{k=5}  & --- & 0.247 & 0.240 & 0.242 & 0.210 & --- & 0.247 & 0.256 & 0.251 & 0.237 & 0.356 & 0.346 & 0.267 & 0.235 & 0.210 &  0.386 & 0.373 & 0.291 & 0.265 & 0.248   \\ \cline{2-22}
%		& \textbf{k=10} & --- & 0.380 & 0.418 & 0.428 & 0.320 & --- & 0.380 & 0.449 & 0.455 & 0.442 & 0.440 & 0.430  & 0.348 & 0.347 & 0.320  & 0.496  & 0.478 & 0.388 & 0.393 & 0.357  \\ \cline{2-22}
%		& \textbf{k=15} & --- & 0.439 & 0.505 & 0.541 & 0.390 & --- & 0.439 & 0.554 & 0.580 & 0.580 & 0.427 & 0.445  & 0.427 & 0.407 & 0.390  & 0.487  & 0.497 & 0.488 & 0.475 & 0.438  \\ \cline{2-22}
%		& \textbf{k=20} & --- & 0.443 & 0.547 & 0.608 & 0.431 & --- & 0.443 & 0.605 & 0.657 & \textbf{0.670} & 0.455 & 0.424 & 0.457 & 0.454  & 0.431 & 0.515  & 0.525 & \textbf{0.530} & 0.514 &  0.486 \\ \hline
%	\end{tabular}
%	\label{tab:Results}
%	\vspace{-.2cm}
%\end{table*}












%We perform the same study for the other two examined tools \ie PAM and \FC. Concerning the former, 
%As described in Table \ref{tab:ResultsPAM}, 

Results for PAM are reported in Table \ref{tab:ResultsPAM}. Similar to \UM, PAM is also not immune from attacks as it recommends to developers the fake APIs. However, PAM is less susceptible to manipulations compared to \UM since we get lower hit ratios. The maximum HR@N is 0.200, obtained when 
$\alpha$=20\% and $\beta$=60\%. 
Varying $N$ as well as $\Omega$ seems to have a negligible impact on the final results. This can be explained by considering the underlying algorithm of PAM, which retrieves APIs that appear more frequently. As the two APIs are planted together, they will be recommended commonly as a pattern. Therefore, adding one API does not significantly affect the final hit ratio. Overall, the results in Table \ref{tab:ResultsPAM} suggest that \emph{the use of PAM may be threatened by malicious attempts concealed in training data.}






%\MAX{should we explicitly say that here recommendations are different, i.e., snippets?}
Finally, we investigate how negative the effect might be for developers using \FC as their recommender, given that the training data has been manipulated. Note that for evaluating the system, we use the whole dataset with \numApps Android apps.
The maximum hit ratio is 0.203 and obtained when $\alpha$=20\%, $\beta$=60\%. In other words, users of the system are likely to be recommended with the manipulated code. 
The hit ratios for \FC recommendations are comparable to PAM, although \emph{(i)} in this case the training set is larger, and hence comparable values of $\alpha$ and $\beta$ mean a larger effort by the attacker; \emph{(ii)} since \FC provides to developers both APIs and snippets, the recommendation of a malicious API pattern may induce a serious consequence on the receiving client. In summary, also for \FC \emph{the seeded data has an adverse effect, \ie the tool is tricked into providing developers with the fake/toxic APIs, as well as code snippets}.


%the systems are prone to attacks coming from malicious data.
%Table~\ref{tab:ResultsUPMiner}, Table~\ref{tab:ResultsPAM}, and 


%\vspace{.05cm}
%\noindent
%$\rhd$~\textbf{\rqsecond} 

%\subsection{\rqfourth} \label{sec:RQ4}



%========================================
%\color{red}
%By adding more fake projects, we increase the hit ratio by both systems. For example, with \LR, for ($\alpha$=$5\%$, k=10, $\Omega$=6) HR@10 is 0.273; and for ($\alpha$=$10\%$, k=10, $\Omega$=6) HR@10 is 0.418. Similarly, with \CR, for ($\alpha$=$5\%$, k=20, $\Omega$=6), HR@10 is 0.207, while the corresponding HR@10 for $\alpha$=$10\%$ is 0.457. 
%The maximum hit ratio is reached, \ie HR@15 = 0.530 when $\Omega$=6 and \emph{k}=20. For \CR, the hit ratio decreases when $\Omega>6$, this means that an attacker should use a small $\Omega$ to get a higher hit ratio. For \LR, the maximum HR@15 is 0.670 and obtained when $\Omega$=10. %\emph{By adding more fake projects ($\alpha$), attackers can increase the number of infected clients by both systems. A small $\Omega$ is more dangerous to \CR, while a large $\Omega$ causes more harm to \LR.} 
%========================================


%It is worth noting that the performance of both systems is not affected by introducing the fake projects. %In two separate attempts, 
%as follows. We made use of %which is defined as 
%measured the accuracy of 
%Finally, we measured the prediction accuracy by means of success rate, \ie the ratio of projects getting at least a matched library (the intersection of the recommended list with the ground-truth data is larger than 0) to the number of testing projects. 

%===============================
%We ran \LR and \CR in two modes, \ie with and without fake projects, and realized that there is almost no difference in their success rate. Due to space limits, we report only the differences as average \emph{SR@N} in two modes, which is 2.6\% and 2\% for \LR and \CR, respectively. 

%This implies that the inadvertent inclusion of fake projects in the recommendation is difficult to notice, and cannot be detected by simply looking at variations in the accuracy values.
%===============================

\color{black}

Overall, RSSE could recommend malicious APIs or code snippets if being trained with malicious data. All three API RSSE are affected by adversarial attacks. Understanding the technical motivations behind such results is not in the scope of this paper. However, according to the performed analysis, \UM and PAM provide fake APIs for a considerably large number of projects, even when only 10\% of the training is manipulated. Though \FC is less prone than \UM, the consequences caused by its recommendations can be devastating as the tool supplies also code snippets.	

\vspace{.1cm}
\begin{shadedbox}
	\textbf{Answer to RQ$_2$.} Toxic training data can pose a prominent threat to the resilience of state-of-the-art RSSE, including \UM, PAM, and \FC.	
\end{shadedbox}

%, the resilience of the three systems,  is considerably compromised
% By conducting push attacks with

%Even with a simple fabrication, 
%\vspace{.1cm}
%\begin{shadedbox}
%	\small{\textbf{Answer to RQ$_4$.} By adding more fake projects ($\alpha$), attackers can increase the number of infected clients by both systems. A small $\Omega$ is more dangerous to \CR, while a large $\Omega$ causes more harm to \LR.}
%\end{shadedbox}

%\vspace{.1cm}% (The detailed scores for the experiments are not reported here due to space limit)

%while keeping a small number of fillers ($\Omega$)

%\begin{figure}[h!]
%	\centering
%	\vspace{-.4cm}
%	\includegraphics[width=0.86\linewidth]{figs/Results.pdf}
%	\vspace{-.2cm}
%	\caption{Experimental results.}
%	\vspace{-.2cm}
%	\label{fig:Results}
%\end{figure}













 





\subsection{Threats to validity} \label{sec:Threats}

%Something goes here.

Threats to \emph{construct validity} concern the relationship between theory and observation. In particular, they are related to the extent to which the simulated feeding of fake APIs or malicious snippets reflects a realistic AML attack  scenario. In our paper, we simply wanted to experiment with how a given percentage of projects with malicious snippets or APIs would affect the recommender's result. Evaluating the feasibility of a real attack is beyond the scope of this paper.

Threats to {\em internal validity} are the confounding factors internal to our study that might have an impact on the results. One possible threat is the choice of venues, \ie there may be AML-related research, as well as relevant RSSE to study, published in venues that we did not consider, for instance, security conferences such as the USENIX Security Symposium.\footnote{\url{https://www.usenix.org/conference/usenixsecurity20}} Nevertheless, as shown in Section \ref{sec:Collection}, we selected all major and topic-relevant software engineering journals and conferences, where RSSE are more likely to be found.

To evaluate the three API recommender systems, we used the original implementations of PAM\footnote{\url{https://github.com/mast-group/api-mining}} and \FC\footnote{\url{https://github.com/crossminer/FOCUS}} made available by their authors. Since the original replication package of \UM is no longer in use, we exploited the remake done by the authors of PAM. To minimize the threats that may affect the internal validity, we adopted the same experimental settings used in the original papers~\cite{Fowkes:2016:PPA:2950290.2950319,Nguyen:2019:FRS:3339505.3339636,Wang2013Mining}. Also, we ran our experiments with different systems configurations to evaluate their impact on the effects of AML attacks.

Threats to \emph{external validity} are related to the generalizability of our results. Such generalizability concerns \emph{(i)} on the one hand the recommenders on which the experimentation has been carried out (conclusions may or may not apply to other recommenders); and \emph{(ii)} on the other hand the considered dataset. For the former, in principle at least all the recommenders in Table \ref{tab:summary} are likely to treat legitimate and malicious APIs and snippets similarly. For the latter, both the push attacks and our evaluation are generalizable also to other languages, such as Python. 




%======================================
%The selection of the venues in our literature review could be subject to a threat to internal validity as it does not include all possible software engineering journals and conferences. However, the ones considered in this work are major venues in the domain, and thus we suppose that they are representative enough to cover the main line of research. Still, we believe that searching for work coming from different conferences and journals should ultimately eliminate the threat.
%journals and conferences in Software Engineering
%Moreover, we also attempted to simulate real-world scenarios, \ie the usage of the API recommender systems in practice, by running the experiments with different system configurations.
%we also evaluated the systems using exactly the same dataset and evaluation metrics. Furthermore, we ran several trials and counter-checks to validate the evaluation outcomes.
%======================================

%We plan to generalize DeepLib to data from GitHub in our future work. In fact, contributions in Maven come by strictly following a well-defined process, whichis not the case for GitHub repositories, where projects are uploaded in an ad hoc manner. In this respect, it is necessary to carefully investigate the performance of DeepLib on projects curated from GitHub.

%to gain advantage. 

==> src/Study.tex <==

%In this section, w
We conduct a preliminary evaluation of our proposed approach using a real dataset. Section~\ref{sec:ResearchQuestions} presents two research questions, while Section~\ref{sec:Process} describes the evaluation process. Section \ref{sec:dataset} gives a detailed description of the dataset used for the evaluation, and the metrics are specified in Section~\ref{sec:metrics}. Section \ref{sec:results} discusses the results by answering the two research questions. %are discussed in .  %We measure.



\subsection{Research questions} \label{sec:ResearchQuestions}
%In this feasibility study, w
%We address t
The following research questions are considered:
%\begin{itemize}
%\item 

\noindent
$\rhd$~\rqfirst~To answer this question, we compute precision, recall, and F-measure, considering real migration data from \GH. Furthermore, we conduct experiments following the ten-fold cross-validation methodology on a well-founded dataset. %to achieve better results.

\noindent
$\rhd$~\rqsecond~Besides the recommended migration steps, we are interested in measuring the time of the overall process, including the graph building phase.
%\end{itemize}

\vspace{-.1cm}
\subsection{Overall process} \label{sec:Process}
\vspace{-.2cm}
%To answer the research questions, 
As depicted in Fig.~\ref{fig:eval}, we perform experiments using the ten-fold 
cross-validation methodology on a well-founded dataset coming from an existing 
work~\cite{kula_developers_2018}. Given a list of projects, we download the entire 
dataset using the Crawler component. Then, the dataset is split into testing and 
training projects, 10\% and 90\% of the entire set, respectively, by each round of the 
process. Given a single testing project, \emph{Commit Analyzer} is used to capture the 
actual upgrade path followed by the repository, as stated in Section \ref{sec:tracker}. 
Concerning the training process, we build a different migration graph and calculate 
every possible upgrade plan for each TPLs extracted from the original dataset. To aim 
for a reliable evaluation, we select the start and the end version of a certain TPL from 
the actual plan of a testing project. This pair is used to feed \emph{Plan Calculator} 
that retrieves the proposed plan. 
%As we are interested only in upgrades, we do not consider the downgrade cases, \ie in 
%which a certain library migrates to an older version.
In such a way, we can compute on the two paths the metrics to assess the overall 
performances, \ie precision, recall, and F-measure.


\begin{figure}[t!]
	\vspace{-.5cm}
	\centering
	\includegraphics[width=0.86\linewidth]{figs/Eval.pdf}
	\vspace{-.4cm}
	\caption{The evaluation process.}
	\vspace{-.6cm}
	\label{fig:eval}
\end{figure}

\vspace{-.1cm}
\subsection{Data gathering} \label{sec:dataset}
\vspace{-.2cm}
%Concerning the dataset, 
We exploit an existing dataset which has been curated by a recent 
study,\footnote{\url{https://github.com/raux/Impact-of-Security-Advisories-on-Library-Migrations}}
 available on \GH. The dataset consists of 10,952 \GH repositories. The 
rationale behind this choice is the quality of the repositories which were 
collected by applying different filters, \ie removing duplicates, including 
projects with at least one \emph{pom.xml}, and crawling only well-maintained 
and mature projects. This dataset has been used to collect statistical 
information about library usages and dependency update. %Considering the 
%imposed quality filter, we decide to employ this dataset in the evaluation of 
%our tool. 
%To aim for a reliable evaluation, we experiment using the ten-fold cross-validation technique: %splitting the dataset in testing and training projects for each round of validation.
The training set is used to create a migration graph to avoid any possible bias. For each round, we tested 420 projects, and 3,821 projects are used to build the graph. 

\vspace{-.1cm}
\subsection{Metrics} \label{sec:metrics}
\vspace{-.2cm}
%To assess the proposed approach, 
%We make use of precision, recall, F-measure to measure the quality of retrieved migration paths. In particular, 
Given a migration path retrieved by \tool, we compare it with the real migration path extracted from a testing project. There are the following definitions: \emph{TP} is true positive, corresponding to the case the recommended path matches with the actual path extracted from the testing projects; False positive (\emph{FP}) means that the recommended upgrade plan is not present in the testing projects; False negative (\emph{FN}) is the migration steps that should be present in the suggested plan but they are not. Considering such definitions, we compute \emph{Precision}, \emph{Recall}, and \emph{F-measure} (or F$_1$-score) as follows. %according to their standard formulas used in Information Retrieval:
%\begin{equation}
%P = \frac{ TP }{TP+ FP}
%\end{equation}
%
%\noindent
%\begin{equation} \label{eqn:Recall}
%R = \frac{ TP }{TP+FN}    
%\end{equation}



\begin{minipage}{0.48\linewidth}
	\begin{equation} \label{eqn:Precision}%\nonumber%
	P = \frac{ TP }{TP+ FP}
	\end{equation}
\end{minipage}% 
\begin{minipage}{0.48\linewidth}
	\begin{equation} \label{eqn:Recall}%\nonumber%
	R = \frac{ TP }{TP+FN}    
	\end{equation}
\end{minipage}%\par\vspace{\belowdisplayskip}


\begin{equation} \label{eqn:F-Measure}
F_1 = \frac{ 2 \times P \times R  }{P + R}    
\end{equation}

\vspace{-.1cm}
\subsection{Preliminary results} \label{sec:results}

We report and analyze the obtained results by answering the research questions introduced in Section~\ref{sec:ResearchQuestions} as follows.


\vspace{.1cm}
\noindent
$\rhd$~\rqfirst~We compute the above-mentioned metrics on seven different popular Java libraries according to the Maven Repository's statistics,\footnote{\url{https://mvnrepository.com/popular}} namely \emph{junit}, \emph{httpclient}, \emph{slf4-api}, \emph{log4j}, \emph{commons-io}, \emph{guava}, and \emph{commons-lang3}. Table \ref{tab:metrics} reports the average results for the cross-fold validation evaluation. %Overall, \tool reaches good performance by considering the average values of the metrics computed over the ten rounds of validation.

\vspace{-.4cm}
\begin{table}[h]
\centering
\caption{Precision, Recall, and F-Measure.}%Metrics' results
\vspace{-.3cm}
\begin{tabular}{|l | p{1.3cm} |  p{1.3cm} | p{1.3cm} |}
\hline
\textbf{Library} & \textbf{Precision} & \textbf{Recall} & \textbf{F-measure} \\ \hline
junit &  0.93 &	\textbf{0.98} &	0.95 \\ \hline
httpclient & 0.75 &	0.64 & 0.68  \\ \hline
slf4j-api & 0.98  &	0.83 &  0.88  \\ \hline
log4j & \textbf{1.00}	&  0.95	& 0.97  \\ \hline
commons-io & 0.97 & \textbf{0.98} &	\textbf{0.98}  \\ \hline
guava & 0.87	&  0.80  &	0.83 \\ \hline
commons-lang3 & 0.73  & 0.78 &	0.72 \\ \hline
\end{tabular}
\vspace{-.4cm}
\label{tab:metrics}
\end{table}

%In particular, we notice that 
\vspace{.2cm}
\tool achieves the maximum precision for \emph{log4j}, \ie P=1.0 in all the rounds. Concerning recall, a value of 0.98 is obtained for the \emph{junit} and \emph{commons-io} libraries. In contrast, the tool achieves the the worst recall values for \emph{httpclient}, \ie while the minimum precision value is observed for \emph{commons-lang3} library, 0.64 and 0.73 respectively. \tool gets the best performance concerning F-Measure for \emph{commons-io}, \ie the score is 0.98. Altogether, we see that there is substantial difference between the performance obtained by \tool for different libraries. We suppose that this happens due to the availability of training data. In particular, by carefully investigating the clients that invoke \emph{httpclient}, we see that there are few migration paths among them, and this should have a negative impact on the overall recommendation.

% records  of the entire dataset
%as the F-measure value overcomes the other libraries' results.
\vspace{.1cm}
\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]
	\small{\textbf{Answer to RQ$_1$.} \tool is capable of predicting the correct upgrade plan given a real-world migration dataset.}
\end{tcolorbox}

%: all the quality metrics reach high values considering real-world data
%Though this is a preliminary evaluation, 

\vspace{.1cm}
\noindent
$\rhd$~\rqsecond~%As the second research question,
We measured the average time required for running experiments using a mainstream laptop with the following information: i5-8250U, 1.60GHz Processor, 16GB RAM, Linux as operating system. The measured time performance is as follows: the querying phase takes just 0.11 seconds to finish; the testing phase is longer: 145.44 seconds; and the most time consuming phase is the creation of graph with 15,120 seconds, corresponding to 280 minutes. It is worth noting that the testing consists of the sub-operations that are performed in actual use, \ie opening CSV files, extracting the actual plan, and calculating the shortest path. Roughly speaking, this means that in one second we can get an update plan for three clients. This is acceptable, given that the laptop used for the measurement possesses an average computational capability. We suppose that with a more powerful computing platform, the time performance can substantially be improved.

%We see that.

%The testing phase for all considered TPLs requires around 145 seconds on average.


%Finally, we computed the time required for a complete round of
%creation of the graph, the testing phase, and . Figure~\ref{fig:time} summarizes such phases by measuring the required time in seconds.
%the following operations 
% involved in the whole process
%computer  All the time measurements have been computed on a 
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=\linewidth]{figs/time.pdf}
%	\caption{Time required for each examined phase.}
%	\label{fig:time}
%\end{figure}

%As we can notice, graph creation is the most time consuming phase, it takes around 280 minutes to complete. Contrariwise, the recommendation of an upgrade path for a single TPL requires only 0,10 seconds on average. 



\begin{tcolorbox}[boxrule=0.86pt,left=0.3em, right=0.3em,top=0.1em, bottom=0.05em]
	\small{\textbf{Answer to RQ$_2$.} The creation of the migration graph is computationally expensive. However, it can be done offline, one time for the whole cycle. \tool is able to deliver a single upgrade plan in a reasonable time window, making it usable in the field.}
\end{tcolorbox}

%, and it can be done offline. 
%allows the usability of
%Concerning the recommendation phase, 

% it takes place at the beginning of the process
%Total number of repo & 10,000 & \textbf{Downloaded repo} & 9,517\\ 













